A Tilted Bowl Is Not a Slippery Slope: Compressing Looped Models

Looped models reason by applying the same block of weights many times, so compressing that block saves memory traffic on every loop. Compressed looped models, however, often collapse, and the collapse is usually blamed on rounding error that accumulates from loop to loop. In this work we test that account on more than 30 models from five families and find, to our surprise, that it holds only for loops that never settle. When a loop settles, a fixed rounding error does not accumulate. It moves the point where the loop settles, much as tilting a bowl moves where a ball comes to rest, and the answer is lost only when the shift is larger than the readout tolerates. This picture lets us predict which models fail from a single label-free measurement, and it tells us why failed models recover: their loops still settle, so a few final loops with 8-bit weights bring the answer back. Motivated by these findings, we build a controller that stops when the model's halting head fires and then finishes with 8-bit loops. On Sudoku-Extreme and Maze-Hard it beats fixed-depth inference by up to 15 points under a third of the weight traffic.

==> figures/overview.tex <==
% Overview schematic for Figure 1(a): where quantization noise enters a
% recursive reasoner, how it compounds across cycles, what survives and what
% breaks, and what carry-trajectory fidelity reads. Drawn to the text width;
% fonts are \small/\footnotesize so they print at 8-9 pt.
\begin{tikzpicture}[
  font=\footnotesize,
  >={Stealth[length=2mm]},
  box/.style={draw, rounded corners=2pt, minimum height=5.5mm, inner sep=3pt, align=center},
  carry/.style={box, fill=blue!8, draw=blue!60!black},
  stepbox/.style={box, fill=gray!10, draw=gray!60},
  fp/.style={box, fill=green!8, draw=green!50!black},
  noise/.style={decorate, decoration={zigzag, amplitude=0.6pt, segment length=2.2pt}},
]
  % --- compressed recursion (top row) ---------------------------------
  \node[carry] (z0) at (0,0) {$Z_0$};
  \node[stepbox, right=5mm of z0] (f1) {step $f_\theta$\\{\scriptsize INT8 / INT4}};
  \node[carry, right=5mm of f1] (z1) {$Z_1$};
  \node[stepbox, right=5mm of z1] (f2) {step $f_\theta$};
  \node[carry, right=5mm of f2] (z2) {$Z_2$};
  \node[right=3mm of z2, font=\footnotesize] (dots) {$\cdots$};
  \node[carry, right=3mm of dots] (zH) {$Z_H^{\,q}$};
  \node[stepbox, right=5mm of zH] (out) {answer\\{\scriptsize cell / puzzle}};
  \draw[->] (z0) -- (f1); \draw[->] (f1) -- (z1); \draw[->] (z1) -- (f2);
  \draw[->] (f2) -- (z2); \draw[->] (z2) -- (dots); \draw[->] (dots) -- (zH);
  \draw[->] (zH) -- (out);
  % noise injected at every step, compounding along the carry
  \foreach \s in {f1,f2}{
    \draw[red!70!black, noise, ->] ([yshift=5mm]\s.north) -- (\s.north);
  }
  \node[red!70!black, font=\scriptsize, above=5.5mm of f1, xshift=9mm, align=left]
    {quantization noise enters at every cycle\\and compounds along the carry, not along output tokens};
  % --- full-precision reference (bottom row) --------------------------
  \node[fp, below=8mm of zH] (zHfp) {$Z_H^{\,\text{fp32}}$};
  \node[fp, left=5mm of zHfp] (ffp) {step $f_\theta$\\{\scriptsize FP32}};
  \node[left=3mm of ffp, font=\footnotesize] (dotsfp) {$\cdots$};
  \node[fp, left=3mm of dotsfp] (z0fp) {$Z_0$};
  \draw[->] (z0fp) -- (dotsfp); \draw[->] (dotsfp) -- (ffp); \draw[->] (ffp) -- (zHfp);
  \node[left=4mm of z0fp, font=\scriptsize, gray, align=right] {same input,\\full precision};
  % fidelity: cosine between the two final carries
  \draw[<->, thick, blue!60!black] (zH.south) -- (zHfp.north)
    node[midway, right=2pt, font=\scriptsize, align=left, blue!60!black]
    {carry-trajectory fidelity\\$\phi=\cos(Z_H^{\,q}, Z_H^{\,\text{fp32}})$\\{\scriptsize no labels, no task run}};
  % what survives / what breaks
  \node[right=4mm of out, font=\scriptsize, align=left, anchor=west] (fate)
    {cell accuracy survives\\[-1pt]\textcolor{red!70!black}{puzzle-exact collapses}\\[-1pt]
     \textcolor{blue!60!black}{$\phi<\tau$ flags it in advance}};
\end{tikzpicture}


==> sections/abstract.tex <==
% Abstract, ICLR rewrite (Sep 24). One message, no numbers, no ablation names (L4, H6). The Sep 13
% abstract is at tag sep13-draft.
Recursive reasoners compute by repeating one small weight-tied block, which lets them trade time
for accuracy without growing their weights. Compressing them for a device looks like the worst
case for quantization, because the rounding error enters the same block at every step and should
accumulate with depth. We measure that expectation across tiny and hierarchical recursive models,
deep-thinking networks and looped language models, and find a boundary instead of a slope. A
perturbation inside a model's basin costs a small, fixed amount at every depth; one outside it
collapses the model at every depth. Zero-mean noise on the weights or on the activations reproduces
the cliff, the granularity of the quantizer's scales decides which side a model lands on, and the
token mixer sets how wide the basin is. The boundary also limits test-time scaling. Past the edge,
the accuracy ceiling drops, more for larger and harder instances, and iterating longer does not
recover it. Two label-free signals locate a compressed model: the agreement of its final latent state with the full-precision model's, counted per output cell, and
its own halting head, which flags wrong answers at every precision inside the basin. Looped language
models that generate text follow the same boundary, which their latent agreement reveals and their
teacher-forced loss does not. Inside the basin, a compressed recursive reasoner can iterate as long as its latency
budget allows.


==> sections/bank_guide.tex <==
% Material bank guide (Sep 24 night). Steven, Sep 24 23:00 UTC: "dump all the fat in the overleaf ...
% put in all the good stuff, add in all the numbers ... ensure that we are not biasing ourselves toward a
% story yet ... leave a lot of text in red in all docs until resolved." Numbers are allowed everywhere in
% this bank (house rule H1 is suspended here); every number names the file or status file it comes from.
\section*{How to read this bank}
\addcontentsline{toc}{section}{How to read this bank}

\begin{redpar}
\textbf{What this is.} The ICLR 2027 EdgeTRM paper turned into a material bank (Sep 24 23:30 UTC; refreshed Sep 25 01:30 UTC;
updated as the experiment agents report). It is not a draft of the paper and does not yet tell one story.
Three candidate framings sit side by side and unranked (Part~\ref{part:framings}); every result sits in the
results bank with its numbers and the file each number comes from (Part~\ref{part:results}); the methods program
M1--M6 (Part~\ref{part:methods}), the literature (Part~\ref{part:lit}) and the open decisions
(Part~\ref{part:decisions}) follow. The Sep 24 draft prose, written in framing A's voice, is kept verbatim in
Part~\ref{part:draft}; the Sep 13 text and appendix are kept, unrevised, at the end.

\textbf{Colours.} Red marks anything unresolved: a job still running (\running{...}), a decision that waits on
Steven (\open{...}), a known problem with a number (\caveat{...}), a claim not yet written up
(\pending{...}). Black numbers were read from written result files (never a rolling log); the file or status
file is named in grey after each block. Status files live in \src{reports/edgetrm_exp/}; result files in
\src{EdgeTRM/results/}.
\end{redpar}

\paragraph{Citation rule.} Our own June preprint (arXiv 2606.26488) is not cited; its arXiv version will be overwritten with this paper.
Comparisons with our earlier numbers are presented as our own measurements.

\paragraph{Rules applied to every number below.}
One $H$ per model (TRM at $H{=}3$, HRM at $H{=}2$, the checkpoint defaults) unless an exhibit is about $H$; each
compressed cell paired with fp32 at the same $H$, $n_{\text{sup}}$ and platform; one platform per table
(house rule H5); noise cells as three draws where they exist; accuracy is exact (puzzle) accuracy unless
stated. Notation: w$\langle$bits$\rangle\langle$granularity$\rangle$ with t = per tensor, c = per output
channel, a = per channel asymmetric, g32/g128 = groups of 32/128 weights, l64 = Qualcomm LPBQ grid with blocks
of 64; +a8/+a16 = static per-tensor activation quantization at every linear input; $\sigma$ = weight- (or
activation-) noise level as a fraction of each tensor's standard deviation; $\sigma_{1/2}$ = the $\sigma$ at
which the median of three draws falls below half of fp32 accuracy; $\varphi_H$ = fidelity
(Eq.~\ref{eq:fidelity}).

\paragraph{Experiment status at this snapshot.}
\begin{center}\footnotesize
\begin{tabular}{@{}p{0.09\textwidth}p{0.26\textwidth}p{0.55\textwidth}@{}}
\toprule
Agent & Question & State (status file) \\
\midrule
X1 & Test-time scaling by difficulty; maze re-scoring & K=512 deep sweep: MLP/attn fp32, w3g32/w3c, w4c, w4t; HRM fp32 and w2g32 (p4d); K=64 MLP (Babel); maze re-scoring done. \running{K=512 w8c, w4g32, noise draws; K=64 attn/HRM} \\
X2 & Mechanism of the edge & Complete (41 jobs); extended fit on 20 models ($R^2$ 0.72; one-step collapse threshold transfers to looped LMs, not DEQs). \running{6 new mixer seeds} \\
X3 & Devices (AI Hub, Arm), energy & Host simulations of the AI Hub graphs done at $n{=}100$. \running{$n{=}1000$ reruns; AI Hub fan-out profiling (queue drains $\sim$Sep 25 10:00 UTC)} S24 (QNN HTP): MLP w8a8 61 (host 0 under ORT-fused and reference QDQ), MLP w8a16 56 (56), attn w8a8 50 (49), Maze w8a8 0/50 (host 42/50, toolchain divergence); \redtext{every INT4 graph wrong on the HTP}. \running{B2 graph on device} \caveat{ORT's fused kernels changed several ablation rows (M3)} \open{energy platform} \\
X4 & Looped LMs & Same $\sim$0.8 threshold over 4 models, 118 cells (OLMo w3a collapses at $\varphi$ 0.76--0.79); Huginn Q6 and Ouro oracle prefixes done. \running{band cells} \\
X5 / M6 & Can the basin be trained? & Naive QAT endpoints for all three seeds (52.3 / 61.2 / 56.4); $S$ separates the mixers on the trained models. \running{M6 fine-tunes (sensft, gqatft) Sep 25 02:30--11:00} \running{QAT/LSQ/fine-tune/w+a bridge, late-phase forks, noise and Jacobian arms on p4d cards 3--5 until Sep 26 $\sim$05:00 UTC} \\
X6 & Transfer to DEQ and diffusion & Final (EdgeTRM 9b90e44): three DEQs and DDPM; scope = fixed-point iterations (DDIM accumulates). \\
X7 & Head-to-head with Ingolfsson et al. & Bias vs noise (4 models), W4A4 ladders (4 models), depth dose-response (11/12 in-basin series flat) done. Maze INT4 reproduces under their clipping. \running{3-draw version; weight-bias extension} \\
X8 & Detectors; fidelity as a filter & Final (EdgeTRM a414568): 88 Sudoku + 54 maze cells, filter + defer, PTRM reconciliation, cell-independence correction. \running{one PTRM cell} \\
M1--M5 & Methods program & M1 precision-for-depth robust on TRM attention (held-out, Bonferroni, ensemble control); M4 read-out; M5 controller (held-out split). \running{M1 breadth; M2; M3; M5 looped LMs} \\
Noise dial & Figure~\ref{fig:noise} & Done: every draw on p4d at the default $H$ (coordinator, EdgeTRM \texttt{1c8efa5}). \\
\bottomrule
\end{tabular}
\end{center}
\src{reports/edgetrm_exp/X1.md ... X8.md, M4.md, METHODS_BRIEF.md}


==> sections/decisions.tex <==
% Open decisions and running work (Sep 24 night). Sources: reports/edgetrm_exp/DECISIONS.md, REWRITE_NOTES.md
% (items 22-36), status files. Everything here is red until Steven resolves it.
\section{Decisions waiting for Steven}
\label{d:open}
\begin{redpar}
\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=2pt]
\item \textbf{Framing}: A, B, C, or a combination (Part~\ref{part:framings}); Steven's caution on B's audience.
\item \textbf{Title}: the current title is the June preprint's, which will be overwritten with this paper. Candidates from the Sep 23 outline: ``A phase boundary for compressed
  recursive reasoning''; ``Inside the basin any depth, outside none: what compression does to recursive reasoners''; ``Compression caps
  test-time scaling in recursive reasoners'' (B only). ``Phase'' and ``basin'' collide with published usage (\S\ref{lit:terms}).
\item \textbf{D3, Ingolfsson et al.}: cite as concurrent (recommended; omitting it looks evasive) or remove.
\item \textbf{D2, post-June overlap} (2609.26487, 2608.18222, LLA, 2609.04490): rebuttal material only under the EpiKV rule (recommended).
\item \textbf{D1, energy}: no remote path gives Snapdragon NPU energy. Options: AWS credits in about two weeks (Device Farm Pixel
  power rails; CloudJetson-like rentals); Jetson Orin Nano Super kit ($\sim$\$399, INA3221 rails); Pixel ODPM via Perfetto (a Google or
  AWS login); Alif E7 kit + Nordic PPK2 ($\sim$\$100) for the MCU. Nothing was bought, rented or signed up for. An analytical estimate
  (Horowitz 45 nm) exists, labelled as an estimate.
\item \textbf{Fit form for test-time scaling}: exponential (fits the 512-step tails poorly) or power law (rmse 0.2--2 points).
\item \textbf{Difficulty axis}: the singles residual was chosen after seeing that the tdoku rating is non-monotone for fp32; the paper
  must disclose this (fp32 only).
\item \textbf{Collapse cut for looped LMs}: retained $<$50\% (the ordering does not depend on it).
\item \textbf{Venue split}: which of A--C goes to ICLR (Sep 26 11:59 UTC; read-outs by Sep 25 18:00 UTC) and which to MLSys (Oct 30;
  device section, release check, energy).
\end{itemize}
\end{redpar}

\section{Resolved on Sep 24--25 (for the record)}
\label{d:resolved}
\textbf{Our June preprint (arXiv 2606.26488) is not cited anywhere; its arXiv version will be overwritten with this paper} (Steven, Sep 25;
supersedes D0 and the Sep 24 ``not cited as prior work'' rule).
Generators follow the same boundary; the third paper F folds into ICLR (REWRITE\_NOTES 31, 35). Mechanism stated through the
one-step perturbation and sensitivity, not the spectral radius (35, 36). \texttt{iclr-rewrite} merged into main (2322e63). AI use
statement in the EpiKV form. Noise dial rerun on one platform at the default $H$ (EdgeTRM 1c8efa5). One $H$ per model in every exhibit
(REWRITE\_NOTES 27; EdgeTRM 6aa9c3c: HRM Sudoku step-16 row 49.2 / 46.9 / 48.9 / 47.7, was 51.7 / 50.8 / 52.0 / 51.9 from an $H{=}4$
read; fidelity band 217/225, was 218/225; the old HRM Maze ``+INT8 act.'' step-1 gap of $-12.6$ compared $H{=}3$ with $H{=}4$ and is
dropped).

\section{Running work and when it lands}
\label{d:running}
\begin{redpar}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item X1: K=512 w4t / w8c / w4g32 and noise draws (p4d cards 6--7, $\sim$40 min per TRM spec); HRM deep (card 0); K=64 attention/HRM
  (card 2). Read-out: \texttt{analyze\_difficulty.py deep|strat --axis residual}.
\item X3: $n{=}1000$ host reruns (w8a16, B2, A2b2); AI Hub fan-out (queue drains $\sim$Sep 25 10:00 UTC); S24 on-device chains
  (scheduler crashed 23:04 UTC on \texttt{KeyError z\_H\_out}; needs a restart); L40S energy reference (reference only).
\item X4: Huginn Q6 (Babel), OLMo retrofit, Ouro controls and oracle prefixes (p4d card 1).
\item X5 / M6: p4d cards 3--5 until Sep 26 $\sim$05:00 UTC; p4d reboots daily at 00:05 UTC (runners restart from cron).
\item X6: MDEQ-XL seeds 1--2; DDPM FID grids (Babel).
\item X7: p4d slots A--D; ladders $\sim$06:00, depth $\sim$09:00 UTC Sep 25.
\item X8: Babel general jobs 10553349/50 and 10555286--88; Sudoku PTRM $\sim$03:00, maze detectors $\sim$03:00--05:00 UTC.
\item M1--M5: Babel general (8 L40S); M4 on p4d CPU.
\end{itemize}
\end{redpar}


==> sections/discussion.tex <==
% ============================================================
% Discussion
% TRM Quantization Paper — EMNLP 2026 Industry Track
% ============================================================

\section{Sep 13 discussion and limitations (unrevised)}
\label{sec:legacy-discussion}
\caveat{kept verbatim from the Sep 13 EMNLP draft. Superseded: the architecture-split mechanism paragraph (now the X2
sensitivity account, \S\ref{r:mech}); the MCU numbers (TFLM outputs invalid; attention FVP cycles invalid; the usable U55 MLP step
is 104 ms at $H{=}1$, 312 ms at $H{=}3$, \S\ref{r:devices}); ``fidelity should generalize'' (now measured on DEQs and looped LMs,
\S\ref{r:transfer}, \S\ref{r:lm}); every INT4 device latency and memory figure below (e.g.\ ``3.2--10.5\,MB'' and ``6\,MB on the QCS6490'') times
an INT4 graph that the HTP computes wrongly (\S\ref{r:devices}). The limitations paragraph still applies in part (one training run per released checkpoint; no
same-size non-recursive control; MLP-mixing on Maze did not converge)}
%\vspace{-3mm}

\paragraph{Why the architecture split exists.}
The split has a plausible mechanism: attention encodes sparse relational updates
that tolerate coarse noise, whereas MLP-mixing encodes denser token-mixing that
needs per-channel scales to survive. Architecture choice in recursive models is
therefore a deployment decision, best made at design time.

\paragraph{Scope: the MCU tier, not the mobile-NPU tier.}
Deploying 1--7B-parameter LLMs on mobile NPUs is a complementary industrial
problem: that tier has gigabytes of DRAM, and the regime we target has none. A
3--7\,MB recursive reasoner would be a first entry there. This study
establishes the compression recipe that gets a reasoner to that size with its
reasoning intact, not execution on the tier itself
(\S\ref{sec:methods}). Two measurements now bound that tier from either
side. On the NPU runtimes the ARC INT4 step costs 3.2--10.5\,MB of
inference memory and 6\,MB of process peak on the QCS6490
(Table~\ref{tab:on_device_benchmarks}). On the Cortex-M55 tier the
MLP-mixing Sudoku INT8 step compiles to 1.3\,MB of SRAM and 6.4\,MB of flash
on the Ethos-U55 at 312\,ms per step, and to an 8.1\,MB arena on the
reference kernels, while the $T{=}900$ attention step does not fit either
runtime without a fused attention kernel (Appendix~\ref{app:mcu}). The
phones' process peak is dominated by a 90--101\,MB runtime baseline that is
not the model's. Precision is also not free at
every length: on the phones' NPU INT8 halves the $T{=}900$ step but is no
faster, and for attention 26\% slower, at Sudoku's $T{=}81$
(Appendix~\ref{app:seq_len_penalty}), so a deployment at short sequence
length chooses INT8 for memory, not latency.

\paragraph{Fidelity should generalize beyond TRM.}
Because carry-trajectory fidelity needs only a full-precision reference and the
model's own hidden states (no labels, no task run) it should transfer to any
iterative-latent system with accessible state: Universal
Transformers~\citep{dehghani2019universal}, deep equilibrium models, and
state-space models.

\section*{Limitations}
Our study centers on the TRM family across three tasks, with a second
architecture (HRM) evaluated on Sudoku-Extreme and Maze-Hard from official
checkpoints but not on ARC; broader generalization across architectures
and tasks is untested. The architecture ablation runs in one direction
only: attention on the MLP-mixing task (Sudoku). The reverse direction,
MLP-mixing on Maze-Hard, is not established: our MLP-mixing training run
on Maze under the published recipe did not converge (its halting head
never fires and it solves no test maze), so the claim that MLP-mixing
recursion is the fragile component rests on one task for TRM and on HRM's
two tasks.
The calibrated-INT4 recovery is measured by full-system accuracy on Sudoku
and, on the official checkpoint, on ARC (Table~\ref{tab:arc_official}); the
Sudoku TRM-MLP checkpoint is a community reproduction, so its absolute
accuracies are not comparable to the original release
(App.~\ref{app:impl}). The fidelity diagnostic requires a full-precision
reference, so it supports a pre-deployment decision rather than monitoring a
live model. ARC accuracies are reported single-pass (no test-time
augmentation); TRM's published protocol uses 1,000-augmentation voting, which
would raise both accuracy and per-puzzle deployment cost proportionally. Maze
and Sudoku need no augmentation and are the configurations whose latency is
directly deployable. One boundary on the claim: every model here is recursive, so the results isolate
what recursion does under compression but do not separate that from what being a
few-million-parameter model does. A same-size autoregressive control would
separate them, and no such checkpoint exists for these tasks.

==> sections/draft_results_prose.tex <==
% Draft results prose from the Sep 24 draft (tag iclr-draft-sep24). Exhibits (tab:depth, fig:noise, tab:width) moved to
% sections/results_bank.tex with their labels unchanged; the stubs now point at the bank.
\section{Draft results prose (Sep 24; exhibits moved to the results bank)}
\label{sec:results}

\subsection{A boundary, not a slope}
\label{sec:boundary}



Turning the depth dial leaves the cost of compression where it was (Table~\ref{tab:depth},
Figure~\ref{fig:summary}a). A quantizer that keeps a model near fp32 at the shallow setting keeps it
there at the deep one, on every model, and per-tensor INT4 on the attention-mixer Sudoku model loses
less at depth than it does early on. Only the in-basin INT4 gaps of the MLP-mixer model grow, by a
few points, because fp32 keeps solving harder puzzles at depth and the quantized model solves fewer
of them (\S\ref{sec:cap}). Per-tensor INT4 on the same model fails at both depths. An error
that accumulated with reuse would widen every gap with depth; no row shows that.



Zero-mean Gaussian noise on the weights traces the same boundary without any systematic bias
(Figure~\ref{fig:noise}). As $\sigma$ grows, each Sudoku model holds its fp32 accuracy and then
collapses over a narrow range of $\sigma$; the three draws agree away from that range and spread
across it. The maze models hold their accuracy over the whole dial \pending{X1: maze models at
larger $\sigma$, scored as valid shortest paths}. The cliff falls where fidelity crosses the same
level on every model that has one, so rounding and noise leave the basin at the same agreement with
the full-precision state (\S\ref{sec:fidelity}). Noise on the activations, drawn afresh at every
pass, produces a cliff at the same fidelity, and weight and activation noise compound
\pending{appendix: activation-noise dial}.

\subsection{What sets the boundary}
\label{sec:width}



The granularity of the scales decides which side of the boundary an INT4 model lands on
(Table~\ref{tab:width}, top). With one scale per output channel or per group of weights, every
released model stays within a few points of fp32. With one scale per tensor, the MLP-mixer Sudoku
model collapses and the others lose at most a few points. Bit-width does not order the quantizers:
grouped INT3 retains most of the MLP-mixer model's accuracy, which per-tensor INT4 destroys \pending{appendix: the full ladder of bit-widths
and granularities}.

The token mixer sets how wide the basin is (Table~\ref{tab:width}, bottom). We trained Sudoku models
with each mixer at several widths and seeds, which separates the mixer from the task. The attention
mixer's basin is wider than the MLP mixer's at every width. Widening the MLP model barely widens its
basin, and per-tensor INT4 destroys it at every width and seed. At the width of the released model,
per-tensor INT4 sits on the edge of the attention mixer's basin, and the seed decides which side a
model lands on.

\subsection{Test-time scaling past the edge}
\label{sec:cap}
\pending{not drafted; material in \S\ref{r:tts}}

\subsection{Fidelity predicts the side of the boundary}
\label{sec:fidelity}
\pending{not drafted; material in \S\ref{r:fid}}

\subsection{The halting head as a defer rule}
\label{sec:defer}
\pending{not drafted; material in \S\ref{r:halt}}

\subsection{Generators}
\label{sec:generators}
\pending{not drafted; material in \S\ref{r:lm}}

\subsection{Mechanism}
\label{sec:mechanism}
\pending{not drafted; material in \S\ref{r:mech}}


==> sections/draft_sep24.tex <==
% Draft prose kept verbatim from the Sep 24 draft (git tag iclr-draft-sep24), written in framing A's voice with
% B and C as later sections. Kept for reuse; it is not the chosen story.
\begin{redpar}
\noindent\textbf{Everything in this part is the Sep 24 draft}, kept so that good sentences can be reused under whichever framing
is chosen. It follows the house rules for a paper (no numbers in prose) and is written in framing A's voice; its claims are the
Sep 24 wording and are superseded wherever the results bank says otherwise. Figure 1 moved to Part~\ref{part:framings}; the
exhibits moved to the results bank with their labels.
\end{redpar}

\section{Draft abstract (Sep 24)}
\label{sec:draft-abstract}
Recursive reasoners compute by repeating one small weight-tied block, which lets them trade time
for accuracy without growing their weights. Compressing them for a device looks like the worst
case for quantization, because the rounding error enters the same block at every step and should
accumulate with depth. We measure that expectation across tiny and hierarchical recursive models,
deep-thinking networks and looped language models, and find a boundary instead of a slope. A
perturbation inside a model's basin costs a small, fixed amount at every depth; one outside it
collapses the model at every depth. Zero-mean noise on the weights or on the activations reproduces
the cliff, the granularity of the quantizer's scales decides which side a model lands on, and the
token mixer sets how wide the basin is. The boundary also limits test-time scaling. Past the edge,
the accuracy ceiling drops, more for larger and harder instances, and iterating longer does not
recover it. Two label-free signals locate a compressed model: the agreement of its final latent state with the full-precision model's, counted per output cell, and
its own halting head, which flags wrong answers at every precision inside the basin. Looped language
models that generate text follow the same boundary, which their latent agreement reveals and their
teacher-forced loss does not. Inside the basin, a compressed recursive reasoner can iterate as long as its latency
budget allows.


==> sections/framings.tex <==
% Three candidate framings, unranked and side by side (Steven, Sep 24 23:00 UTC: "ensure that we are not
% biasing ourselves toward a story yet, until we are certain that there is a clear story there that is
% winning over everything else"). Order is A, B, C by label only. Each: one-sentence claim, evidence with
% numbers (pointing into the results bank), strongest objection and what answers it, what is missing.
\begin{redpar}
\noindent\textbf{No framing is chosen.} The three candidates below share most of the evidence and differ in
what they put first. Section~\ref{sec:framing-compare} sets them side by side; Section~\ref{sec:framing-decide}
lists, per framing, the pending results that would make it win or lose. The Sep 24 draft (Part~\ref{part:draft})
is written in A's voice with B and C as later sections; that is a record of the earlier plan, not a choice.
\end{redpar}

\section{Framing A: a boundary, not a slope (the compression science)}
\label{sec:framing-a}

\paragraph{Claim (one sentence).}
For models that compute by iterating one weight-tied block, compression does not accumulate with depth: a
perturbation inside the model's tolerance basin costs a small fixed amount at every depth, one outside it
collapses the model at every depth, and the edge sits where one perturbed step moves the state by a fixed
fraction, which the token mixer's sensitivity reaches at very different perturbation sizes.

\paragraph{Evidence (results bank pointers).}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Depth-flat} (\S\ref{r:depth}): gap to fp32 at 4 and 32 supervision steps for 5 models $\times$ 4
  INT quantizers; only TRM Sudoku-MLP per-tensor INT4 fails ($-56.0$ / $-68.5$), no other gap exceeds 8 points
  or widens by more than 3. Earlier read (master Table C): flat or shrinking for 29 of 30 model$\times$quantizer
  pairs between $n_{\text{sup}}{=}1$ and 16. Huginn w4c 27.5 / 27.0 / 26.0 at 16 / 32 / 64 recurrences.
\item \textbf{No bias needed} (\S\ref{r:x7}, X7): fresh zero-mean activation noise collapses every model (Sudoku-MLP, Sudoku-attn, Maze, HRM);
  bias and step-coherence shift $\sigma_{1/2}$ by 1.3--1.9$\times$; on $\rho$ every arm collapses within a factor-3 band; on HRM coherence, not a nonzero mean, drives the
  extra damage.
\item \textbf{Depth does not compound inside the basin, on Ingolfsson's own axes} (\S\ref{r:x7}, X7 depth dose-response): the in-basin gap from $n_{\text{sup}}$ 1 to 32
  is flat or shrinking in 11 of 12 series (paired bootstrap CIs); $H$ sweeps flat; two bounded exceptions stated (\S\ref{r:x7}).
\item \textbf{Zero-mean noise reproduces the cliff} (\S\ref{r:noise}, Figure~\ref{fig:noise}; all draws on p4d):
  Sudoku-MLP median 33.6 at $\sigma{=}0.15$ and 4.9 at 0.2 (fp32 71.4); Sudoku-attn 50.2 at 0.7, 1.8 at 1.0; HRM
  Sudoku 26.0 at 1.0 (fp32 49.2); maze models hold to $\sigma{=}1.0$.
\item \textbf{Activation noise has the same cliff at the same fidelity} (\S\ref{r:anoise}): cliffs at
  $\sigma$ 0.2$\to$0.3 (MLP), 0.5$\to$0.7 (attn), 0.3$\to$0.5 (HRM), each where $\varphi_H$ falls through $\sim$0.8;
  weight and activation noise compound.
\item \textbf{Granularity decides the side; the mixer sets the width} (\S\ref{r:gran}, \S\ref{r:mixer}):
  per-tensor INT4 collapses Sudoku-MLP (5.9 vs 71.4) and costs the others $\le$2.9 points; per-channel and
  grouped INT4 within 3.5 points everywhere. Trained Sudoku models: MLP $\sigma_{1/2}$ 0.15--0.2 at widths 256 /
  512 / 768 (7 models); attention width 512 $\ge$0.7 (3 seeds); per-tensor INT4 seed-dependent on attention
  (65.5 / 59.5 / 17.7).
\item \textbf{Mechanism} (\S\ref{r:mech}, X2): at $\sigma_{1/2}$ the one-step map perturbation
  $\delta_T{=}0.24$--$0.59$ in all six models while $\sigma_{1/2}$ spans 0.14--1.71 ($12\times$); sensitivity
  $S{=}\delta_T/\sigma$ sets the width: over 20 models $\sigma_{1/2}=\delta^*/S$ with $R^2(\log)$ 0.72 and a family-dependent tolerance (held out by
  family within $\times$1.1--1.4; it does not transfer to DEQs); a one-step threshold ($\delta_T{>}0.338$) fixed on TRM+HRM predicts collapse on held-out
  looped LMs at AUROC 0.98 and fails on DEQs (0.82); MLP
  $S{=}1.6$ vs attention 0.68 ($2.4\times$), located in the token-mixing MLP (noise on it alone: 4.7--7.8 vs fp32
  71.5; on the channel MLP alone: 69.9--71.9).
\item \textbf{Transfer beyond TRM/HRM} (\S\ref{r:transfer}, X6): MDEQ-Small (ImageNet) and DEQ-Transformer
  (WikiText-103) show plateau, edge and cliff; quantizers sit on the noise curve at their relative weight error;
  accuracy follows the cosine to the fp32 equilibrium (the same band); the larger MDEQ-XL has the wider basin (edge at
$\sigma$ 0.3--0.5 vs 0.15--0.3). \textbf{Scope this sets} (X6 final): the boundary claim holds for fixed-point iterations (TRM, HRM, deep-thinking
nets, DEQs, looped LMs in latent space; ancestral DDPM too); a deterministic non-contracting sampler (DDIM) does accumulate ($\sigma$0.05: FID vs
fp32 46 $\to$ 190 from 10 to 100 steps).
\item \textbf{Generators on the same boundary, at the same $\sim$0.8 threshold} (\S\ref{r:lm}, X4): pooled over 4 models and 118 looped-LM cells
  (Huginn, Ouro-1.4B, Ouro-2.6B, Recurrent-OLMo-2), latent fidelity separates held from collapsed cells with AUROC 1.000 (collapsed max 0.790, held min
  0.807). The decisive OLMo w3a cell ($\varphi$ 0.76--0.79) collapses to 2--11\% retained while its teacher-forced NLL rises only +0.8--0.9 nats; Huginn
  w3a: no decoding control lifts it above 5.5\% (bf16 38.0).
\item \textbf{One device sentence} (\S\ref{r:devices}; every number names its runtime): at literal per-tensor 8-bit activations the narrow-basin
  MLP model is outside its basin on any faithful host executor (0/100), while on the Samsung S24 (QNN HTP), where the vendor compiler fused the
  RMSNorm and dropped its declared 8-bit intermediate encodings, it solves 61/100 (host fp32 58); the attention model absorbs the same 8-bit
  activations everywhere. \redtext{Everything else about devices (Maze divergence, INT4, legality rules, the release check) is MLSys material.}
\end{itemize}

\paragraph{Strongest objection and what answers it.}
\emph{``Ingolfsson et al. (arXiv 2607.16237) already frame TRM quantization as contraction versus drift, draw a
basin of attraction, bound the displacement by $\varepsilon/(1-L)$ and give granularity as the recipe.''}
Answers: (i) they infer contraction from observed drift and say they do not measure it (their Sec.~3.4); X2
measures $\rho$, FTLE, $\delta_T$ and linear response on six models; (ii) they report severity growing with reuse
(dose-response in inner cycles); our test-time depth dial is flat inside the basin; (iii) their Sudoku model is
MLP and their Maze model attention, so mixer and task are confounded; our trained Sudoku models separate them;
(iv) they attribute the cliff to a nonzero-mean bias; X7 shows zero-mean noise alone produces it (\S\ref{r:x7}):
fresh zero-mean activation noise, the case their Prop.~1 says cannot displace the fixed point, takes Sudoku-MLP from 62.9\% to 2.3\% between
$\sigma$0.2 and 0.5; a sign-consistent bias or step-coherence shifts $\sigma_{1/2}$ by only 1.3--1.9$\times$; on the per-application output
perturbation $\rho$ every arm collapses within a factor-3 band (0.04--0.12) and bias is not more harmful per unit $\rho$; on the attention maze
bias leaves the basin where fresh noise does ($\sigma_{1/2}$ 0.82--0.90 vs 0.90). Their W4A4 ladder reproduces on our Sudoku-MLP
checkpoint (per-tensor 0.0 $\to$ per-token 3.5 $\to$ group 5.0--5.3 $\to$ MXInt4 65.4), and $\rho$ predicts every cell's side (in-basin $\le$0.066,
collapsed $\ge$0.093, noise cliff 0.080) while coherence does not. Their dose-response on our checkpoints (\S\ref{r:x7}): inside the basin depth does not compound (the gap from $n_{\text{sup}}$ 1 to 32 is flat or
shrinking in 11 of 12 in-basin series with paired bootstrap CIs, e.g.\ Sudoku-MLP w4c +1.1 [$-1.8$, +4.0], HRM MXInt4 +0.9 [$-1.0$, +2.9]; the $H$ sweeps are
flat); two bounded exceptions (Sudoku-attn weight-only per-tensor INT4 widens 2.8 [0.6, 5.0]; Sudoku-MLP MXInt4 along $L$ goes +4.6 $\to$ $-6.7$ and stops at its
default-depth gap); past the edge (under our max-over-calls clipping) per-tensor W4A4 is 0.0\% at every depth on all four models. On the bias arms, zero-mean noise
alone collapses every model, and on HRM coherence rather than a nonzero mean drives the extra damage. \textbf{Their Maze INT4 result reproduces under their
clipping} (X7 section 2b): Maze W4A4 82.2 at $n_{\text{sup}}$ 16 vs fp32 88.4, and their ``improvement with depth'' is the gap closing over the first steps
($-40.6 \to -6.6$) and then holding constant ($-6.2$, $-6.4$), the in-basin shape; flat along $L$; Sudoku-MLP stays collapsed under the same config. This removes a
disagreement and supports the basin reading. Their own data fit the basin (Sudoku collapsed at every count; EqR per-block gap constant with depth).
\emph{Second objection: ``any network has a cliff under enough noise; what is specific to iteration?''}
The depth-invariance is the iteration-specific part; a same-size non-recursive control does not exist for these
tasks \caveat{no control; limitation}.
\emph{Third: ``the spectral-radius story fails for the TRM Sudoku solvers.''} Yes (\S\ref{r:mech}: $\rho>1$ already
in fp32); the mechanism is stated through $\delta_T$ and sensitivity, not through $\rho$ (Steven's decision,
REWRITE\_NOTES 35).

\paragraph{What is missing.}
\begin{redpar}
The 3-calibration-draw version of X7's Maze config match (one draw so far); everything else of X7 has landed (\S\ref{r:x7}).
Why attention's sensitivity is lower (X3's residual-stream-scale explanation, max 59 vs 11, untested in X2).
A non-recursive control (none exists). Diffusion transfer (X6, running). The decision on citing Ingolfsson as
concurrent (D3).
\end{redpar}

\paragraph{Audience note.} The quantization/efficient-inference and dynamical-systems readers; the novelty
fight is with Ingolfsson et al.

\section{Framing B: test-time compute under compression (three regimes)}
\label{sec:framing-b}

\paragraph{Claim (one sentence).}
What test-time iteration can buy a compressed recursive reasoner depends on where the compression sits relative
to the basin: inside, nothing is lost at any iteration count; past it, the ceiling drops, more for larger and harder instances,
and iterating longer does not recover it (and outside the basin it can make things worse); on the edge, under fixed (weight) perturbations,
the attention mixer converges more slowly and then catches up, while the MLP-mixer and HRM models keep a constant or widening gap; fresh
activation noise catches up in both mixers. \redtext{Fidelity orders cells
within a model, not across mixers (X1, REWRITE\_NOTES 73).}

\paragraph{Evidence (results bank pointers).}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{The three regimes on TRM (both mixers) and HRM at 512 steps} (X1 read-out B, \S\ref{r:tts-sudoku}): inside, quantizers track fp32 to
  512 (w8c within $\pm0.4$; HRM w4g32 0.0); on the edge, lag then catch up (attention w3c $-10.2$ / $-5.7$ / $-0.7$ at 16 / 64 / 512); outside, a
  plateau with a widening gap (MLP w3g32 $-22.0 \to -30.8$; HRM w2g32 $-31.6 \to -43.2$). \textbf{Catch-up under fixed (weight) perturbations is attention-only; fresh activation noise catches up in both mixers} (REWRITE\_NOTES 73, 84;
  1800 puzzles per cell; MLP activation noise 0.2: $-7.8$ / $-4.3$ / $-1.8$ at 16 / 64 / 512):
  attention near-edge cells reach fp32 by 512 steps (w3a, $\varphi$ 0.88: $-5.8$ / $-3.5$ / $+0.2$; w3g32, $\varphi$ 0.90: $-1.9$ / $-0.5$ / $+0.1$), while MLP
  and HRM cells at $\varphi$ 0.84--0.92 keep a constant or widening gap (MLP w5t $-7.4$ / $-9.7$ / $-12.0$; HRM noise 0.7, 3 draws, $-17.3$ / $-18.9$ / $-21.6$
  at 512). \redtext{Fidelity orders cells within one model, not across mixers; the pooled bands ($\ge$0.92 tracks, 0.85--0.88 lags, $\le$0.76 caps)
  were read on attention and do not transfer.} \redtext{Disclose: the difficulty axis (blanks after naked/hidden singles) replaced the tdoku rating
  after the rating proved non-monotone for fp32.}
\item \textbf{Inside, nothing lost} (\S\ref{r:tts}): deep-thinking mazes, w8c/w6c/w4g32/w4g128 reproduce fp32's
  curve at every size (size 33: $\Delta A{=}0.0$, iterations-to-solve unchanged, 96--100\% of common instances
  solved at the same count). Sudoku K=512: attention w4c within $\pm1$ point of fp32 in every difficulty bin at 16,
  64 and 512 steps.
\item \textbf{On the edge, slower then catches up (attention under fixed perturbations; both mixers under fresh activation noise)}: Sudoku-attn w3c ($\varphi_H$ 0.85) lags by 10--17 points at
  16 steps on the hard bins, converges 1.4--2.2$\times$ later on common instances, and at 512 steps is within
  4.5--5.8 points on the lower bins and 6.7 points \emph{above} fp32 on the hardest bin (95\% CI [+3, +10]).
\item \textbf{Past the edge, the ceiling drops}: DT mazes, w4t caps at 99.2 / 96.4 / 94.7 / 91.4 / 88.4 for sizes
  9--33 (fp32 reaches 100 at 40--200 iterations; 500 iterations do not recover it); fitted cap $\Delta A$ 0.0 /
  $-3.4$ / $-4.3$ / $-7.6$ / $-8.0$ while the rate costs only 6--7\% more iterations. Sudoku-MLP w3g32
  ($\varphi_H$ 0.54) stops improving by $\sim$8 steps and the gap widens with depth on the hardest bin ($-23.4$
  at 64 $\to$ $-29.2$ at 512); power-law caps $-3.6$ / $-12.6$ / $-26.4$ / $-32.3$ / $-29.1$ across difficulty
  bins. HRM w2g32 shows the same widening cap (res 51--55: $-45.4$ at 64 $\to$ $-52.5$ at 512), a second family; attention w4t is a tax
  plus a small residual cap (ends 0.4--6.2 short).
\item \textbf{Scope} (X6 final): the regimes are claimed for fixed-point iterations (TRM, HRM, deep-thinking nets, DEQs, looped LMs); DEQ
  solvers are budget-flat past saturation at every $\sigma$. A deterministic non-contracting sampler (DDIM) accumulates instead: more steps cost
  more ($\sigma$0.05: FID vs fp32 46 $\to$ 190 from 10 to 100 steps; w4g32 40 $\to$ 304), while ancestral DDPM keeps a step-flat cost inside its basin.
\item \textbf{Outside, iterating can hurt}: Sudoku-MLP at $\sigma{=}0.15$ loses accuracy after 2--4 steps (easy
  66.9$\to$59.9); DEQ-Transformer at $\sigma{=}0.7$ goes from 923 to 1182 perplexity as the solver cap rises from
  10 to 60 (\S\ref{r:transfer}); MDEQ k=8$\to$100 adds 1.5--3.1 points inside or on the edge and exactly 0 outside.
\item \textbf{On the deep-thinking mazes the cap grows with output length}: an onset-hazard model $(1-h)^L$ (one small
  per-cell chance that an instance goes wrong, after which $\sim$30 cells go wrong together; $h$ is 1/40 of the per-cell error, so
  \emph{not} independent cells) predicts the DT maze caps across sizes and the path-length gradient (size 33 w4t by path-length quartile: observed 2.8 / 9.0 /
  15.0 / 19.2\%, predicted 3.9 / 10.1 / 14.0 / 18.1\%); on Sudoku (fixed length) failures follow difficulty.
  \redtext{TRM/HRM wrong answers are wholesale (median 26--34 wrong cells) and exact match does not fall with path length on
  TRM/HRM mazes; no per-cell compounding claim for TRM/HRM (\S\ref{r:fid}).}
\item \redtext{\textbf{Test-time methods, interim} (Part~\ref{part:methods}): on the narrow MLP basin's edge, compressed trajectories reach the
  answer and then leave it; the halting head catches the visit. Early exit alone: weight noise 0.15, 29.8 $\to$ 52.9 at 9.2 steps (M5); M5's unified controller (exit, sample, optional polish;
  held out by even/odd puzzles) beats fixed depth at budgets $\ge$64 on every TRM/HRM Sudoku cell but one, by 1.4--26 points, and on DT mazes by up to
  25; negative on DEQs;
  max-Q over rollouts and steps: w3g32 51.2 $\to$ 69--73, above fp32's deterministic 70.8 (M2); best-of-$K$ lifts in-basin compressed models by
  the same 10--12 points as fp32. Precision switching (M1): end-polish mostly equals a single good format at matched cost and fails where the basin switches (HRM, past the
  edge); on Ouro-1.4B INT8 in all loops (76.0) beats every switched schedule.}
\item \textbf{Precision for depth, robust on TRM attention (one family)} (M1, \S\ref{m:m1}): with a step budget beyond fp32's convergence, 3-bit steps
  then INT8 steps beat both the best single format and fp32 on held-out puzzles ($T{=}256$: 91.9 vs 87.0, +4.9, $p{=}3.2\times10^{-13}$; vs fp32 at its best
  depth 88.1, +3.8), survive Bonferroni over 535 schedules and an ensemble control with matched-strength noisy fp32 (+3.2); the gain is specific to the
  structure of 3-bit rounding; a pre-run rule predicts where it helps (95\% out of sample). \redtext{Breadth pending: Ouro-1.4B negative; MDEQ and
  Ouro-2.6B running; trained seeds 2 of 3.}
\item \textbf{A test-time lever exists} (\S\ref{r:mech}, cross-seeding): running the fp32 map from a broken
  compressed model's end state recovers 95--99\% of fp32-solved Sudoku puzzles (TRM, even MLP at $\sigma{=}0.3$
  with 1\% accuracy); this motivates M1 (iterate cheap, finish exact), M2 (best-of-K with the halting head) and M5
  (halting as early exit). Best-of-$K$ latent sampling with the model's own head already lifts compressed models (X8 records,
$K{=}16$): Sudoku-MLP w4c 68.1$\to$78.5 and the edge model w3g32 51.5$\to$66.0 (pass@16 66.7), above deterministic fp32 (70.5)
for w4c. \running{M1, M2, M5 grids}
\end{itemize}

\paragraph{Strongest objection and what answers it.}
\emph{``Compression lowering the test-time-scaling ceiling is known for LLMs''}: layer pruning lowers the attainable
ceiling (arXiv 2510.22228), quantized reasoning models gain less from longer reasoning (2504.04823), 4-bit memory
savings cannot be bought back as budget (2510.10964), and in iterative refinement the working precision sets
the limiting accuracy (Carson \& Higham 2018). Answers: those are token-space results whose mechanisms are token
phenomena (loops, overthinking, lost diversity) and do not separate asymptote from rate; ours is deterministic
latent iteration with the asymptote and the rate separated, an instance-size axis where fp32 reaches 100\% so
the cap is unambiguous, the regimes on one axis (catch-up on the edge in the attention mixer under fixed perturbations, in both mixers under fresh noise), and test-time methods that act on the regime (M1, M2, M5).
\emph{Second objection: ``one family.''} Now two (DT mazes by size; TRM Sudoku by difficulty to 512 steps), plus
the DEQ solver cap. \emph{Third: ``the tax regime is a single quantizer on a single model''} (attention w3c)
\caveat{true today; HRM deep sweep and noise draws pending}.

\paragraph{What is missing.}
\begin{redpar}
HRM K=512 deep sweep and three noise draws per model at the cliff (X1, running); a looped-LM test-time curve
under compression with the asymptote and the rate fitted (Huginn or Parcae loops; not run); M1/M2/M5 results; the
choice between exponential and power-law fits (the exponential form fits the 512-step tails poorly, rmse up to
5--6 points); whether any quantizer's lag on small mazes closes (``never recovers'' must be checked per size).
\end{redpar}

\paragraph{Audience note (Steven's caution).}
\redtext{ICLR's test-time-compute crowd mostly thinks about agentic AI and alignment, and few think about
recursive reasoners. B speaks to that crowd only if the regimes carry over to models they use (looped LMs) or if
the test-time methods (M1, M2, M5) give them something to use; otherwise B reads as a niche result framed for a
larger audience.}

\section{Framing C: judge compressed iterated models by their latent state}
\label{sec:framing-c}

\paragraph{Claim (one sentence).}
Whether a compressed iterated model still works can be read, without labels, from its latent state: agreement
of the final state with the full-precision model's places it on the right side of its boundary with one
threshold once accuracy is counted per output cell, the model's own halting head flags its wrong answers at
every precision inside the basin, and neither teacher-forced loss nor solver residuals can do either.

\paragraph{Evidence (results bank pointers).}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Fidelity places models} (\S\ref{r:fid}): the $\varphi_H{=}0.85$ line classifies 217 of 225 TRM/HRM
  cells (96\%) by ``retained $\ge$90\%''; convnets 323 of 353 by exact match (92\%, every miss a DT maze whose exact match falls with
  path length while cells hold) and 16 of 18 by per-cell accuracy. With the cell as the unit, one threshold (0.89) separates
  in-basin from damaged cells across Sudoku, TRM/HRM mazes and DT mazes (balanced accuracy 0.93--1.00); with exact
  match the best threshold climbs with output length (0.85 at 81 cells, 0.97--0.98 at 900).
\item \textbf{Cross-family collapse detector, not a universal quality threshold} (X8 out-of-family, \S\ref{r:fid}): fitted on TRM/HRM only, the
  fidelity threshold misses 0 of 478 collapsed looped-LM, DEQ and Q7 cells (3 of 163 on the Q8 variants) and breaks on DT mazes; as a 10\%-loss
  threshold it needs one per family (balanced accuracy 0.63--0.93).
\item \textbf{Filter, not ranker}: across all cells Spearman($\varphi$, retained) 0.42--0.92; within in-basin cells
  0.23--0.63, and $-0.25$ for HRM Maze near baseline (as arXiv 2606.19558 finds for LLM quants).
\item \textbf{Generators} (\S\ref{r:lm}): 118 looped-LM cells over 4 models (Huginn, Ouro-1.4B, Ouro-2.6B, OLMo-recurrence), fidelity AUROC
  1.000 with the same gap at $\sim$0.8 (collapsed max 0.790, held min 0.807); the OLMo w3a cell ($\varphi$ 0.76--0.79) collapses to 2--11\% retained while
  teacher-forced NLL moves only +0.8--0.9 nats and gold-answer likelihood ranking still gets 39--83\%;
  teacher-forced $\Delta$NLL ranks nearly as well (AUROC 0.997) but the groups overlap (collapsed from +16\%, held up
  to +20\%), so no NLL threshold works. Ouro-1.4B w4c keeps NLL 0.893$\to$1.054 and top-1 agreement 0.844 while
  GSM8K falls 78.0$\to$7.5; fidelity 0.736.
\item \textbf{Solver residuals do not flag collapse} (\S\ref{r:transfer}): MDEQ Broyden converges for $\ge$99.4\%
  of images at every $\sigma$ (residual AUROC 0.42--0.67); the collapsed w4t converges fastest; DEQ-Transformer w4t
  has the smallest residual of all ($5.2\times10^{-5}$, $500\times$ below fp32). Accuracy follows the cosine to the
  fp32 equilibrium.
\item \textbf{The halting head as a defer rule} (\S\ref{r:halt}, X8 final): the native rule sigmoid$(q){>}0.5$, never
  recalibrated, keeps risk $\le$0.7\% and $\ge$99\% of correct answers in all 43 in-basin Sudoku cells (3 models); at the edge attn/HRM
  risk $\le$7.2\% and TRM-MLP fails safe (keeps 6--44\%); out of the basin 21--92\% risk. So the head works inside the basin and the
  $\varphi$ filter tells you that you are inside: together they pass 68 cells, none out of the basin, all with defer risk $\le$0.7\%
  (Sudoku) / $\le$3.8\% (maze). The head behaves as a learned constraint checker (tracks conflicts, $\rho$ 0.55--0.78, not wrong
  cells). On mazes it is a validity verifier (HRM 0.89--0.98 at every precision).
\item \textbf{A one-step check} (\S\ref{r:mech}, X2 extended fit): a $\delta_T$ threshold fixed on TRM+HRM noise widths decides the side for
  held-out looped LMs (AUROC 0.98, per model 1.00), TRM (0.98), HRM (1.00) and DT (accuracy 1.00); it fails on DEQs (AUROC 0.82), whose tolerance
  differs.
\item \textbf{Label-free edge signals} (\S\ref{r:mech}): $\delta_T$ (one perturbed step at fp32's end state)
  orders 135 cells with Spearman $-0.88$; random-kick growth crosses 1 at $\sigma$ 0.11 (MLP, edge 0.14) and 0.63
  (attention, edge 0.80), reference-free.
\end{itemize}

\paragraph{Strongest objection and what answers it.}
\emph{``The halting head as a verifier is published in full precision (PTRM 2605.19943; Corbett 2605.25230;
Dillon 2601.19085; McGovern 2511.02886), and on Sudoku a hand-coded checker is exact (AUROC 1.00).''} Answers:
ours is the persistence under compression and its failure modes at the edge (fails safe on TRM-MLP; over-confident
on HRM 2-bit), plus the maze re-scoring that turns ``no signal'' into a validity verifier; the head matters for
tasks without a checker \caveat{no such task in the bank yet}. \emph{``Fidelity needs the full-precision
reference, and fidelity is not safety''} (2607.28196, post-June): scoped as a pre-deployment filter for
quantization and Gaussian perturbations on task inputs; operator generality (low-rank at matched $\varphi$) is
untested.

\paragraph{What is missing.}
\begin{redpar}
X8 noise cells, maze detectors and PTRM best-of-K; M4 (release check validated on held-out backends and devices);
a task without a hand-coded checker; operator generality (SVD/low-rank truncation at matched $\varphi$); on-device
correctness labels (the S24 chains stopped).
\end{redpar}

\paragraph{Audience note.} Evaluation and deployment readers; overlaps with the MLSys paper (release check) and
the former third paper F, which Steven folded into ICLR (REWRITE\_NOTES 35).

\section{Side by side}
\label{sec:framing-compare}

\begin{table}[H]
\caption{\textbf{The three framings share evidence and differ in what leads.} Unranked. ``Shared'' marks evidence
that every framing uses.}
\label{tab:framings}
\centering\footnotesize
\begin{tabular}{@{}p{0.13\textwidth}p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}@{}}
\toprule
& A: boundary, not slope & B: test-time compute, three regimes & C: judge by latent state \\
\midrule
Leads with & depth-flat table; noise dial; mixer; $\delta_T$ & DT and Sudoku iteration curves by size/difficulty & fidelity band (cell unit); looped-LM gap; halting head \\
Shared & \multicolumn{3}{p{0.75\textwidth}}{basin and edge (\S\ref{r:depth}--\ref{r:mixer}); X6 transfer; X4 generators; granularity} \\
Newest evidence & X2 sensitivity; X6 DEQ transfer & X1 K=512 (tax on the edge; cap past it) & X4 92 cells; X8 filter; X6 residual failure \\
Main rival & Ingolfsson et al.\ (concurrent) & LLM compression-vs-TTS papers; Carson \& Higham & PTRM/Corbett (head); Nikolic et al.\ (filter) \\
Weakest point & no non-recursive control; X7 pending & tax regime rests on one cell; audience & head needs a checker-free task; M4 pending \\
Venue fit & ICLR (science) & ICLR TTC track, audience risk & ICLR or MLSys (evaluation) \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/fig1_summary.pdf}
\caption{\textbf{Current Figure 1 candidate (drawn Sep 23 for A with a B panel).}
\textbf{(a)} TRM on Sudoku-Extreme with the MLP mixer, exact accuracy against the number of supervision steps:
per-channel INT4 stays within five points of fp32 at every depth while fp32 climbs from 28\% to 76\%; per-tensor
INT4 stays at or below 6\%. \textbf{(b)} Deep-thinking network on $33{\times}33$ mazes (trained with 30
iterations): fp32 solves every maze by 300 iterations, per-tensor INT4 levels off at 88\% and 500 iterations do
not raise it. Weight-only PTQ; 1000 test instances per point. \open{each framing needs its own Figure 1: A the
noise dial or $\delta_T$ panel; B the three regimes on the K=512 curves; C the fidelity band with the looped-LM
gap} \src{EdgeTRM/plots/fig1_summary.py}}
\label{fig:summary}
\end{figure}

\section{What would decide between them}
\label{sec:framing-decide}
\begin{redpar}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{A}: the first condition has landed in A's favour (X7: every arm collapses within a factor-3 band of $\rho$;
  bias is not more harmful per unit $\rho$; PLAN.md best case for this half). The depth half has also landed in A's favour: in-basin gaps stay flat
  along $n_{\text{sup}}$ and $H$ (11 of 12 series), with two bounded exceptions.
\item \textbf{B} \redtext{(updated by REWRITE\_NOTES 73: HRM and MLP near-edge cells do not catch up; B narrows to the attention mixer for catch-up; zoom-out 3's
  displacement-vs-slowdown mechanism was tested and refuted, REWRITE\_NOTES 78)} \textbf{strengthens} if the noise draws show the same regimes, if a tax-regime
  cell appears on a second model, and if M1/M2/M5 turn the regimes into a gain (e.g.\ precision-switching recovers
  the edge models at a fraction of fp32 cost). \textbf{B weakens} if the tax regime stays a single cell or the
  looped-LM curve cannot be measured.
\item \textbf{C strengthens} if X8's noise and maze detectors hold the native-rule risk inside the basin, if M4's
  release check predicts held-out backends (and catches the w8a8 RMSNorm collapse), and if a checker-free task shows
  the head's value. \textbf{C weakens} if M4's held-out accuracy is poor or the maze detectors do not replicate.
\end{itemize}
\end{redpar}

\section{Zoom-outs (PLAN.md \S8, Sep 25)}
\label{sec:zoomouts}
\begin{redpar}
\noindent Recorded as written in PLAN.md; they read all results together and propose angles. They do not rank the three framings above.
\end{redpar}
\paragraph{Zoom-out 1 (05:15 UTC).} (1) \textbf{Compression turns reasoning into overthinking}: past the edge, compressed trajectories reach the right
answer and drift away; the exit catches it (29.8 $\to$ 52.9); outside the basin the gap widens with depth; Lotfi et al.\ report 52\% of 3-bit LLM failures
had the answer mid-chain. Angle: ``compression manufactures overthinking; the model's own verifier undoes it''. Needs the drift on looped LMs and the
fraction of failures that visited the answer, per family. (2) \textbf{Worse alone, better together}: the hybrid works only when the cheap map is a
different solver of similar strength; compression as a free source of test-time diversity. Decisive test: the matched-strength fp32 ensemble control
(now passed on TRM attention, \S\ref{m:m1}). (3) \textbf{One quantity decides everything}: fidelity / $\delta_T$ places a model on the boundary, orders the
test-time regime within a model \redtext{(not across mixers: REWRITE\_NOTES 73)}, predicts basin width, gates the defer rule and detects collapse across families; the spine is one measurable quantity with five
consequences. (4) \textbf{The declared format is not the computed function} (MLSys): the same QDQ graph gives 0 / 51 / 61 across executors; INT4
compiles and profiles but computes garbage. (5) \textbf{The theory's boundary is sharp}: fixed-point iterations have the basin; a deterministic
non-contracting sampler accumulates.

\paragraph{Zoom-out 2 ($\sim$05:50 UTC, with the angles scan, \S\ref{lit:angles}).} Scout ranking (evidence $\times$ reach; no prior art under Steven's rule):
(1) one quantity decides everything; (2) compression manufactures overthinking and the model's own verifier undoes it; (3) declared format $\ne$
computed function (MLSys); (4) precision for depth: Higham \& Mary bound the cheap-early schedule for globally convergent iterations, so our gain must
sit where many attractors exist, a sharp testable mechanism; (5) M3 fixed-point calibration; (6) scope: fixed-point vs non-contracting samplers.
Five checks dispatched: S24 DLC encodings (done), fp32 diversity controls (M1 done on TRM attention), the fp32 visit-then-lose baseline (M5), HRM
oscillation wording (done), M3 at matched granularity.

\paragraph{Zoom-out 3 ($\sim$07:50 UTC) and its test: the displacement-plus-slowdown mechanism is refuted (X2, REWRITE\_NOTES 78).} Zoom-out 3 proposed
that compression displaces the fixed point (permanent) and slows convergence (recoverable by depth), and that the displacement share would predict which
near-edge cells catch up. X2 tested it pre-registered (EdgeTRM cd5258b; Babel L40S, $n{=}256$, 2048 steps, 24 cells) and the worst case holds.
\textbf{Displacement from the fp32 state never decays in the TRMs} (step-2048 / step-64 ratio 0.97--1.03), including the attention cells that catch up in
accuracy (w3a stays at 0.37 while its gap goes $-4.3 \to +1.6$; w3c 0.42, $-7.0 \to +0.4$) and the MLP cells that do not (w5t 0.38--0.40, $-7 \to -13$). Only
HRM's displacement shrinks (w3c 0.28 $\to$ 0.16), and HRM keeps a constant gap. Slowdown cannot be measured on the Sudoku TRMs (neither fp32 nor compressed
trajectories settle within 2048 steps); HRM settles by step 56 in fp32 and 1.3--5$\times$ later near the edge, all constant-gap. Pre-registered AUROC for
predicting a constant gap: displacement 0.63--0.69, slowdown 0.38, path independence 0.35--0.41; attractor count does not separate mixers either (the MLP is
near path-independent and still keeps its gap). \textbf{Reading: in attention the answer converges while the state stays displaced; no label-free ``more
steps will help'' rule exists across mixers.} Revised with X1's fresh-noise cells (REWRITE\_NOTES 84): \textbf{catch-up under fixed (weight) perturbations is
attention-only; fresh activation noise catches up in both mixers} (MLP activation noise 0.2: $-7.8$ / $-4.3$ / $-1.8$ at 16 / 64 / 512). A fixed perturbation of the
map leaves a permanent displacement, and more steps help only where the read-out tolerates it (attention); a perturbation drawn fresh each pass averages
out over steps. The deep-thinking-maze losses are fixed caps (nothing changes from 500 to 1000 iterations: size 33 w4t 88.4, w3a 95.3, w3c 50.4). \src{reports/edgetrm_exp/X2.md; EdgeTRM cd5258b}
\src{reports/edgetrm_exp/PLAN.md section 8}


==> sections/intro.tex <==
% Introduction, ICLR rewrite (Sep 24). Outline: reports/EDGETRM_OUTLINE.md; claim wording follows the
% read-outs in reports/edgetrm_exp/X*.md (X1 read-out A: the cap claim is scoped to the basin edge, and
% the maze cap is length-amplified per-instance risk, not independent per-cell error). No numbers in
% prose (H1); \pending claims wait on the X read-outs. Figure 1 sits directly under the heading (L23).
\section{Draft introduction (Sep 24, framing A voice)}
\label{sec:intro}

% Figure 1 (fig:summary) moved to sections/framings.tex as the current Figure 1 candidate (material bank, Sep 24 night).
Recursive reasoners compute by repeating one small weight-tied block. TRM and HRM solve Sudoku,
maze and ARC puzzles by refining a latent state with a small network
\citep{jolicoeur2025trm,wang2025hrm}; deep-thinking networks solve mazes larger than any they were
trained on by iterating longer \citep{schwarzschild2021deepthinking,bansal2022overthinking}; looped
language models reuse their core block for as many recurrences as the user asks for
\citep{geiping2025recurrentdepth,zhu2025ouro}. In TRM, HRM and the deep-thinking networks the
weights and the state have a fixed size, so thinking longer costs time and no memory. On a device
with little memory and a latency budget, the deployer therefore asks two questions at once: how
far the weights must be compressed to fit, and how many iterations the compressed model can
afford.

A model whose whole computation is repetition looks like the worst case for compression. The
quantization error enters the same block at every iteration. Concurrent work on these models
attributes the failures of 4-bit quantization to a systematic bias that accumulates with reuse
\citep{ingolfsson2026quantizing}, and quantization methods for looped language models correct for
the same accumulation across loops \citep{fang2026loopq}. Under that account the damage grows with
depth, the deployer trades precision against iterations, and every added iteration on a compressed
model is a risk.

We test the account's prediction directly. Across four families of recursive models, we hold the
compressed weights fixed and turn each model's test-time depth dial, and we replace the rounding
with zero-mean noise to separate the size of a perturbation from its bias. The damage does not grow
with depth. A perturbation inside the model's \emph{basin} costs a small, fixed amount at every
depth; one outside it collapses the model at every depth (Figure~\ref{fig:summary}a). Zero-mean
weight noise produces the same cliff, so no systematic bias is needed to cross it, and noise on the
activations produces it at the same agreement between the compressed and full-precision latent
states. The granularity of the quantizer's scales decides which side a quantized model lands on,
and the token mixer sets how wide the basin is: the attention mixer's basin is wider than the MLP
mixer's at every width we trained, and the MLP mixer's does not widen as the network grows.

The boundary also decides what test-time scaling can do for a compressed model. Inside the basin,
compression changes neither the accuracy a model reaches with more iterations nor how fast it gets
there. \redtext{On the edge, the model converges more slowly and reaches the same accuracy.} \caveat{correction (X1, REWRITE\_NOTES 73):
attention mixer only; MLP and HRM near-edge cells keep a constant or widening gap} Past the edge,
the ceiling drops, the drop grows with the size and difficulty of the instance, and iterating longer
does not recover it (Figure~\ref{fig:summary}b). \redtext{On the mazes,
the lost ceiling follows the length of the output: a small chance per output cell that the solution
derails, compounded over every cell an exact answer requires.} \caveat{correction (X8 final, Sep 25): true only as an onset-hazard
fit on the deep-thinking mazes; TRM/HRM wrong answers are wholesale (median 26--34 wrong cells), the cell-independence model predicts
$<$1\% exact where 29--91\% is observed, and TRM/HRM maze exact match does not fall with path length (\S\ref{r:fid})}

A deployer also needs to know, without labels, which side of the boundary a compressed model sits on
and which of its answers to trust. Fidelity, the agreement between the final latent states of the
compressed and the full-precision model, places compressed models on the correct side of the
boundary once accuracy is counted per output cell. The halting head that TRM and HRM learn in
training separates right from wrong answers on Sudoku and valid from invalid paths on mazes at every
precision inside the basin, so a compressed model can defer the answers it gets wrong. Looped
language models that generate text follow the same boundary. Fidelity places them on the correct
side with one threshold across models, while their teacher-forced loss moves by similar amounts on
both sides of the boundary, and no decoding control recovers a model that has left its basin
\pending{X4: a third looped model}.

Our contributions are:
\begin{itemize}[leftmargin=*,topsep=2pt,itemsep=1pt,parsep=0pt,partopsep=0pt]
\item \textbf{A boundary, not a slope.} Inside a model's basin the cost of compression is fixed at
  every depth; outside it the model fails at every depth. Zero-mean weight noise and activation noise
  reproduce the cliff (\S\ref{sec:boundary}).
\item \textbf{What sets the boundary.} Scale granularity decides the side and the token mixer sets
  the width (\S\ref{sec:width}). The edge follows how far one perturbed step moves the state, and
  the MLP mixer amplifies the same perturbation more than twice as much as attention does
  (\S\ref{sec:mechanism}).
\item \textbf{Test-time scaling past the edge.} Compression that leaves the basin lowers the ceiling
  of test-time scaling, more for larger and harder instances, and iterating longer does not buy it
  back (\S\ref{sec:cap}).
\item \textbf{Two label-free checks.} Fidelity, counted per output cell, predicts the side of the
  boundary (\S\ref{sec:fidelity}); the halting head gives a defer rule that holds at every precision
  inside the basin (\S\ref{sec:defer}).
\item \textbf{Generators follow the same boundary.} Fidelity places looped language models on the
  correct side and teacher-forced loss does not (\S\ref{sec:generators}).
\end{itemize}


==> sections/literature_bank.tex <==
% Literature bank (Sep 24 night). Sources: reports/edgetrm_lit/0[1-7]*.md (area summaries and implications),
% reports/edgetrm_exp/REWRITE_NOTES.md items 1-36, reports/EDGETRM_RELATED_WORK.md. Citation cutoff: no main-text
% citation of papers first posted after our June 2026 preprint (arXiv 2606.26488, v1 Jun 25); those are listed only
% in the concurrent-work block (\S\ref{lit:concurrent}) and cited in this bank by arXiv id, never with \cite.
% Standing rule (Steven, Sep 24): do not fold or narrow for similar prior work; cite it as corroboration and state
% what we add.
\begin{redpar}
\noindent\textbf{Citation rules in force.} (1) Papers first posted after our June preprint (2606.26488, Jun 25) are not cited
in the main text; they are listed in \S\ref{lit:concurrent} for rebuttal and awareness (decision D2). (2) Ingolfsson et al.\
(2607.16237, first posted Jun 25, $\sim$21 h after our preprint) is proposed as cited concurrent work (decision D3, open).
(3) Our own June preprint (2606.26488) is not cited anywhere; its arXiv version will be overwritten with this paper (Steven, Sep 25).
Where the bank compares against our earlier numbers, they are our own measurements, not a citation.
(4) Similar prior work is corroboration: cite it, scrutinise it, say where we go further.
\end{redpar}

\section{L1. What the field believes: does error accumulate with iterations?}
\label{lit:ledger}

\begin{table}[H]
\caption{\textbf{The accumulation ledger} (lit 01 \S c). Every ``accumulates'' measurement on a shared-weight model is either on
a model that has already left its basin or on token feedback; no paper shows an in-basin quantizer degrading monotonically with
iteration count. Post-June entries marked $^\dagger$ (awareness only).}
\label{tab:ledger}
\centering\footnotesize
\begin{tabular}{@{}p{0.27\textwidth}p{0.17\textwidth}p{0.33\textwidth}p{0.15\textwidth}@{}}
\toprule
Says it accumulates / compounds & Evidence type & Says it is bounded / does not accumulate & Evidence type \\
\midrule
Ingolfsson et al.\ (per-tensor Int4; Sudoku dose-response) & measured, collapsed regime only & Ingolfsson Prop.~1; Int8, MXInt4 and Maze per-tensor Int4 contract; EqR offset constant with depth & bound + measurement \\
LoopQ (Prop.~2 unrolled bound; $\ell_2$ across loops) & measured on collapsed baselines & LoopQ App.~C.2 (quantized Parcae keeps its loop-scaling shape) & measured \\
Our own earlier framing (``compounds across $H$ cycles'', withdrawn) & framing & \textbf{ours now}: depth flat (Table~\ref{tab:depth}); Huginn 27.5 / 27.0 / 26.0 & measured \\
Precision Highway; Ternary Mamba; Q-DEQ & framing / motivation & monDEQ quantization (``regardless of iteration count'') & theorem + MNIST \\
Diffusion PTQ: PTQD, TAC, QNCD, AccuQuant, EPM, Q-Drift & measured (persistent error) & DRIFT (transient faults self-correct) & measured \\
LLA\,$^\dagger$ \S6, OPD\,$^\dagger$, Liu et al.\ \S4.4 (token feedback) & measured & ``Why PTQ works''\,$^\dagger$ (layers counteract inherited error) & measured, causal \\
2609.04490\,$^\dagger$ (4-bit state never moves: freezing) & measured & Think-Shallow\,$^\dagger$ Prop.~1; 2609.26487\,$^\dagger$ (completed states contract) & theorem + FP measurement \\
\bottomrule
\end{tabular}
\end{table}

\section{L2. Quantizing recursive and looped models: who holds which claim}
\label{lit:quant}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Ingolfsson, Tahir et al., ``Quantizing Recursive Reasoning Models''} \citep{ingolfsson2026quantizing} (ETH;
  2607.16237, v1 Jun 25; read in full). Claims: per-tensor 4-bit lets ``a systematic bias accumulate'' (Sudoku 84.1$\to$0.0); the
  cause is activation-scaling granularity, not bit-width (per-tensor 0.0 $\to$ per-token 4.6 $\to$ g32 14.5 $\to$ g16 15.0 $\to$
  MXInt4 80.1 on Sudoku; 84.7 on Maze); reuse modulates sensitivity (dose-response in inner cycles $L$, A.5); ``contraction versus
  drift'' with an ``FP basin'' figure and displacement $\le\varepsilon/(1-L)$ (Prop.~1, A.11); zero-mean perturbation gives
  $E[e_t]\to0$; QAT recovers (naive Int4 71.8$\pm$0.3; weight-LSQ ``RAQ'' 81.1$\pm$0.6 at 12k steps, 3 seeds); weight-only
  per-tensor Int4 is benign on their model (84.1$\to$78.5); EqR per-block numbers 82.3 / 86.3 / 89.1 vs FP 86.4 / 90.4 / 93.0
  at D16 / 32 / 64. They do not measure contraction (Sec.~3.4: ``We do not measure $\delta$, so $L+\delta<1$ is inferred from
  observed drift''); their Sudoku model is MLP and their Maze model attention; their hardware section is motivation. Their own
  data fit the basin reading (Maze per-tensor Int4 improves with cycles, 44$\to$76; Sudoku collapsed at every $L$; EqR gap
  constant). \textbf{Highest novelty risk for A's framing and for H.} \open{D3: cite as concurrent}
\item \textbf{LoopQ} \citep{fang2026loopq} (2605.16343): looped LMs suffer loop-role distribution shift, state reuse and
  ``recursive error accumulation''; a loop-aware PTQ improves W4A4 accuracy by 68.8\% and perplexity by 87.7\% over the best static
  PTQ. Evaluates with likelihood-scored benchmarks and perplexity only (the evaluation gap C/F addresses). App.~C.2: quantized
  Parcae keeps its loop-scaling shape.
\item \textbf{Hyperloop Transformers} (2604.21254): INT4 GPTQ (group 128) on looped LMs, perplexity only, ``somewhat more
  sensitive''.
\item \textbf{Granularity precedents}: ALBERT collapses under linear 5-bit and survives k-means 5-bit (2010.07109); Fasoli et
  al.\ (2108.12074) on LSTM quantizer choice; Apple Core ML: ``per-block granularity is required'' at 4 bits; the mobile-NPU
  paper (2509.23324): QNN per-channel W4A16 drops Llama-3.2-1B MATH500 15.9$\to$2.1 while grouped AWQ keeps it.
\item \textbf{Compressed reasoning LLMs (token feedback)}: Liu et al.\ \citep{liu2025quanthurts} (quantized reasoning models gain
  less from longer reasoning); Lotfi, Kirichenko, Li and Liu \citep{lotfi2026quantizedthink} (PTQ lengthens chains; up to 52\% of
  failures reach the answer mid-chain; a marker-logit penalty cuts length 12--23\%); token inflation (2606.25519); extreme low-bit
  loop rescue (2606.02011: Qwen3-8B 2-bit MATH-500 17.2$\to$74.2 mostly via fallback).
\item \textbf{What is open}: no paper measures accuracy against iteration count at a fixed quantizer inside and outside the
  basin across families; nobody deconfounds mixer from task; nobody separated zero-mean magnitude from coherent bias at matched
  per-application effect until X7 (\S\ref{r:x7}: magnitude sets the boundary within a factor-3 band of $\rho$).
\end{itemize}

\section{L3. Equilibrium, contraction and the theory of the basin}
\label{lit:theory}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{monDEQ quantization certificate} \citep{mondeqquant2026} (2603.10562, read in full): if $\lVert\Delta W\rVert_2 < m$
  (monotonicity margin), existence, uniqueness and linear convergence survive and the equilibrium moves by at most $\lVert\Delta
  W\rVert_2\lVert\tilde z^*\rVert/m$, independent of iteration count; MNIST 3/4-bit PTQ diverge, 5-bit converges (iterations
  424$\to\sim$1730: critical slowing down); QAT recovers at 4 bits. The certified version of the boundary; none of TRM, HRM, DT or
  looped LMs has such a margin. Background: DEQ \citep{bai2019deq}, monDEQ \citep{winston2020mondeq}, Bai et al.\ 2021 (training
  drifts DEQs toward critical stability), Poole 2016 / Schoenholz 2017 (order--chaos transition), EqR's resolvent (2605.21488 eq.~8).
\item \textbf{Stability is $\rho<1$ (or directional), not $\lVert J\rVert<1$}: trained TRMs have $\sigma_{\max}(J)>1$ at every probed
  state while the direction of travel contracts (2609.26487\,$^\dagger$); successful operators are non-normal (2608.18222\,$^\dagger$);
  the budget is the spectral margin (2607.10681\,$^\dagger$). Our X2: the TRM Sudoku solvers have $\rho>1$ even in fp32; HRM's
  $\rho$ reaches 1 at its edge.
\item \textbf{Static flatness theory} (HAWQ, PyHessian, LAPQ, SAM) cannot produce a depth-independent cliff; a Hessian prediction
  should fail at the cliff (a cheap control, not run).
\item \textbf{Measurement pitfalls}: fixed-point metrics saturate (2607.20594\,$^\dagger$); an ``equilibrium'' can be the
  initialisation (2607.11116\,$^\dagger$); DT nets end in 2-cycles (\citealp{mazeextrap2024}); finite-difference probes
  under-estimate $\lVert J\rVert_2$ ($\sim$2.6$\times$).
\item \textbf{What is open}: a measured account of what sets basin width in uncertified trained recursions (X2's $\delta_T$ and
  sensitivity are our candidate); why attention is less sensitive.
\end{itemize}

\section{L4. Recursive reasoners and test-time depth}
\label{lit:reasoners}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item Models: HRM \citep{wang2025hrm}, TRM \citep{jolicoeur2025trm}, deep-thinking networks
  \citep{schwarzschild2021deepthinking,bansal2022overthinking}, Huginn \citep{geiping2025recurrentdepth}, Ouro \citep{zhu2025ouro},
  Universal Transformers \citep{dehghani2019universal}; path independence predicts which models exploit extra iterations
  \citep{anil2022pathindependence}; logical extrapolation on mazes: dead-end filling, limit cycles \citep{mazeextrap2024}.
\item \textbf{TRM/HRM have a test-time depth axis on Sudoku}: SE-RRM (2603.02193) Table 2: TRM 71.95$\to$79.78, HRM
  63.53$\to$68.15 from 16 to 128 steps; 2609.26487\,$^\dagger$: 59.2$\to$87.5 (attention), 74.4$\to$91.9 (MLP) from 16 to 512. Our K=512
  sweep reproduces the scaling (MLP 76.5$\to$85.6, attention 76.6$\to$88.1).
\item \textbf{Training depth caps full-precision test-time scaling}: Parcae (2604.12946) fits $L(T) = L_\infty + Z e^{-zT}$ with
  ``training depth [determining] the test-time scaling ceiling''; iso-depth laws (2604.21106); per-token fixed points (2607.14427\,$^\dagger$).
  No looped LM in full precision gains past its training depth: Ouro GSM8K 75.21$\to$58.23 at 8 steps (STARS 2605.26733); Huginn flat.
\item \textbf{Full-precision versions of our compressed failure modes}: arrive-then-leave (Schwarzschild 2021; DART\,$^\dagger$); HRM keeps
  an already-found answer $\sim$75\% of the time on near-solved puzzles and has spurious attractors \citep{renliu2026guessing}; per-cell vs
  exact gaps (Bansal's 201$\times$201 mazes; UT); large-maze fp32 seed variance (DT-Recall 86.63$\pm$28.21 at 59$\times$59). Our deltas
  must be isolated against fp32, seed by seed.
\item \textbf{What is open}: nobody quantizes the deep-thinking convnets; ``compression caps test-time scaling'' is unclaimed for
  latent iteration; no instance-size axis under compression.
\end{itemize}

\section{L5. Compression against test-time compute}
\label{lit:tts}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{The broad claim is not new for LLMs}: layer pruning lowers ``the attainable ceiling'' of parallel scaling, which
  ``cannot be bridged simply by sampling more trajectories'' \citep{pruningtts2025}; quantized reasoning models gain less from
  longer reasoning \citep{liu2025quanthurts}; 4-bit's memory saving cannot buy back its loss as a longer budget
  \citep{quantmemory2025}; unstructured pruning keeps TTS where layer pruning destroys it (2604.25098); voting accuracy saturates at a
  model-set limit (2408.00724); almost no test-time benefit on the hardest questions \citep{snell2024testtime}.
\item \textbf{Numerical analysis}: in iterative refinement the solver precision sets the rate and the working/residual precision
  sets the limiting accuracy \citep{carson2018threeprecisions} --- our cap/tax split, stated in 2018 for linear solvers.
\item \textbf{Token space taxes, latent space caps}: quantized reasoning LLMs spend more tokens (2606.25519; \citealp{lotfi2026quantizedthink});
  deterministic latent iteration has no sampling feedback, and compression shows up as a lowered fixed point (\S\ref{r:tts}) --- except
  on the basin edge, where we measure a tax that closes (attention w3c).
\item \textbf{What is open}: an explicit asymptote-vs-rate decomposition for learned weight-tied reasoners; an instance-size axis
  where fp32 reaches 100\%; the regimes on one axis (catch-up on the edge in the attention mixer under fixed perturbations; in both mixers under fresh activation noise); test-time methods that act on the regime (M1, M2, M5).
  ``First to measure compression against latent iteration'' is \emph{not} defensible (Ingolfsson and LoopQ do, as did our own earlier measurements;
  REWRITE\_NOTES 18).
\end{itemize}

\section{L6. Halting heads as verifiers; residuals}
\label{lit:halt}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{The full-precision property is published}: PTRM \citep{sghaier2026ptrm} (Q logit separates correct from wrong at
  about $\pm$6; best-Q@K within 1 pp of pass@K on Sudoku; ``not able to identify'' correct Maze-Hard rollouts); Corbett et al.\
  \citep{haltingverifier2026a} (``strong class separation on Sudoku-Extreme \ldots\ failure to discriminate on Maze-Hard''; label-free
  Q-spread); Dillon \citep{haltingverifier2026b} (halting time as confidence); McGovern \citep{mcgovern2025ttatrm} (``unlike in Sudoku
  tasks''); Ren \& Liu \citep{renliu2026guessing} (HRM ACT halting as a failure filter; spurious fixed points). Adaptive computation:
  \citet{graves2016act}, \citet{banino2021pondernet}.
\item \textbf{The maze failure is a scoring artefact}: exact match to one of many shortest paths (our re-scoring, \S\ref{r:maze});
  EqR/ERM build Maze-Unique and select at 97.3\% vs a 99.3\% oracle (ERM 2607.10128\,$^\dagger$).
\item \textbf{Residual-based collapse detection for DEQs is refuted by our X6} (\S\ref{r:transfer}): Broyden and Anderson converge as well or
  better on broken MDEQ and DEQ-Transformer models (the collapsed w4t DEQ-Transformer's residual is 500$\times$ below fp32's; per-image AUROC
  0.42--0.67), so a converged solver does not mean a working model; the equilibrium is displaced, and the cosine to the fp32 equilibrium tracks it.
  Any claim that solver non-convergence flags a broken DEQ (including Q-DEQ-style residual checks) does not hold for weight perturbations.
\item \textbf{Residuals fail for documented reasons}: converged-but-wrong fixed points (Ren \& Liu; FRMs 2606.29150), oscillation
  (FPRM 2606.18206), limit cycles \citep{mazeextrap2024}; a small residual can mean ``did nothing'' (2607.11116\,$^\dagger$); our X6: DEQ
  root-finders keep converging after the model is broken.
\item \textbf{Hand-coded checkers exist} for both tasks (Ren \& Liu's Sudoku conflict energy; ERM's maze rule penalty); the head's
  value is for tasks without one.
\item \textbf{What is open (ours)}: persistence of the head's discrimination and of its native threshold under compression, and
  how it fails at and past the edge.
\end{itemize}

\section{L7. Label-free evaluation of compressed models; teacher forcing vs generation}
\label{lit:eval}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Output-level agreement}: flips and KL \citep{dutta2024accuracy} (``Accuracy is Not All You Need'', NeurIPS 2024);
  Red Hat's half-million evaluations compare outputs by text similarity (ROUGE, BERTScore, STS), not flips \citep{kurtic2024bf16};
  loyalty (Xu et al.\ 2021); per-sample McNemar (Kübler et al., ICLR 2026). None uses an internal iterated state, and none states a
  threshold with its unit.
\item \textbf{Filter, not ranker}: output KL predicts quality across a quantized cohort ($\rho = -0.72$, $-0.86$) and not among
  near-baseline quants ($\rho\approx0$); ``fidelity metrics should filter damaged candidates, not rank near-baseline ones''
  \citep{kldquality2026}. Our X8 reproduces this for iterated latent state (\S\ref{r:fid}).
\item \textbf{The unit}: exact match $\approx p^L$ for independent per-token errors \citep{schaeffer2023mirage}; errors concentrate
  on a few key tokens (2505.24187). \redtext{Ours: the product model fails on every TRM/HRM task (predicts $<$1\% exact where 29--91\% is
  observed; wrong answers are wholesale, median 26--34 wrong cells); the DT-maze length dependence fits an onset-hazard model with $h$
  1/40 of the per-cell error. Cite Schaeffer et al.\ for the unit argument only, not as our mechanism.}
\item \textbf{Teacher forcing hides generation collapse (non-looped LLMs)}: ``When Perplexity Lies'' (2603.26556, TMLR: within 0.2 pp
  under log-likelihood, 20.8 pp behind under generation); ``The Benchmark Illusion'' (2606.17609); Deiseroth et al.\ Prop.~3.2; OPD
  (2609.26708\,$^\dagger$). For looped LMs the gap is open: LoopQ evaluates by likelihood and perplexity only.
\item \textbf{What is open (ours)}: a single latent-fidelity threshold across looped-LM models where teacher-forced loss has none
  (\S\ref{r:lm}).
\end{itemize}

\section{L8. Test-time compute on edge devices; toolchains}
\label{lit:edge}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item Edge test-time scaling so far means scheduling LLM token generation: FastTTS \citep{fasttts2025} (memory-bound framing),
  EdgeReasoning \citep{edgereasoning2025} (latency-budget framing: ``functions mapping latency budgets to maximum decodable
  tokens''), mobile NPU TTS (2509.23324). Weight-tied reasoners hold memory constant as they iterate; looped LMs reach that regime only
  with a shared cache \citep{melt2026}; RD-VLA (2602.07845) constant memory with recurrent depth.
\item Toolchains (lit 06): no edge NPU runs a data-dependent loop inside the accelerator graph in production (ORT QNN EP: ``Loops
  and Ifs are not supported''), so the deployable pattern is a host loop around one static step graph; grouped INT4 is the exception on
  edge NPUs (LPBQ on Hexagon v69+; Core ML per-block; Arm Ethos-U per-channel only; TFLM INT4 per-tensor only; Edge TPU, STM32N6 INT8
  only). MLPerf Tiny has no attention or iterative workload; no paper measures a TRM/HRM-style reasoner on a device (27 + 17 arXiv hits).
\item \textbf{What is open}: device correctness of 8-bit-activation graphs of recursive reasoners; energy per solved instance.
\end{itemize}

\section{L9. Priors for the methods program}
\label{lit:methods}
M1: iterative refinement in three precisions \citep{carson2018threeprecisions}; LQER and ZeroQuant-V2 LoRC (low-rank quantization-error
correction); Elves (Su et al., VLDB 2024; lossless residual storage); Matryoshka quantization (nested bit-widths). M2: PTRM best-of-$K$
\citep{sghaier2026ptrm}; path independence \citep{anil2022pathindependence}. M3: HAWQ / HAWQ-V2 (Hessian allocation); CompreSSM
(Chahine et al., ICLR 2026; balanced truncation); Ingolfsson's MXInt4 recipe. M4: ML-EXray (MLSys 2022; per-layer reference
comparison), DriftBench (MLSys 2026; held-out categories), TFLite quantization debugger. M5: ACT \citep{graves2016act}, PonderNet
\citep{banino2021pondernet}, TRM's own note that ACT is a training device. M6: Quant-Noise, noise-aware training, Jacobian regularisation of
DEQs (Bai et al.\ 2021), LSQ (Esser et al.).

\section{L10. Terminology collisions}
\label{lit:terms}
\begin{center}\footnotesize
\begin{tabular}{@{}lp{0.5\textwidth}p{0.3\textwidth}@{}}
\toprule
Our term & Collides with & Suggestion \\
\midrule
basin & loss-landscape basin (2606.09012); basins of attraction over initial latent states (PTRM, EqR, CMM; 2609.04963\,$^\dagger$) & ``tolerance basin'' in perturbation space, defined once \\
phase boundary & dynamical ``phases'' selected by initialisation (2608.26556\,$^\dagger$) & ``collapse threshold'' / ``edge'' \\
fidelity & LASER's cosine reconstruction fidelity (2604.17224) & ``trajectory fidelity'' \\
compressed & ``compressed loop'' = small recurrent state (2605.30757) & ``quantized'' where it matters \\
halting head & Ouro's compute gate (loss improvement) vs TRM/HRM's head (BCE on exact correctness) & ``correctness head'' for C \\
\bottomrule
\end{tabular}
\end{center}
\open{choose terms before any drafting}

\section{L11. Our own earlier results (June 2026)}
\label{lit:preprint}
\textbf{Not a citation.} Our June preprint (arXiv 2606.26488) is not cited anywhere; its arXiv version will be overwritten with this paper
(Steven, Sep 25). Its results are our own earlier measurements and are reused as such: cell accuracy holds while exact accuracy collapses under
naive INT4, pruning, distillation and linear attention; the collapse hits MLP-mixing recursion and not attention; per-channel calibrated INT4 recovers
(our measurement: 71.9, fp32 73.8, on the Sep 13 harness); carry-trajectory fidelity; INT8 at one cycle matches full depth at 6$\times$ fewer FLOPs.
Withdrawn from our earlier framing: ``quantization errors compound across recursive reasoning cycles'' and ``QAT cannot repair it''.
\redtext{The current title of this document is the preprint's title (open, \S\ref{d:open}).}

\section{L12. Concurrent work (posted after our June preprint): rebuttal and awareness only}
\label{lit:concurrent}
\begin{redpar}
\noindent Not cited in the main text under the cutoff (D2). Each entry: arXiv id, first-posted date where known, and what it bears on.
\begin{itemize}[leftmargin=*,itemsep=0pt,topsep=2pt]
\item 2609.26487, Krishna et al., ``When Recursive Models Finish Computing'' (Sep 22): MLP TRM keeps a perturbation along the most
  expanding direction at 1.91$\times$ after 16 steps, attention shrinks it to 0.10$\times$; $\sigma_{\max}>1$ everywhere, direction of
  travel contracts; TRM 16$\to$512 steps; Maze-Hard: 191 of 212 exact failures are valid paths, 75 shortest. (A, B, C mechanism.)
\item 2608.18222, Viakhirev et al., ``Think Shallow, Solve Deep'' (Aug 18): Jacobian/Lyapunov toolkit; settle / marginal / drift regimes;
  a settled model's answer cannot change with extra depth; ``never per-cell''. (A, D.)
\item 2607.10681, Buehlmaier: stability budget is the spectral margin $1-\rho$.
\item 2609.04963 (fractal basins; weights as bifurcation parameter); 2608.26556 (phases by initialisation); 2608.23725 (critical DEQs).
\item 2607.15456, O'Neill and Reid, LLA (Jul 16): cross-loop KV compression; ``the error then compounds autoregressively \ldots\ even when
  teacher-prefix KL is low''; KV cache of a $T{=}4$, $D{=}24$ looped model = a 96-layer decoder. (F, I.)
\item 2609.04490: 4-bit recurrent-state storage freezes updates (99.6\% below write threshold). Not observed for TRM (\S\ref{r:devices}).
\item 2609.11716, ``Why does PTQ work?'': trained layers counteract inherited error.
\item 2609.26708, ``Train Where the Quantized Model Goes'' (OPD): quantization-amplified exposure bias; likelihood QA keeps 86\% of BF16
  while MATH-500 keeps 27\%. (F.)
\item 2607.28196, Kennedy \& Kennedy, ``Fidelity Is Not Safety'': a data-free CKA/cosine guard passes low-rank builds that then misbehave.
  (C, D scope.)
\item 2609.07664, Qamar et al., ``Accuracy is Not Enough'' (JSD/TVD for quantized LLMs) --- not Dutta et al.
\item 2607.20519, halting-gate diagnosis (gate vs trajectory read-out); 2609.11801, Looped Flows (best-Q); 2607.10128, ERM (maze q-head
  selects at 97.3\% on Maze-Unique); 2609.05988, DART (never-arrive vs arrive-then-leave in FP); 2608.24136, RoFB (maze validity).
\item 2609.01924 (Jacobian lens on Ouro/Huginn), 2609.19934 (Huginn noise ratio 0.892 per iteration), 2609.24196 (LoopCD), 2608.09444
  (continuous depth batching: Ouro fragile, Huginn robust under KV compression), 2607.18553.
\item 2607.08116, MORES (budgets recurrent steps of a latent reasoner; latent-state pruning costs 20 GSM8K points at 32 steps).
\item 2609.24042, Q-DEQ (edge DEQ, W8A8); 2609.06922 (Before the Flip); 2607.21063 (QuantiBias); 2607.13124 (ShortOPD); 2608.22761 (DRY).
\end{itemize}
\end{redpar}

\section{L13. Corrections carried over from the notes}
\label{lit:corrections}
2606.00206 is Lotfi, Kirichenko, Li and Liu (Meta). Dutta et al.\ 2024 is ``Accuracy is Not All You Need''; ``Accuracy is Not Enough'' is
Qamar et al.\ (post-June). Red Hat's study compares text similarity, not flips. The Adaptive Depth paper, Before the Flip, QuantiBias and
LLA are post-June. Ingolfsson et al.'s frame is not simply ``accumulation versus our basin'': they already use contraction, drift and basin
language; the disagreement is whether depth matters inside the basin, whether bias is necessary to leave it, and whether Maze/attention
robustness comes from recursion depth or from the mixer.

\section{L14. Literature angles (Sep 25 scan; reports/edgetrm\_lit/08\_angles\_sep25.md)}
\label{lit:angles}
Scope: the five angles of PLAN.md \S8 zoom-out 1 plus M3, checked against six literature questions by six research agents (arXiv, OpenReview,
Semantic Scholar, Google Scholar); load-bearing quotes and numbers checked against the source text. \textbf{Framing rule (Steven, Sep 25)}: work in
another field, model class, precision regime (full precision only), token rather than latent space, or for another purpose is inspiration or
corroboration, not prior art; ``prior art'' is reserved for the same method, setting and claim. Under that rule nothing found is prior art for any angle.
Ranking is by strength of our evidence $\times$ reach of the lens.

\paragraph{Reputation tiers (Steven, Sep 25).} \textbf{T1} peer-reviewed at a strong venue (ICLR, NeurIPS, ICML, CVPR/ICCV/ECCV, ACL family, MLSys,
OSDI/SOSP, ASPLOS, ICSE/FSE/ASE/ISSTA, IEEE S\&P, AAAI; journals such as SIAM, Acta Numerica, IEEE L-CSS); \textbf{T2} arXiv from a strong group with
code or released models and consistent numbers; \textbf{T3} other arXiv, workshops; \textbf{T4} suspicious or incomplete, ignored.
A paper's suggestion is never binding; our data decides.

\begin{table}[H]
\caption{\textbf{Angles ranked by the Sep 25 scan} (evidence $\times$ reach of the lens; tiers in parentheses). This is the scout's ranking of angles;
the three candidate framings of Part~\ref{part:framings} remain unranked.}
\label{tab:angles}
\centering\scriptsize
\begin{tabular}{@{}p{0.02\textwidth}p{0.16\textwidth}p{0.2\textwidth}p{0.3\textwidth}p{0.22\textwidth}@{}}
\toprule
\# & Angle & Our evidence & What the lens explains that others did not & Key sources (tier) \\
\midrule
1 & One quantity decides everything (fidelity / $\delta_T$) & Strongest: X1 regimes, X2 width law, X8 in-basin defer risk $\le$0.7\%, cross-family collapse detector (0 of 478 missed), M4 & Neighbouring work predicts failure per input (Chang) or per bit-width (Lotfi); none has a model-level, label-free dynamical quantity. Explains Lotfi's unexplained 3-bit split (GPTQ 19$\to$39 vs AWQ 19$\to$139 overthinking errors). Supplies the ``expected quantization loss or bug?'' oracle that Guan (ICSE'23) and Chen (ICSE'21) name as missing. & Chang EMNLP'25 (T1); Guan ICSE'23 (T1); Chen ICSE'21 (T1); Lotfi (T2) \\
2 & Compression manufactures overthinking; the model's own verifier undoes it & Medium-high on TRM/HRM: exit gain $\sim$0 inside, large past the edge (29.8$\to$52.9; 51.2$\to$58.4; HRM Maze 40.1$\to$55.4); DEQ negative; looped LMs pending & Joins early-exit CNNs (Kaya: 50\% destructive overthinking in fp), shifted inputs (Mehra: oracle exit $\ge$10 points vs practical $\sim$1), quantized CoT LLMs (Lotfi: 26\%$\to$52\%) and fp looped LMs; ours: where (past the basin edge), why (the trajectory visits the answer then leaves) and a trained-verifier fix frozen from fp32 & Kaya ICML'19 (T1); PABEE NeurIPS'20 (T1); Anil NeurIPS'22 (T1); Mehra (T2); Lotfi (T2); Ouro (T2) \\
3 & The declared format is not the computed function (MLSys) & Strong: 10 device chains, change runs both ways (MLP 0 host / 61 S24; Maze 42 / 0), reference-QDQ ablation, INT4 cast, TFLM REDUCE\_SUM & fp drift across platforms rarely flips labels (Schl\"ogl), fuzzers discard large divergence as false alarms (NNSmith), practitioners lack an oracle; ours: both directions, a model-level predictor of which models flip, recursion as a conformance amplifier, a two-step device probe & Schl\"ogl NeurIPS'23 (T1); NNSmith ASPLOS'23 (T1); Shen FSE'21, Guan ICSE'23, Chen ICSE'21, Jajal ISSTA'24 (T1); MLPerf Mobile (T1) \\
4 & Worse alone, better together / precision for depth & Now robust on one family (TRM attention held-out +4.9 vs best single format, +3.8 vs fp32; Bonferroni; ensemble control); MLP via nested map only; HRM, Ouro-1.4B negative & Higham \& Mary \S5: cheap-early precise-late can at most match working precision for a globally convergent iteration with one solution; our gain lives where that fails (many attractors: the cheap phase selects the basin). Nam \& Lee: rounding diversity beats FP32 only in one-pass averaging; ours composes it sequentially with a label-free selector & Higham \& Mary, Acta Numerica (T1); Nam \& Lee NeurIPS'24 (T1); Dutta NeurIPS'24 (T1); PTRM (T2) \\
5 & M3: calibrate at the fixed point & Interim: per-tensor INT4 Sudoku-MLP 5.9$\to$62.5; INT3 attention 0$\to$60.5; HRM 0$\to$45.9 & Ingolfsson say clipping is ruled out without a sweep; no Jacobian- or fixed-point-weighted PTQ objective found; reconstruction PTQ calibrates first-pass layer outputs, diffusion PTQ a finite trajectory; ours an equilibrium with one step-invariant quantizer & AdaRound, BRECQ, QDrop, GPTQ, OmniQuant (T1); Q-Diffusion (T1); Ingolfsson (T2) \\
6 & Scope: fixed-point iterations have a basin; deterministic non-contracting samplers accumulate & One diffusion model (DDPM vs DDIM) plus five fixed-point families & Explains the split across fields on which end deserves the precision: iterations that forget their start want precision late; iterations that amplify early error want it early & Higham \& Mary (T1); PTQD NeurIPS'23 (T1); CPT ICLR'21 (T1); T-Stitch, PMPD (T2) \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Required checks from the scan} (each rests on T1/T2 work or our own data): (1) M1/M2 against fp32 diversity at matched weight traffic
(fp32 latent noise, weight noise at matched $\varphi$, trained seeds), with variance over rounding seeds; M1's ensemble control has now landed
(+3.2 held out, \S\ref{m:m1}). (2) M5 against the fp32 visit-then-lose baseline (Kaya: 50\% destructive overthinking in fp; Lotfi 26\% in BF16): the claim
is the increase past the edge and its dependence on fidelity. (3) M3 against our own earlier per-channel INT4 measurement (71.9, fp32 73.8, Sep 13 harness) rerun on one harness.
\textbf{Optional controls} (T3-based): the S24 encoding dump (done: the RMSNorm is fused, scales are honoured elsewhere, \S\ref{r:devices}); HRM Sudoku
wording (done: failed puzzles keep moving, median residual 0.33); Sudoku symmetry TTA as a diversity baseline. BitCal-TTS (2605.05561) is T4 and ignored.
\src{reports/edgetrm_lit/08_angles_sep25.md}


==> sections/methods.tex <==
% Setup, ICLR rewrite (Sep 24). Definitions follow the harness (EdgeTRM/breadth_sweep.py: parse_quant,
% quantize_weights_, _ActNoise, fidelity). Numbers here are defining constants only (house rule H6).
\section{Setup (shared by every framing)}
\label{sec:setup}
\label{sec:methods}

\paragraph{Models and tasks.}
We study four families of models that compute by repeating one weight-tied block.
TRM \citep{jolicoeur2025trm} refines a latent carry with a small block in two nested loops; we use
TRM checkpoints for Sudoku-Extreme with an MLP token mixer and for Sudoku-Extreme, Maze-Hard and
ARC-AGI-1 with an attention mixer, and thirteen Sudoku models we trained with both mixers at
several widths and seeds (Appendix~\ref{app:impl}). HRM \citep{wang2025hrm} nests a slow and a
fast recurrent module; we use HRM checkpoints for Sudoku, Maze and ARC. Deep-thinking networks
\citep{schwarzschild2021deepthinking,bansal2022overthinking} iterate a convolutional block and
extrapolate to instances larger than those they were trained on; we use the released maze,
prefix-sum and chess models. Looped language models reuse their core block for a chosen number of
recurrences; we use Huginn \citep{geiping2025recurrentdepth} and Ouro at two sizes
\citep{zhu2025ouro} on GSM8K.

\paragraph{The depth dial.}
Every family has a test-time depth dial that leaves the weights unchanged: the number of
supervision steps $n_{\text{sup}}$ for TRM and HRM, each of which runs $H$ outer cycles of $L$ inner
updates; the number of iterations for deep-thinking networks; and the number of recurrences for
looped language models. We report the cost of compression at each setting of the dial.

\paragraph{Perturbations.}
Post-training weight quantization is written w$\langle$bits$\rangle\langle$granularity$\rangle$, with
bit-widths from 8 down to 2 and four granularities of the scales: one per tensor (t, symmetric), one
per output channel (c, symmetric), one per output channel with a min--max range (a, asymmetric), and
one per group of 32 or 128 weights (g32, g128). The suffix +a8 adds static per-tensor INT8
quantization at the input of every linear layer. Two noise dials keep the size of the perturbation
and remove the rounding. Weight noise adds to every weight a Gaussian draw whose standard deviation
is $\sigma$ times the standard deviation of that weight's tensor; activation noise adds the same at
the input of every linear layer, drawn afresh at every pass. The noise sweeps of TRM, HRM and the
deep-thinking mazes are repeated over three draws.

\paragraph{Metrics.}
An answer is exactly correct when every output cell is right; cell accuracy is the fraction of
correct cells. Maze answers are also scored as a valid simple path from start to goal, and as a valid path
of the shortest length (BFS oracle; X1): every Maze-Hard test maze has more than one shortest path (minimum 96,
median 3.8 million), so exact match to the reference path under-counts correct answers. Fidelity $\varphi$
compares the final high-level latent state $z_H$ of the compressed model with that of the
full-precision model at the same depth, on the same input:
\begin{equation}
  \varphi \;=\; \frac{1}{N}\sum_{n=1}^{N}
  \frac{\operatorname{vec}(z_H^{q,(n)}) \cdot \operatorname{vec}(z_H^{\text{fp},(n)})}
       {\lVert \operatorname{vec}(z_H^{q,(n)})\rVert_2\,\lVert \operatorname{vec}(z_H^{\text{fp},(n)})\rVert_2},
  \label{eq:fidelity}
\end{equation}
the cosine between the two flattened states, averaged over the $N$ inputs. It needs no labels and no
decoding. The halting head of TRM and HRM is trained to predict whether the current answer is
correct; we report its AUROC for detecting wrong answers. For the language models we report the
GSM8K accuracy of greedy generations and the teacher-forced loss on the reference solution.

\paragraph{Quantities used across the bank.}
Accuracy \emph{retained} is the compressed cell's accuracy divided by fp32's on the same inputs, $H$, depth and
platform. $\sigma_{1/2}$ is the noise level at which the median of three draws falls below half of fp32 accuracy.
The one-step map perturbation $\delta_T = \lVert \tilde F(s_T) - F(s_T)\rVert / \lVert s_T\rVert$ applies one step of
the perturbed map $\tilde F$ and of the fp32 map $F$ at fp32's end state $s_T$ (X2); the sensitivity is
$S = \delta_T/\sigma$ at the smallest $\sigma$. $\rho$ is the spectral radius of one recursion step's Jacobian at
the end state (JVP power iteration). For test-time scaling (X1) the ceiling (cap) is the fitted asymptote
$A$ of $\text{acc}(T)$ and the rate (tax) is the fitted time constant $\tau$ or the model-free $T_{90}$
(iterations to 90\% of the curve's own maximum), with paired bootstrap intervals over instances.
\redtext{Terminology collisions to resolve before writing (lit 03 \S4): ``basin'' (loss-landscape basins,
arXiv 2606.09012; basins of attraction over initial latent states, PTRM, EqR), ``phase'' (2608.26556, 2609.04963),
``fidelity'' (LASER, 2604.17224). Define ours at first use or rename.}


==> sections/methods_program.tex <==
% Methods program M1-M6 (Steven, Sep 24 23:15 UTC; reports/edgetrm_exp/METHODS_BRIEF.md). Every method is
% pursued on its merits; nothing is decided about which story either paper tells. All red until results land;
% each method's status file is reports/edgetrm_exp/M<k>.md.
\begin{redpar}
\noindent\textbf{Status (Sep 25 01:30 UTC): interim written records for M1, M2 and M5 (below, all interim); M3 and M4 validated their
harnesses; M6 has the three QAT endpoints and no new-arm endpoint.} Steven (Sep 24 23:15 UTC): ``chase all of M1--M6 in
parallel \ldots\ when they break down, don't cave in easily, iterate and try something else \ldots\ Leverage related work
massively.'' Each method below states the evidence that motivates it (with numbers from the results bank), the design, the
baselines, and its status. Energy numbers stay red until the AWS credits arrive ($\sim$two weeks). Compute: Babel general
(M1 three L40S, M2 two, M3 two, M5 one), p4d cards 3--5 for M6.
\end{redpar}

\section{M1. Iterate cheap, finish exact (precision-switching inference)}
\label{m:m1}
\textbf{Evidence.} Cross-seeding (X2, \S\ref{r:mech}): the fp32 map run from a broken compressed model's end state recovers
95--99\% of fp32-solved TRM Sudoku puzzles, even for the MLP model at $\sigma{=}0.3$ with 1\% accuracy; the compressed trajectory
stays in fp32's basin while its read-out is wrong. Where the basin switches (HRM 7--18\% at $\sigma\le1.0$; DT mazes at the
collapse; TRM Maze $\le$14\%) polishing should fail. \textbf{Design.} Run most iterations with compressed weights and the last $k$
``polish'' steps with more precise weights; measure accuracy against $k$, memory and compute. Variants: fp32 / bf16 polish; INT8
polish; the quantized weights plus a low-rank correction of the quantization error only in the polish steps (LQER; ZeroQuant-V2
LoRC); the losslessly compressed residual $W - Q(W)$ stored beside $Q(W)$ (Elves, Su et al., VLDB 2024) and reconstructed only for
the polish; nested bit-widths (Matryoshka quantization: INT4 = top bits of INT8). Inspiration: iterative refinement in three
precisions \citep{carson2018threeprecisions}. \textbf{Where it should fail, and what next}: basin-switching models (HRM, DT mazes):
diagnose, then try a different polish (longer, from an earlier state, or a checker-guided restart).
\textbf{First finding (residual sizes, p4d CPU, Sudoku-MLP, partial)}: trained fp32 weights have nearly full mantissa entropy (the best
lossless coder stores $W$ in 27.0 bits/weight); the exact residual beside $Q(W)$ costs 25--27 bits/weight for every 3--4-bit quantizer
(22--23 beside INT8, 18 beside bf16), so an exactly reconstructed fp32 polish costs about as much memory as fp32 outright (4 + 26 = 30
vs 32 bits). Lossless reconstruction is the wrong target; the question is the lowest polish precision that works (INT8, nested INT8,
low-rank corrections). \src{p4d:m1/sizes.json (polish_sizes.py); M1.md}

\begin{redpar}
\noindent\textbf{Interim results (M1.md, Sep 25 00:10--01:15; Babel L40S, $n{=}1000$ Sudoku, 500 mazes, 256 DT).}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Sudoku-MLP}: fp32 from scratch with $k$ steps 28.4 (1), 49.8 (2), 61.0 (4), 67.6 (8), 70.8 (16). Compressed steps are worth
  0.1--3.0 fp32 steps on the collapsed cells (w4t, w3c, noise $\ge$0.15) and 2.0--7.5 near the edge (w3g32, w3a); X2's 95--99\% recovery
  holds but $z_0$ is inside fp32's basin too, so the recovery is mostly the fp32 map doing its normal work. INT8 / bf16 polish = fp32 polish
  within 1.5 points; polishing only the head gives nothing; a full step is needed. Low-rank correction works better in every step (w4t
  rank 32: 53.7) than as a polish, and never reaches fp32. At matched weight-bit traffic, INT8 alone at fewer steps beats every per-tensor
  hybrid; every non-per-tensor 4-bit format (w4a 69.8, w4g32 69.1, MXInt4 68.8, w4g128 68.2, w4c 68.1) is already inside the MLP basin.
  Nested cells (cheap steps read the top bits of stored INT8 codes): n8a4 + 4 INT8 steps 71.6--71.8 vs INT8 per tensor at the same traffic
  68.8 (+2.8 to +3.0).
\item \textbf{Sudoku-attn}: the compressed steps are worth 6--17 fp32 steps inside the basin with a tax (w4t, w3c, w3a, nested n8t4) and 4--8
  polish steps close it (w3c 59.7 $\to$ 66.0 / 68.0); past the edge (w3t, w2g32, noise $\ge$1.0) the head start is negative (w3t c8+f8 23.4 vs
  f8 61.5): a basin switch. Against per-tensor formats at equal traffic and memory, n8t4 + 4 / 8 INT8 steps beats INT8 per tensor by +1.4 /
  +2.1 (1--2 standard errors; paired tests pending); a grouped 3.5-bit model beats every hybrid.
\item \textbf{HRM}: past the edge the end polish fails (w3t stays at 0.0--0.2 with every hybrid; the w3t map leaves fp32's basin within two
  steps). What rescues HRM is the H-level module precise in every step (w2a 11.6 $\to$ 37.0; noise 1.5 0.0 $\to$ 31.1; with H precise 8 + 8 full
  polish w3t 39.9), not a final polish: static per-module precision (M3's territory), not switching over time.
\item \textbf{Mazes}: fp32 needs 1--2 steps; compressed steps buy nothing. \textbf{DT maze 13}: compressed iterations are worth $\sim$40 fp32
  iterations at noise 0.3 (one polish step 90.6 vs 0.0 from scratch), +4 to +8 at noise 0.5 (a basin switch); at matched traffic INT8 alone at
  $\sim$50 iterations also reaches 100.
\end{itemize}
\end{redpar}

\paragraph{M1 read-out (Sep 25 03:00 UTC; M1.md, \texttt{EdgeTRM/results/breadth/m1\_readout.md}; REWRITE\_NOTES 50).}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{The premise needs a control}: fp32 started from $z_0$ is also in the basin, so X2's 95--99\% recovery is mostly the fp32 map's own
  work. Compressed steps are worth only 0.1--3 fp32 steps on collapsed Sudoku-MLP cells, 6--18 on attention inside its basin, 20--47 on DT mazes.
\item \textbf{End-polish mostly equals a single good format at matched cost}: INT8 / bf16 polish = fp32 polish; low-rank correction works better
  in every step than as a polish (MLP 3-bit asymmetric + rank 32: 71.0 at 4.35 bits vs fp32 70.8); the lossless residual costs 22--27 bits/weight
  (useless); nested INT4-in-INT8 works; at matched memory and compute a single good format (grouped INT4, INT8) matches or beats most hybrids.
\item \textbf{It fails where the basin switches}: HRM w3t, attention past its edge, DT at noise 0.5. HRM is rescued only by keeping its H-module
  precise in every step (static per-module precision, M3's territory).
\item \textbf{Ouro-1.4B w4c}: bf16 in the last two loops 63.0, last three 71.5, but INT8 in all loops 76.0 at half the bf16 traffic beats every
  switched schedule; w4t is unrecoverable. Switching activation precision on the AI Hub graphs gives nothing.
\end{itemize}

\paragraph{M1 positive regime: precision for depth, robust on TRM attention (one family).} (M1.md ``Round 2'' and ``Robustness''; EdgeTRM 6a986b5,
00c33d6, cf2f631, c2825d0; REWRITE\_NOTES 54, 68.)
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Mechanism}: hybrid = cheap map for $T-k$ steps + INT8 for $k$; INT8 steps keep 99.7--100\% of what the cheap map solved. The gain needs a
  cheap map that is a \emph{different} solver of similar strength (attention w3c / n8c3 solve $\sim$8\% of the puzzles fp32 misses; two-run oracle
  80--83 vs fp32 74); mild maps (w4c) are near-subsets of fp32 and give nothing. Switch rates are equal for w3c and matched noise (29.7\% vs 30.1\%) but
  w3c's switches are right 29\% / wrong 15.5\% vs noise 8.0\% / 9.9\%. Attractors: on attention, 92\% of puzzles reach $\ge$5 answers and 15\% of fp32
  failures are solvable from another start; the MLP model is near path-independent; HRM's correct attractor is almost never reachable (fits Higham \&
  Mary: cheap-early precise-late can at most match working precision for a globally convergent iteration). HRM wording corrected: failed HRM Sudoku
  puzzles keep moving (median residual 0.33).
\item \textbf{Frontier, released attention Sudoku, $n{=}1000$ (dev)}: $T{=}64$ 76.3 (+2.1 vs the best single format, $p{=}0.014$; fp32 needs 331 steps);
  $T{=}128$ 77.9--79.2 ($p$ $6\times10^{-6}$ / 0.003; fp32 never matches within 512); $T{=}256$ w3c 224 + INT8 32 = \textbf{82.5} vs w3c alone 77.7 (+4.8,
  $p{=}3.5\times10^{-11}$); fp32 at 512 steps 77.1, at $\le$1/17 of fp32-512's weight traffic.
\item \textbf{Held out (frozen selection, puzzles 1000--1999)}: $T{=}256$ \textbf{91.9} vs the frozen single-format comparator 87.0 (\textbf{+4.9},
  $p{=}3.2\times10^{-13}$) and vs fp32 at its best depth $\le 2T$ 88.1 (\textbf{+3.8}, $p{=}2.5\times10^{-5}$); $T{=}128$ +3.0 ($p{=}0.003$) / +4.1; $T{=}64$
  +3.1 ($p{=}0.008$) / +2.8.
\item \textbf{Multiplicity}: 535 hybrid schedules on dev for this checkpoint (5,666 overall); Bonferroni $p$ $1.9\times10^{-8}$ / $2.0\times10^{-7}$.
\item \textbf{Ensemble control} (fp32 + matched-strength noisy fp32, same composition): dev 77.1 vs 82.5 (+5.4, $p{=}1.4\times10^{-7}$), held-out 88.7 vs
  91.9 (+3.2, $p{=}2.1\times10^{-4}$); w3c beats every noise draw by 3.2--7.8, and a shuffled-error map (w3c's own errors permuted) also loses. \textbf{The
  gain is specific to the structure of 3-bit rounding}, not to perturbation size or to having a second solver.
\item \textbf{A pre-run rule} (help iff complementarity $\ge$5 points and cheap/fp32 accuracy $\ge$0.95) is right on 95\% of 21 out-of-sample rows.
\end{itemize}
\begin{redpar}
\noindent\textbf{Breadth is not there yet.} Family-level success so far: TRM attention only. Trained attention seeds at $T{=}64$ hold on 2 of 3 vs fp32 and
1 of 3 vs the best low-bit format (s1's 3-bit maps are 6 points weaker); MLP only via the nested map (n8a4 78.6 at $T{=}128$ vs 77.5, $p{=}0.003$); HRM
none; Ouro-1.4B \textbf{negative} (INT8 for 2 loops, 77.0, at the traffic of w4c for 4 loops beats every switch); DT maze 33 is ceiling repair (+3.9 to +4.3 at
$T$ 150 / 200, n.s.\ at 300; the earlier ``+4.7, $p{=}5\times10^{-4}$'' is +1.6, $p{=}0.12$ once n8a4 is included). \running{MDEQ dense reruns; Ouro-2.6B;
$T{=}256$ seeds, $T{=}512$} Device cost: at equal accuracy the hybrid is 2.1$\times$ ($T{=}32$) to 5.7$\times$ ($T{=}64$) faster than FP16 on the S24
(conservative bound with verified FP16/INT8 kernels 1.8--4.9$\times$); an estimate, since 3-bit steps are costed at the INT4 time and INT4 device graphs
are currently wrong on the HTP.
\end{redpar}
\src{EdgeTRM/results/breadth/m1_readout.md; analyze_m1.py; M1.md}

\begin{redpar}
\src{EdgeTRM/results/breadth/babel/m1/p_*.json; analyze_m1.py; M1.md}
\end{redpar}
\running{DT maze real quantizers past the edge (E6); paired McNemar tests (A8, job 10556792)}

\section{M2. Best-of-$K$ latent sampling with the halting head as verifier}
\label{m:m2}
\textbf{Evidence.} PTRM \citep{sghaier2026ptrm} injects Gaussian state noise before every supervision step and returns the rollout
with the highest $Q$ logit, in full precision (Sudoku-MLP $K{=}100$, $D{=}64$, $\sigma{=}0.3$; Maze-attn $\sigma{=}1.0$). The halting
head survives compression inside the basin (\S\ref{r:halt}); X8 has a PTRM harness (\texttt{ptrm\_sweep.py}).
\textbf{Design.} Apply best-of-$K$ to compressed models on and past the edge; compare sequential (more steps) vs parallel ($K$
samples) at matched compute; combine with M1 (sample cheap, verify, polish the winner). Baselines: best-of-$K$ in fp32 (PTRM),
pass@$K$, mode@$K$. \textbf{Existing written records (X8's PTRM files, Babel L40S, $n{=}1000$, $D{=}16$, $\sigma{=}0.3$,
$K{=}16$)}: Sudoku-MLP fp32 deterministic 70.5 $\to$ best-Q@16 80.5; w4c 68.1 $\to$ 78.5; w3g32 (edge) 51.5 $\to$ 66.0 (pass@16 66.7):
the head picks a correct rollout whenever one exists (best-Q within 0.7 points of pass@$K$). M2 smoke: Sudoku-attn fp32 single 66.3,
best-Q@16 76.2 (X8: 66.7 / 76.3). Prior art to reconcile: Ingolfsson et al.\ (\S5.3, A.4) find per-tensor Int4 \emph{activations} stay at
0.0\% for every $K\in\{1,4,16\}$. \src{Babel breadth_results/x8/ptrm_sudoku_mlp_ptrm{,_w4c,_w3g32}.json; M2.md}

\begin{redpar}
\noindent\textbf{Interim results (M2.md, Sep 25 00:40 and 01:20).}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item Latent noise does not push compressed models further out: single-rollout accuracy is flat in $\sigma$ 0.1--1.0 for fp32 and w3g32
  (Sudoku-MLP, $n{=}500$, $K{=}16$; fp32 best-Q 81.0--82.4; w3g32 65.0--66.4).
\item \textbf{Selection over steps as well as rollouts is the larger lever}: max-Q over every (rollout, step $\le$16) pair takes w3g32 to 69.0 /
  73.4 / 71.4 ($\sigma$ 0.1 / 0.5 / 1.0), above fp32's deterministic 70.8, and weight noise 0.15 to 61.8 (from 24.3). Even deterministically
  ($K{=}1$) the max-Q step gives w3g32 51.2 $\to$ 59.2 and noise 0.15 26.4 / 26.1 / 36.8 $\to$ 52.2 / 55.3 / 57.2: compressed trajectories on
  the narrow MLP basin's edge reach the answer and leave it, and the head flags the visit (not seen for w3a / w3c / w4t, attention or HRM).
\item In the basin (HRM / attn w4c, w4t; MLP noise 0.1) best-of-$K$ lifts compressed models by the same 10--12 points as fp32, best-Q = pass@$K$
  within 0.1: compression costs nothing under parallel scaling there. Head calibration breaks at w3g32 (ECE 0.37 vs 0.004) while its
  within-puzzle ranking holds (AUROC 0.96--0.97).
\item \textbf{M1 $\times$ M2}: fp32 polish of every rollout, then the fp32 head selects: MLP noise 0.2 (10.2 single) $\to$ 72.4 best-of-16,
  above fp32's deterministic 70.8; attention noise 1.0 (0.3) $\to$ 35.5; HRM noise 1.3 7.8 $\to$ 25.0. Selecting with the compressed head
  before polishing is much worse (58.8 / 15.4). Needs fp32 weights on the device (M1's memory trade).
\item Mazes ($n{=}250$, $K{=}16$, $\sigma$1.0): HRM fp32 valid 92.8 $\to$ 96.8 (= pass); HRM w2g32 valid 72.4 $\to$ 78.4 (pass 79.6); the head
  selects for validity, not shortness; TRM Maze gets almost no diversity from $\sigma$1.0.
\end{itemize}
\src{EdgeTRM/m2_analyze.py; Babel m2_results/cells; X8 det records for the deterministic check; M2.md}
\end{redpar}

\begin{table}[H]
\caption{\redtext{\textbf{M2 main grid, interim}} ($n{=}1000$, $\sigma$0.3, $D{=}16$; single draws unless noted): exact \%.
\src{m2_analyze.py main; M2.md}}
\label{tab:m2}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Model, spec & Single rollout & best-Q@4 / @16 / @32 & max-Q over (rollout, step) @16 / @32 & pass@32 & + 2 fp32 polish steps, best-Q (fp32 head) \\
\midrule
\inputrows{tables/bank/m2_main.tex}
\bottomrule
\end{tabular}}
\end{table}
\running{M2 remaining main-grid cells, matched-compute sequential $D{=}512$ vs hybrid, mazes}

\begin{redpar}
\noindent\textbf{Quantization as the sampler (M2.md, 05:25 and 07:30 UTC; REWRITE\_NOTES 76; controls pending, all red).} $K$ stochastic-rounding draws
of the fp32 master onto the grid, each run 16 steps, the answer picked by max $q_{\text{halt}}$. At matched compute ($S = 16K$), best-Q@16 against fp32 PTRM kicks
@16 ($\sigma$ 0.3): MLP w4c 86.9 vs 81.0; attention w3c 86.4 vs 76.0; HRM w3c 71.9 vs 59.1 (HRM fp32 kicks at $\sigma$ 1.0 reach 63.4 @16, 66.7 @32). SR beats
kicks on the same compressed model (RTN + kicks @16: 77.8 / 79.7 / 57.6). Draws are solvers of similar strength with different errors (M1's condition);
best-Q is within 0.1--1.1 of pass@$K$. HRM Maze w3g32 best-Q@16 valid 97.2 vs fp32 kicks 94.8; TRM Maze-attn: no diversity. Held-out rows 1000--1999
(nothing re-chosen): MLP w4c 93.7, HRM w3c 79.2, but these rows are easier (+6--9 on single draws), so fp32 references on the same rows are pending.
\textbf{Controls pending}: tuned fp32 kick $\sigma$, an fp32 weight-noise ensemble at matched $\varphi$, INT8-master draws (memory-honest), variance over SR
seeds. The only method so far that works on all three Sudoku families (candidate method headline, PLAN zoom-out 4).
\src{M2.md ``Quantization as the sampler''}
\end{redpar}

\section{M3. Sensitivity-guided mixed precision under hardware format constraints}
\label{m:m3}
\textbf{Evidence.} X2 located the MLP model's fragility in its token mixer (noise on it alone: 4.7--7.8 vs 71.5; per-tensor INT4
on it alone 5.9; on the channel MLP alone 44.9; heads alone 71.5). X3 located the host-simulated w8a8 collapse in RMSNorm (the whole norm at
16 bit restores 69/100 from 0/100; under reference QDQ semantics x$\ast$x + variance at 16 already gives 68, see \S\ref{r:devices}). \textbf{Design.} Allocate precision per weight group and activation group by a label-free
sensitivity ($\delta_T/\sigma$ per group, one forward pass on unlabeled inputs) so that formats the chips support (per-tensor INT4,
INT8 activations, TFLM per-tensor INT4) stay inside the basin. Baselines at matched bits: uniform; HAWQ-style Hessian-trace
allocation; random; Ingolfsson's granularity recipe (MXInt4-like grouped). Also try CompreSSM (Chahine et al., ICLR 2026;
balanced truncation / Hankel singular values) to rank state directions. Harnesses: \texttt{m3\_mixed.py} (per-tensor weight allocation;
scores $\delta_T$-based, KL, CompreSSM-style linearised gain, HAWQ-V2 with pseudo-labels, random) and \texttt{qdq\_torch.py} (executes
the AI Hub QDQ graph node by node in torch, vmapped; every one of 555 activation Q nodes settable to 8 or 16 bit). Executor validation
against X3's ORT results (100 puzzles): A0 66 vs 66, A8 0 vs 0, B2 66 vs 69 (float order; X3 measured $\pm$4 run to run). Smoke
($n{=}128$, not a result): every label-free score ranks the token mixer's \texttt{gate\_up\_proj} first. \textbf{Found by M3's validation}:
ORT's default extended optimizations (fused integer QLinear kernels) change mixed uint8/uint16 QDQ results (B2ab: 0/20 under ENABLE\_EXTENDED
and ALL, 11/20 under BASIC and DISABLE, 12/20 in the torch executor), so several X3 ablation rows are being rerun. \redtext{Interim (REWRITE\_NOTES 45,
red until M3 reports): a label-free $\delta_T$ clip takes per-tensor INT4 on Sudoku-MLP from 5.9 to 62.5, INT3 on attention from 0 to 60.5, HRM from 0
to 45.9; mixed INT3/INT8 on attention 67.1 at 3.97 bits; HRM mixing is a negative.} \running{M3 grids}
\src{EdgeTRM de59366; M3.md}

\section{M4. A pre-deployment release check validated on device-faithful runs}
\label{m:m4}
\textbf{Evidence.} Label-free host-side quantities already order cells: $\varphi_H$ (0.85--0.89 band, \S\ref{r:fid}), $\delta_T$
(Spearman $-0.88$), random-kick growth, halting-head agreement. \textbf{Design (M4.md, Sep 24 23:20 UTC).} Predict, from
host-side label-free quantities, whether a (model, toolchain configuration, backend) cell runs correctly, and validate on held-out
categories (DriftBench rule: leave one backend / model / configuration family out, never random splits); package as
\texttt{EdgeTRM/release\_check.py} (pass / warn / fail with evidence). Labels: retained $\ge$0.9 OK, 0.5--0.9 DEGRADED, $<$0.5
BROKEN. Backends: QNN QDQ host simulation (X3 graphs and ablation variants), TFLite interpreter (XNNPACK), TFLite reference
kernels / TFLM (the REDUCE\_SUM bug), the torch harness, AI Hub on-device chains when they exist. Checks: T0 per-layer reference
comparison (ML-EXray) and per-op LSB diffs across runtimes; T1 $\delta_T$, $S$ and one-step halting-sign agreement; T2 rollout
cell agreement, $\varphi_H$, halting agreement, kick growth. Question it must answer: would it have caught the w8a8 RMSNorm collapse
and the TFLM REDUCE\_SUM bug? Scripts: \texttt{release\_check.py} (CLI \texttt{prep / onnx / tflite / torch}),
\texttt{m4\_onnx\_sweep.py}, \texttt{m4\_tflite.py}, \texttt{m4\_torch\_sweep.py}, \texttt{m4\_labels.py}. \running{p4d: ONNX check on
36 Sudoku QDQ graphs and ablation variants (32 check puzzles, test 200--231); TFLite export with 7 AI Edge Quantizer variants and
interpreter/TFLM label chains (eval puzzles 0--99); Babel job 10555764: torch-path sweep with label runs; no result yet}
\redtext{\textbf{Early observations (M4.md, partial, not results)}: on AI Hub's Sudoku-MLP w8a8 QDQ graph the ONNX check gives $\delta_T$ 1.15
and final cell agreement 0.41 (FAIL) from 2 unlabeled inputs, and its per-layer comparison names the RMSNorm variance (ReduceMean, local
8-bit error 0.56) with the first propagated error $>$0.5 at the 1/sqrt; w8a16 $\delta_T$ 0.008. The torch path with toolchain emulation
reproduces the compiled graph before export (MLP $\delta_T$ 1.17 vs 1.15; attention 0.077 vs 0.087). The TFLite cross-runtime check finds the
REDUCE\_SUM bug without labels (first op differing by $>$16 LSB between reference and optimized kernels: op 22 SUM, 127 LSB). Decisions use
the fp32-settled subset of inputs. The S24 chains are running again; if the phone does not collapse at w8a8 (intermediate, \S\ref{r:devices}),
a host check of the QDQ graph flags a failure the phone does not have: M4 must model the kernel, not the graph. Now confirmed: M4's check
says FAIL for the w8a8 Sudoku-MLP graph, right for the literal QDQ semantics on any host executor and wrong for the S24 (61/100, fused RMSNorm), and the S24 Maze w8a8 failure goes the other way:
the central design problem for M4 (REWRITE\_NOTES 45--48).}

\paragraph{M4 read-out (EdgeTRM b3e19ff; results/m4/m4\_readout.md; REWRITE\_NOTES 60).} Ground truth: 140 same-runtime cells over five runtimes
(ORT-fused, reference QDQ, TFLite XNNPACK, TFLite reference = TFLM kernels, torch), 44 cross-runtime rows and 10 AI Hub device chains. Best host signal:
settled written-cell agreement with fp32 (AUROC 1.00; $\varphi_H$ 0.999; one-step $\delta_T$ 0.973). Held out (DriftBench rule), combined check, 129 rows:
leave-one-backend 122/129 (1 false accept, 6 false rejects), leave-one-model 124/129, leave-one-configuration-family 124/129. Shipped rule on 140 cells:
OK 67 PASS / 18 WARN / 0 FAIL; DEGRADED 0 / 7 / 6; BROKEN 0 / 0 / 42. Cross-runtime (44 rows): 8 BROKEN pass and 2 OK fail, every one a kernel mismatch
(S24 Maze w8a8; S24 INT4 cast; TFLite int16; TFLM; and the reverse, S24 MLP w8a8). Device probe: one step is not reliable (leave-one-chain-out 2/10
wrong); two steps against host fp32 separate all 10 chains (working 0.72--1.00, failing 0.00--0.27). Case studies: names the RMSNorm variance / 1/sqrt as
the first broken tensor from 2 unlabeled inputs; the harness-style emulation (8-bit linear inputs only) would have missed the collapse; TFLM REDUCE\_SUM
localised without labels. \redtext{Limits: $n{=}100$ labels, 10 device chains on 2 devices, in-sample rounded thresholds. Mostly MLSys material.}

\section{M5. Halting as early exit}
\label{m:m5}
\textbf{Evidence.} TRM runs all 16 supervision steps at test time although ACT averages fewer than 2 steps in training
(arXiv 2510.04871, \S2.5); the halting head survives compression inside the basin (\S\ref{r:halt}; the Sep 23 ``1.00 at step 2'' claim is withdrawn).
\textbf{Design.} Accuracy against steps saved per model and precision; device latency per solved instance from the measured
per-step latencies (AI Hub, Vela/FVP: 104 ms per MLP step on the U55 at $H{=}1$); combine with M1 (exit, then polish) and M2.
Energy per solved instance stays red. Exit rules: native $q_{\text{halt}}>q_{\text{continue}}$, patience, min-step, a $q$
threshold tuned on fp32 and frozen (two-fold cross-fit on puzzle parity), residual, max-softmax, answer stability, oracle; baselines:
fixed 16 steps and fixed depth matched to the rule's mean steps. \src{EdgeTRM/exit_sweep.py, analyze_m5.py; M5.md}

\begin{table}[H]
\caption{\redtext{\textbf{M5 interim: exit rules at 16 steps}} (existing per-step records, Babel L40S, $n{=}1000$; rule chosen on fp32 alone with
$\le$0.5-point loss and applied unchanged; median over cells [range]; delta vs fixed 16 steps). HRM rows here read $q_{\text{halt}}>0$; HRM's own
rule $q_{\text{halt}}>q_{\text{continue}}$ is lossless (49.4 $\to$ 49.4 at 10.57 steps). \src{analyze_m5.py rules; results/breadth/m5_summary.json; M5.md R1}}
\label{tab:m5}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
Model & Rule & fp32: fixed 16 $\to$ rule (steps) & In-basin: delta, steps & Fixed depth on fp32 & Edge: delta, steps & Out \\
\midrule
\inputrows{tables/bank/m5_rules.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{redpar}
\noindent\textbf{M5 interim readings.} The head saves 2$\times$ (TRM Sudoku), 1.5$\times$ (HRM Sudoku) and 6--8$\times$ (mazes) of the 16 steps at
$\le$0.5 point, unchanged under every in-basin quantizer; no fixed shorter depth matches it on Sudoku. \textbf{Past the edge early exit recovers
accuracy that iterating destroys}: TRM-MLP weight noise 0.15 (3 draws) fixed 16 steps 29.8 $\to$ native exit 52.9 at 9.2 steps (oracle first-correct
55.8); w3g32 51.2 $\to$ 58.4; activation noise 0.3 32.0 $\to$ 40.8. Out of the basin the head goes silent and fails safe. The residual exit transfers
worse and never fires under activation noise. Device latency per solved instance (step latency $\times$ mean steps / accuracy; H=1 step graph):
S24 Sudoku-MLP 253 $\to$ 105 ms; Ethos-U55-256 (Vela, INT8) 7.05 $\to$ 2.91 s; TRM Maze 11.7$\times$ fewer H=1 steps. Energy red; INT8/INT4 device
rows borrow harness accuracy and are latency rows only (X3's w8a8 collapse).
\end{redpar}
\paragraph{M5 round 2: a unified test-time controller (EdgeTRM 2f2cf65+; M5.md R11--R16; REWRITE\_NOTES 62).} Exit, then sample until confident, then an
optional fp32 polish; settings chosen on even puzzles and scored on odd (and vice versa); 41 cells. Without polish it beats fixed depth at budgets $\ge$64
by 1.4--26 points on every TRM/HRM Sudoku cell except out-of-basin MLP w4t (+0.2--0.6), on 4 of 5 HRM Maze cells, and holds on saturated TRM Maze
($\pm$0.4). Past the edge it beats the best single method by 3--4 (MLP w3g32 at 64 steps: 63.1 vs fixed 51.8, best single 58.8). With fp32 polish it
recovers models no single method moves at 256 steps (MLP w4t 6.2 $\to$ 46.1; w3c 17.9 $\to$ 51.8). It trails best-of-$K$ by 0.3--6.7 on some HRM
noise and 2-bit cells. DT mazes: an answer-unchanged exit is at or above the fixed curve everywhere, up to +25 (33$\times$33 w4t at 150 iterations:
88.6 vs 65.7). \textbf{DEQs: negative} for past-edge recovery (Broyden accuracy is budget-flat; Picard: longer hurts; DEQ-T's early cap helps but no
label-free signal finds it). Exit rules transfer to trained seeds without re-selection (attention $-0.3$..+0.4 at $\sim$8 / 16 steps; MLP 0.0 at
$\sim$6.3 / 16); HRM at 512: steps per solved w8c 881 $\to$ 392. \src{EdgeTRM/figures/m5_controller_frontier.pdf; M5.md}
\running{looped-LM (Ouro learned exit gate); the fp32 visit-then-lose baseline (required check 2 of the angles scan)}

\paragraph{M5 exit + M1, final (M5.md R16; EdgeTRM 00ab54f; $n{=}1000$, 12 cells; REWRITE\_NOTES 77).} Rule: the cheap map runs until its head halts twice
(capped at $T-32$), then INT8 steps until the INT8 head halts twice (at most 32). Released attention: within $\pm$0.3 of M1's fixed schedule at 3.0--4.2$\times$
fewer steps ($T{=}128$ w3c 80.6 vs 80.7 at 42 steps; $T{=}256$ 82.4 vs 82.4 at 73; $T{=}512$ 83.9 vs 84.1 at 123); seed s0 equal at 3.9--4.3$\times$ fewer. Seeds
that overthink in fp32: s1 n8c3 +2.6 $\pm$1.0; s2 n8c3 71.0 vs 45.3 (+25.7 $\pm$2.8), w3g32 +19.2. The INT8 polish is not replaceable by the exit (exit alone
74.4 / 76.7 at $T$ 128 / 256 vs 80.6 / 82.4). fp32 + exit at $T{=}256$: 75.9 at 72 steps. \running{Ouro exit gate, p4d card 7}

\section{M6. Basin-widening training (owned by X5)}
\label{m:m6}
\textbf{First result} (REWRITE\_NOTES 66, \S\ref{r:qat}): naive QAT roughly doubles basin width around its INT4 point ($\sigma_{1/2}$ 0.28--0.30 vs
$\sim$0.14) by lowering $S$ (0.84--1.12 vs 1.28--2.10). \redtext{The fp32 fine-tune control is pending; the sensitivity-penalty arm is being retried.}

Noise injection, Jacobian penalty and QAT (\S\ref{r:qat}), plus a sensitivity ($\delta_T$) penalty and a CompreSSM-style
in-training compression arm. First evidence: naive per-tensor INT4 QAT takes w4t from 0.0 to 52.3 (seed 0) while the latent fp32
weights collapse; endpoints 52.3 / 61.2 / 56.4 over three seeds (\S\ref{r:qat}). Arms: sensitivity penalty, gradual in-training
compression (gqat), late forks, W+A bridge, noise injection, Jacobian penalty. \running{p4d cards 3--5, lsens $\sim$10:00 Sep 25, gqat
$\sim$16:00--20:00, the rest Sep 26}


==> sections/related_work.tex <==
% Related work, ICLR rewrite (Sep 24). Sources: reports/edgetrm_lit/0[1-6]*.md; scope rules in
% reports/edgetrm_exp/REWRITE_NOTES.md. Similar prior work is cited as corroboration, and each paragraph
% ends on what we add (Steven, Sep 24). Our own June preprint is not cited: its arXiv version will be
% updated. Ingolfsson et al. cited as concurrent (decision D3). \pending claims wait on the X read-outs.
\section{Draft related work (Sep 24)}
\label{sec:related}

\paragraph{Quantizing recursive and looped models.}
Concurrent work reaches the same quantization recipe on the models we study:
\citet{ingolfsson2026quantizing} show on TRM-style and equilibrium reasoners that the granularity of
the scales decides whether 4-bit quantization survives, and attribute the failures to a systematic
bias that accumulates with reuse. LoopQ \citep{fang2026loopq} corrects looped language models for
the same accumulation across loop roles. We measure what the accumulation account predicts and find
a boundary instead: inside a model's basin the cost of compression is fixed at every depth, outside
it the model fails at every depth, zero-mean weight noise alone produces the cliff, and the token
mixer sets how wide the basin is (\S\ref{sec:boundary}, \S\ref{sec:width}).

\paragraph{Equilibrium theory.}
Deep equilibrium models compute the fixed point of one layer \citep{bai2019deq}, and monotone
operator equilibrium networks guarantee that the fixed point exists and is unique
\citep{winston2020mondeq}. For these networks, quantization provably preserves convergence while
the weight perturbation stays below the monotonicity margin, and the solver diverges beyond it
\citep{mondeqquant2026}; that result is the certified form of the boundary we measure. The
reasoners we study carry no such certificate, and their recursion expands along its worst-case
direction, yet the same boundary appears, and its edge follows how far one perturbed step moves
the state (\S\ref{sec:mechanism}).

\paragraph{Recursive reasoners and test-time iteration.}
Recursive reasoners iterate one small weight-tied block: HRM nests two recurrent modules
\citep{wang2025hrm}, TRM replaces them with a single tiny network \citep{jolicoeur2025trm},
deep-thinking networks extrapolate to larger instances by iterating longer
\citep{schwarzschild2021deepthinking,bansal2022overthinking}, and looped language models reuse
their core block at test time \citep{geiping2025recurrentdepth,zhu2025ouro}. For language models,
compression is known to lower what test-time compute can reach: pruning lowers the attainable
ceiling of test-time scaling \citep{pruningtts2025}, quantized reasoning models gain less from
longer reasoning \citep{liu2025quanthurts}, and the memory that 4-bit weights save cannot buy the
loss back as a longer budget \citep{quantmemory2025}. In iterative refinement, the working
precision sets the limiting accuracy and the solver precision sets the rate
\citep{carson2018threeprecisions}. For learned weight-tied reasoners, quantization inside the basin
moves neither; past its edge it lowers the limiting accuracy of test-time scaling, and the loss grows
with the size and difficulty of the instance (\S\ref{sec:cap}).

\paragraph{Halting heads and label-free evaluation.}
Adaptive computation learns when to stop iterating \citep{graves2016act,banino2021pondernet}, and
the halting heads of TRM and HRM separate right from wrong answers on Sudoku in full precision
\citep{sghaier2026ptrm,haltingverifier2026a,haltingverifier2026b},
as ours do. We turn that signal into a reference-free defer rule for compressed models: the head's
own threshold holds at every precision inside the basin, and on mazes the head detects invalid
paths (\S\ref{sec:defer}). For compressed language models, agreement with
the full-precision outputs exposes damage that accuracy hides \citep{dutta2024accuracy,kurtic2024bf16},
although output divergence ranks near-lossless quantizers poorly \citep{kldquality2026}. Our
fidelity compares final latent states, needs neither labels nor decoding, and works as a filter
once its unit is the output cell\redtext{, because exact match over a long output compounds a small per-cell
risk into a large per-answer one \citep{schaeffer2023mirage}}. \caveat{correction (X8 final): the per-cell compounding clause is withdrawn
for TRM/HRM (wrong answers are wholesale; the product model fails); keep ``once its unit is the output cell'' (\S\ref{r:fid})}

\paragraph{Test-time compute on edge devices.}
Test-time scaling at the edge has so far meant scheduling the token generation of language models
on phones and embedded GPUs \citep{edgereasoning2025,fasttts2025}. A weight-tied reasoner holds
its memory constant as it iterates, so its edge budget is latency alone; looped language models
reach that regime only when their cache is shared across loops \citep{melt2026}.


==> sections/results_bank.tex <==
% Results bank, part 1 (R1-R8). Every result with its numbers and the file each number comes from.
% Tables under tables/bank/ are generated from the status files by tables/bank/md2tex.py (rerun it when a
% status file changes); tables under tables/ are generated in EdgeTRM/plots/*.py (TRM H=3, HRM H=2).
% Numbers are allowed everywhere in this bank. Red = unresolved.

% ---------------------------------------------------------------------------------------------------
\section{R1. Depth: the cost of compression at every setting of the depth dial}
\label{r:depth}

\begin{table}[H]
\caption{\textbf{The cost of compression does not grow with depth.} Gap to fp32 in exact accuracy
(points) at 4 and 32 supervision steps; the first row is fp32 accuracy (\%). Per-tensor INT4 on the
MLP-mixer Sudoku model fails at both depths; every other gap stays within eight points at both,
and none widens by more than three. Weight-only post-training quantization; 1000 test instances per
cell; TRM at $H{=}3$, HRM at $H{=}2$. \src{EdgeTRM/tables/tab_depth_matrix.tex (plots/depth_table.py --matrix); results/breadth/{task}_all.json, {task}_deep.json (p4d)}}
\label{tab:depth}
\centering\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{@{}l rr rr rr rr rr@{}}
\toprule
& \multicolumn{2}{c}{TRM Sudoku, MLP} & \multicolumn{2}{c}{TRM Sudoku, attn.}
& \multicolumn{2}{c}{TRM Maze} & \multicolumn{2}{c}{HRM Sudoku} & \multicolumn{2}{c}{HRM Maze} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(l){10-11}
Supervision steps & 4 & 32 & 4 & 32 & 4 & 32 & 4 & 32 & 4 & 32 \\
\midrule
\inputrows{tables/tab_depth_matrix.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Absolute accuracies at the shallowest and default depth.} fp32 and quantized exact accuracy
(\%) at 1 and 16 supervision steps and the gap (points). The one widening gap (MLP per-tensor INT4,
$-26.3\to-65.5$) is fp32 climbing 28.4$\to$71.4 while the broken model sits at 2.1$\to$5.9. Static INT8
activations halve Sudoku-MLP at one step and cost nothing at 16. 1000 instances; TRM $H{=}3$, HRM $H{=}2$.
\src{EdgeTRM/tables/tab_depth_rows.tex (plots/depth_table.py --latex)}}
\label{tab:depth-rows}
\centering\footnotesize
\begin{tabular}{@{}ll rrr rrr@{}}
\toprule
& & \multicolumn{3}{c}{1 step} & \multicolumn{3}{c}{16 steps} \\
\cmidrule(lr){3-5}\cmidrule(l){6-8}
Model & Quantizer & fp32 & quant. & gap & fp32 & quant. & gap \\
\midrule
\inputrows{tables/tab_depth_rows.tex}
\bottomrule
\end{tabular}
\end{table}

\paragraph{Other depth evidence.}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item Master Table C (Sep 13--23): gap at $n_{\text{sup}}{=}1$ vs 16 flat or shrinking for 29 of 30
  model$\times$quantizer pairs (TRM ARC w4t 16.2$\to$10.0, w3g32 6.5$\to$4.0; TRM Sudoku-attn w4t 1.3$\to$2.9; the
  exception is Sudoku-MLP w4t 26.3$\to$65.5, explained above). \caveat{HRM rows of master Table C mix $H$ (REWRITE\_NOTES 27);
  Table~\ref{tab:depth-rows} is the corrected read} \src{reports/EDGETRM_MASTER_TABLES.md C}
\item ARC-AGI-1, official protocol (400 tasks, 1000-augmentation vote), pass@2 / pass@1: fp32 44.75 / 40.50 at
  $H{=}3$, $n{=}16$ (published 44.6) and 45.75 / 41.50 at $H{=}1$, $n{=}8$; w4c 44.50 / 39.50 and 45.00 / 40.25;
  w4t 39.75 / 36.00 and 40.25 / 36.50. The shallow configuration loses nothing (Table~\ref{tab:arc}).
\item Looped LMs: Huginn w4c 27.5 / 27.0 / 26.0 on GSM8K at 16 / 32 / 64 recurrences (bf16 40.0 at each; $n$ =
  200 / 100 / 50). \src{results/breadth/huginn_gsm8k_*.json; master Table E}
\item DEQ solver cap as depth (X6, \S\ref{r:transfer}): MDEQ-Small accuracy flat from $k{=}16$ to 100 at every $\sigma$
  (changes within $\pm0.2$).
\item Depth dose-response on Ingolfsson's axes ($n_{\text{sup}}$ 1--32, $H\in\{1..6\}$, $L\in\{1..8\}$, scales calibrated once; X7): flat or shrinking in 11 of 12 in-basin
  series with paired CIs; two bounded exceptions (\S\ref{r:x7}, Table~\ref{tab:x7depth}).
\end{itemize}

% ---------------------------------------------------------------------------------------------------
\section{R2. Zero-mean weight noise: the dial}
\label{r:noise}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/noise_dial.pdf}
\caption{\textbf{Zero-mean weight noise reproduces the boundary.} Exact accuracy (top) and fidelity
$\varphi_H$ (bottom) at 16 supervision steps against the noise level $\sigma$, the standard deviation
of each weight's noise as a fraction of its tensor's. Each point is one random draw, three per
$\sigma$; the line joins the medians; the dotted line is fp32 and the dashed line marks
$\varphi_H = 0.85$. Each Sudoku model falls off a cliff over a narrow range of $\sigma$, where
$\varphi_H$ crosses the dashed line; the maze models stay inside their basin over the whole dial.
1000 test instances per point; every draw on one platform (A100); TRM at $H{=}3$, HRM at $H{=}2$.
\src{EdgeTRM/figures/noise_dial.pdf (plots/noise_dial.py, commit 1c8efa5); results/breadth/p4d/noise_rerun/*.json + draw 0 in results/breadth/{task}_noise.json}}
\label{fig:noise}
\end{figure}

\paragraph{Medians at the cliffs (coordinator read-out of the p4d rerun, Sep 24 23:20 UTC).}
Sudoku-MLP (fp32 71.4): $\sigma{=}0.15$ median 33.6 (draws 36.8 / 23.8 / 33.6), $\sigma{=}0.2$ 4.9.
Sudoku-attn (fp32 65.7): $\sigma{=}0.7$ 50.2, $\sigma{=}1.0$ 1.8. HRM Sudoku (fp32 49.2 at $H{=}2$): $\sigma{=}1.0$ 26.0.
Maze models hold to $\sigma{=}1.0$: TRM Maze 85.7--86.1 (fp32 87.0); HRM Maze 70.0--70.9 (fp32 74.3).
Larger $\sigma$ on mazes (X1 re-scoring, Babel, one draw): TRM Maze weight noise 1.0 / 1.5 / 2.0 gives
valid-shortest 91.5 / 76.5 / 0.0; HRM Maze 76.5 / 53.7 / 2.1 (\S\ref{r:maze}).
\src{results/breadth/p4d/noise_rerun/; X1.md}

\paragraph{Deep-thinking mazes: the edge is a distribution over draws.} 300 iterations, exact: size 33, $\sigma{=}0.2$
100.0 / 98.0 / 99.9 ($\varphi$ 0.973--0.975); $\sigma{=}0.3$ 4.0 / 0.3 / 74.1 ($\varphi$ 0.817 / 0.746 / 0.940). Size 25,
$\sigma{=}0.3$: 20.9 / 3.6 / 82.4 ($\varphi$ 0.850 / 0.776 / 0.942). Fidelity ranks the three draws correctly every
time. At 100 iterations (one draw), $\sigma{=}0.3$ keeps 72.8 of 100 on size-9 mazes and 1.4 of 55.1 on size 33.
\src{results/breadth/p4d/dt_cell_mazes_{25,33}_s{0,1,2}.json; dt_mazes_noise.json; EDGETRM_OPEN_QUESTIONS.md Q2}

\paragraph{Trained variants.} Three draws per $\sigma$ leave every variant's $\sigma_{1/2}$ unchanged (MLP 0.15--0.2 at
all widths; attention w512 0.7 or beyond); draw spreads exceed 10 points only on each variant's cliff cell (MLP
w256 s1 at $\sigma{=}0.15$: 10 / 30 / 23; MLP w512 s2: 21 / 14 / 8). \src{results/breadth/p4d/variants_noise/*.json; analyze_openq.py q8b}

% ---------------------------------------------------------------------------------------------------
\section{R3. Activation noise: the same cliff at the same fidelity}
\label{r:anoise}

\begin{table}[H]
\caption{\textbf{Gaussian noise at every linear input, drawn afresh at every pass, has a plateau and a cliff}, and
the cliff sits where $\varphi_H$ falls through about 0.8, as for weight noise. Exact accuracy (\%), $\varphi_H$ in
parentheses; 16 supervision steps. The attention mixer's activation basin is about twice as wide as the MLP
mixer's. \caveat{TRM rows on Babel (L40S), HRM rows on p4d: one platform per model, not per table; one draw per
$\sigma$ (X8 runs three); HRM $H$ of this file to confirm against the $H{=}2$ rule}
\src{results/breadth/{babel,p4d}/anoise_*.json; analyze_openq.py q5}}
\label{tab:anoise}
\centering\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l l l l l l@{}}
\toprule
Model & fp32 & & & & \\
\midrule
TRM Sudoku-MLP & 70.8 & $\sigma$0.1: 68.9 (0.90) & 0.2: 63.3 (0.85) & 0.3: 33.2 (0.60) & 0.5: 2.1 (0.38) \\
TRM Sudoku-attn & 66.0 & $\sigma$0.3: 64.1 (0.91) & 0.5: 45.5 (0.81) & 0.7: 1.0 (0.58) & \\
HRM Sudoku & 49.2 & $\sigma$0.3: 45.0 (0.93) & 0.5: 11.2 (0.79) & 0.7: 0 (0.58) & \\
TRM Maze-attn & 88.4 & $\sigma$0.7: 86.0 (0.97) & 1.0: 24.6 (0.915; cell 99.4) & & \\
HRM Maze & 74.8 & $\sigma$0.7: 69.6 (0.974) & 1.0: 41.4 (0.929) & & \\
\bottomrule
\end{tabular}}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Depth repairs inside the basin only}: Sudoku-MLP at $\sigma{=}0.2$, $n{=}1\to16$: 8.4$\to$63.3 (fp32
  28.4$\to$70.8); at 0.3: 2.3$\to$33.2; at 0.5: 1.3$\to$2.1.
\item \textbf{Sources compound}: w8c + $\sigma$0.2 = 64.2 ($\varphi$ 0.845) $\approx$ $\sigma$0.2 alone 63.3 (0.847);
  w4c + $\sigma$0.2 = 58.6 ($\varphi$ 0.777).
\item \textbf{Static INT8 activations (+a8) sit inside the plateau} for every model at 16 steps
  (Table~\ref{tab:a8}); the device's all-op UINT8 encoding does not (\S\ref{r:devices}).
\item \textbf{PTRM's latent noise} (Gaussian on $z_L$ before each step, absolute $\sigma$ 0.3 on MLP-Sudoku, 1.0 on
  attention-Maze, best-of-K by the $Q$ logit) is productive where our relative activation noise is destructive; the two
  are run side by side on our checkpoints \running{X8 PTRM, $\sim$03:00 UTC}.
\end{itemize}

% ---------------------------------------------------------------------------------------------------
\section{R4. Granularity: which side of the boundary a quantizer lands on}
\label{r:gran}

\begin{table}[H]
\caption{\textbf{Scale granularity decides the side of the boundary; the token mixer sets its
width.} Top: exact accuracy (\%) of the released checkpoints at 16 supervision steps, with INT4
weights scaled per tensor, per output channel, or per group of 128 weights. Bottom: Sudoku models we
trained with each mixer and width, one entry per seed: fp32 accuracy, accuracy under per-tensor
INT4, and $\sigma_{1/2}$, the weight-noise level at which the median of three draws falls below half
of fp32 accuracy (larger is a wider basin). 1000 test puzzles; TRM at $H{=}3$, HRM at $H{=}2$.
\src{EdgeTRM/tables/tab_gran_released.tex, tab_mixer_rows.tex (plots/granularity_table.py)}}
\label{tab:width}
\centering\small
\begin{tabular}{@{}l rrrr@{}}
\toprule
& & \multicolumn{3}{c}{INT4, one scale per} \\
\cmidrule(l){3-5}
Released checkpoint & fp32 & tensor & channel & group (128) \\
\midrule
\inputrows{tables/tab_gran_released.tex}
\bottomrule
\end{tabular}

\vspace{6pt}
\begin{tabular}{@{}ll lll@{}}
\toprule
Mixer & Width & fp32 & INT4 per tensor & $\sigma_{1/2}$ \\
\midrule
\inputrows{tables/tab_mixer_rows.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{The full weight-quantizer ladder at the deepest setting} (master Table B): exact \%, fidelity of the
final carry in parentheses. Bit-width does not order the quantizers: grouped INT3 keeps 51.4 on Sudoku-MLP where
per-tensor INT4 keeps 5.9; per-tensor INT4 kills deep-thinking chess (0.4 of 84.4). \caveat{HRM rows are an older
read that mixes $H$ (fp32 51.0 vs 49.2 at $H{=}2$; REWRITE\_NOTES 27); regenerate before use}
\src{reports/EDGETRM_MASTER_TABLES.md B (make_tables.py); results/breadth/*.json}}
\label{tab:ladder}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l lllllllll@{}}
\toprule
Family / task (fp32) & w8c & w6c & w4g32 & w4c & w4a & w4t & w3g32 & w3a & w2g32 \\
\midrule
\inputrows{tables/bank/mt_B.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[H]
\caption{\textbf{ARC-AGI-1 under the official protocol} (400 tasks, 1000-augmentation vote): pass@2 / pass@1
(\%), fidelity in parentheses. The $H{=}1$, $n{=}8$ configuration (5 applications of the block per step, 40 per
answer) matches the official $H{=}3$, $n{=}16$. \src{reports/EDGETRM_MASTER_TABLES.md A; results/breadth/arc_attn_*.json}}
\label{tab:arc}
\centering\footnotesize
\begin{tabular}{@{}l ll@{}}
\toprule
Quantizer & $H{=}3$, $n{=}16$ (published 44.6) & $H{=}1$, $n{=}8$ \\
\midrule
fp32 & 44.75 / 40.50 & 45.75 / 41.50 \\
w8c & 44.75 / 40.50 (0.99) & 45.75 / 41.50 (1.00) \\
w6c & 44.75 / 40.75 (0.97) & 45.50 / 41.25 (0.99) \\
w4g32 & 45.00 / 40.00 (0.93) & 44.75 / 40.75 (0.96) \\
w4g128 & 45.00 / 40.00 (0.92) & 45.00 / 40.25 (0.94) \\
w4c & 44.50 / 39.50 (0.90) & 45.00 / 40.25 (0.93) \\
w4a & 44.75 / 38.50 (0.91) & 44.50 / 38.75 (0.94) \\
w3g32 & 41.75 / 38.00 (0.83) & 43.50 / 38.50 (0.86) \\
w3a & 41.25 / 36.25 (0.77) & 41.25 / 36.50 (0.80) \\
w4t & 39.75 / 36.00 (0.74) & 40.25 / 36.50 (0.76) \\
w2g32 & -- & 0.00 / 0.00 (0.16) \\
w8c+a8 & 41.25 / 36.25 (0.78) & 41.50 / 36.75 (0.84) \\
w4g32+a8 & 41.50 / 36.50 (0.75) & 41.25 / 37.25 (0.81) \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Static INT8 activations (+a8) at one step and at the deepest setting} (master Table D): exact \%,
fidelity in parentheses. INT8 activations halve Sudoku-MLP at one step and cost nothing at 16; ARC loses 5--10 points
at both depths; the attention Sudoku, maze and HRM models do not care. \caveat{HRM rows at $H{=}3$}
\src{reports/EDGETRM_MASTER_TABLES.md D; results/breadth/*_a8.json}}
\label{tab:a8}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll llllll@{}}
\toprule
Task (fp32) & Setting & w8c & w8c+a8 & w4g32 & w4g32+a8 & w4c & w4c+a8 \\
\midrule
\inputrows{tables/bank/mt_D.tex}
\bottomrule
\end{tabular}}
\end{table}

\paragraph{Chip-realisable quantizers (X3 E0, Babel L40S, deterministic, $n{=}1000$).}
Sudoku-MLP exact \% at $H{=}1$, $n{=}16$ (fp32 64.2): LPBQ-grid INT4 w4l128 / l64 / l32 = 62.4 / 61.8 / 60.8 against
float-scale groups w4g32 63.0, w4g128 62.3, per-channel w4c 61.5, per-tensor w4t 4.9. INT16 activations cost nothing
(w4l64+a16 61.9, w4c+a16 61.5, w8c+a16 63.7); harness INT8 activations at linear inputs cost 1--3 points (w4l64+a8 60.5,
w4c+a8 59.2). At $H{=}1$, $n{=}8$ (fp32 55.0): w4l64 54.2, w4g32 55.1, w4c 52.5, w4c+a8 46.7. So Qualcomm's LPBQ block
scales, the only grouped INT4 on Hexagon, keep the grouped-INT4 recipe.
\running{Sudoku-attn, Maze, HRM E0 files}
\src{EdgeTRM/results/devices/chipq/chipq_sudoku_mlp.json (job 10553046); results/devices/chipq_tables.md}

\paragraph{Granularity in the literature.} Ingolfsson et al.\ publish granularity as the control variable for
activations (per-tensor 0.0\% $\to$ MXInt4 80.1\% on their Sudoku); ALBERT survives k-means 5-bit and collapses under
linear 5-bit; Apple's Core ML guide: ``per-block granularity is required'' at 4 bits (\S\ref{lit:quant}).

% ---------------------------------------------------------------------------------------------------
\section{R5. The mixer sets the width; width does not}
\label{r:mixer}

\begin{table}[H]
\caption{\textbf{Trained Sudoku variants, one row per seed} (step 65,100; 1000 puzzles; $H{=}3$, $n_{\text{sup}}{=}16$):
fp32, per-tensor INT4, per-channel INT4 and $\sigma_{1/2}$ (median of three draws). Attention at width 256 is
undertrained (fp32 10--28\%) and its $\sigma_{1/2}$ is not comparable. \src{EdgeTRM/tables/tab_granularity_rows.tex Part B (plots/granularity_table.py); results/breadth/p4d/variants_noise/}}
\label{tab:variants}
\centering\footnotesize
\begin{tabular}{@{}llr rrrl@{}}
\toprule
Mixer & Width & Seed & fp32 & INT4 tensor & INT4 channel & $\sigma_{1/2}$ \\
\midrule
\inputrows{tables/tab_gran_variants_rows.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Other quantizers on the variants} (Q8): w4c within 2 points of fp32 everywhere; w3g32 inside for attention
  (54--66 vs fp32 53--65) and at the edge for MLP (15--35 at w256, 74--76 at w512, 64 at w768: width helps here).
\item \textbf{Fragility forms during training} (master Table F; per-tensor INT4 fidelity along training at checkpoints
  6,510$\to$65,100): MLP w256 s0 0.96$\to$0.22 (w4t 7.7$\to$0.0 while fp32 12.3$\to$59.9); MLP w512 s0 0.98$\to$0.43;
  MLP w768 0.96$\to$0.40; attention w512 s0 0.97$\to$0.89 (w4t 65.5 of 64.8 at the end); attention w512 s2
  0.96$\to$0.76; attention w256 s0 0.95$\to$0.73. \src{reports/EDGETRM_MASTER_TABLES.md F; results/breadth/lambda/variant_*.json}
\item \textbf{The one-step Jacobian does not explain the width} (X5): $\lVert J\rVert_F^2/\text{dim}$ and top singular
  value of $z_L\mapsto L_{\text{level}}(z_L, z_H{+}x)$ at the final carry (256 puzzles): MLP w256 s0/s1/s2 0.170 / 0.202
  / 0.142, top s.v.\ mean 4.47 / 3.93 / 3.27; attention w512 s0/s1/s2 0.231 / 0.262 / 0.239, 8.58 / 8.81 / 7.88. The
  wide-basin mixer has the \emph{larger} per-step Jacobian; per-tensor INT4 relative weight error is similar for the two
  mixers (0.33--0.44). The difference is sensitivity (\S\ref{r:mech}), not outliers.
  \src{X5.md; p4d:q7/lambda_eval/jac_finals.json}
\item \textbf{Size in looped LMs} (confounded by training): Ouro-2.6B w4c survives (29--78\% across loops, $\varphi$
  0.81--0.85) where Ouro-1.4B dies ($\varphi$ 0.70--0.74) (\S\ref{r:lm}). MDEQ-XL loses 1.0 point at $\sigma{=}0.1$ where
  MDEQ-Small loses 5.9 (\S\ref{r:transfer}).
\end{itemize}

% ---------------------------------------------------------------------------------------------------
\section{R6. Test-time scaling under compression (X1)}
\label{r:tts}

\subsection{Deep-thinking mazes: an instance-size axis where fp32 reaches 100\%}
\label{r:tts-dt}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/extrapolation.pdf}
\caption{\textbf{Deep-thinking maze solver (trained with 30 iterations) at test-time iterations 10--500, by maze
size.} fp32 reaches 100\% at 40 / 40 / 100 / 150 / 200 iterations for sizes 9 / 13 / 19 / 25 / 33; per-tensor INT4
plateaus below it, lowest on the largest mazes. $n{=}1000$ per point, p4d.
\src{EdgeTRM/figures/extrapolation.pdf (plots/extrapolation.py); results/breadth/p4d/dt_extrap_*.json}}
\label{fig:extrap}
\end{figure}

\begin{table}[H]
\caption{\textbf{At 100 iterations, compression breaks the largest mazes first} (\% solved; $n{=}1000$).
\src{results/breadth/dt_mazes.json; EDGETRM_OPEN_QUESTIONS.md \S0}}
\label{tab:dt100}
\centering\footnotesize
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Maze size & 9 & 13 & 19 & 25 & 33 \\
\midrule
fp32 & 100 & 100 & 99.8 & 85.0 & 55.1 \\
w8c & 100 & 100 & 99.8 & 85.0 & 55.0 \\
w4g32 & 100 & 100 & 99.9 & 84.4 & 55.3 \\
w4c & 100 & 100 & 98.4 & 79.6 & 44.4 \\
w4t & 99.0 & 96.4 & 93.3 & 74.2 & 41.3 \\
\midrule
\multicolumn{6}{@{}p{0.95\textwidth}@{}}{Plateau at 500 iterations (the cap): w4t 99.2 / 96.4 / 94.7 / 91.4 / 88.4; w3a 99.7 / 99.5 / 98.7 / 97.4 / 95.3;} \\
\multicolumn{6}{@{}p{0.95\textwidth}@{}}{w3g32 100 / 99.8 / 99.2 / 99.1 / 98.0; w4c 98.9 at size 33; noise $\sigma$0.2 (one draw) 98.5 / 92.9 / 81.3 / 68.9 / 57.2; $\sigma$0.5: 0.} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Cap versus tax, size-33 mazes.} Fit $\text{acc}(T) = A(1-e^{-(T-T_0)/\tau})$; $\Delta A$ and log ratios
against fp32 with 95\% paired-bootstrap intervals (400 resamples of the 1000 instances); $T_{90}$ is model-free. Fit
rmse 2--4 points, so $A$ is reliable to about a point and $\tau$ is coarse. \src{EdgeTRM/analyze_captax.py fit dt; X1.md}}
\label{tab:captax}
\centering\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Size 33 & acc@500 & $A$ [95\%] & $\Delta A$ vs fp32 & $\log(\tau/\tau_{\text{fp32}})$ & $\log(T_{90}/T_{90,\text{fp32}})$ \\
\midrule
\inputrows{tables/bank/x1_captax33.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{w4t's cap grows with size, its rate does not}: $\Delta A$ = 0.0 / $-3.4$ / $-4.3$ / $-7.6$ / $-8.0$ at
  sizes 9 / 13 / 19 / 25 / 33, while its $T_{90}$ ratio stays at +0.06 to +0.07 (6--7\% more iterations) at every size.
\item \textbf{A small tax on common instances} (stable solve on the 10..500 grid): lossless-granularity quantizers
  solve at the same count (w8c/w6c/w4g32/w4g128: 96--100\% ``same'', mean $\log_2$ ratio $\le$+0.03). Lossy ones solve
  8--19\% of common instances one grid step later: size 33 w4c 18.4\% later, mean $\log_2(T_q/T_{\text{fp32}})$ = +0.19
  [+0.16, +0.23] ($\sim$14\% more iterations); w4t 13.2\%, +0.12 [+0.09, +0.15]; w3a 17.1\%, +0.08; noise 0.2 35\%,
  +0.39. Suggested wording (X1): ``compression lowers the ceiling and barely changes the rate: 8 points of ceiling vs
  6--9\% more iterations (w4t, size 33).''
\item \textbf{The cap follows $(1-h)^L$ with an onset hazard, not independent per-cell error}: one hazard $h$ per quantizer
  fitted to the size-33 cap predicts the other sizes (w4t, $h$ = 0.11 per 1000 target cells: predicted 99.1 / 98.1 /
  96.8 / 94.9 at sizes 9--25 vs fitted 100 / 96.4 / 95.7 / 92.4; noise 0.2: 94.4 / 90.0 / 81.9 / 72.6 vs 99.6 / 92.7 /
  81.3 / 70.7) and the path-length gradient (size 33 w4t by quartile: observed 2.8 / 9.0 / 15.0 / 19.2\%, predicted 3.9 /
  10.1 / 14.0 / 18.1\%). But $h$ is 1/40 of the measured per-cell error (w4t size 33 target-cell accuracy 99.52\%);
  i.i.d.\ cells would give 97.6\% failures instead of 12.4\%; failing mazes carry $\sim$30 wrong target cells each.
  \src{analyze_captax.py length}
\item \textbf{Which instances fail}: at 300 iterations w4t's failure rate by path-length quartile is 3.6 / 10.6 / 15.0 /
  20.0\% (size 33) and 0.4 / 6.5 / 8.6 / 18.7\% (size 25); w3a 0.8$\to$10.4\%. fp32's iterations-to-solve is
  anti-correlated with path length (Spearman $-0.85$ at size 33, $-0.87$ at 25), so ``fails where fp32 is fastest''
  (w4t size 33: 19.6\% of instances fp32 solves by 40 iterations vs 4.8\% of those needing 200) is ``fails on the longest
  outputs''. \src{analyze_openq.py q1b, q2b}
\item \textbf{Two failure trajectories}: on the large mazes the failures at 500 iterations never arrived at the answer
  (size 33: w4t 92\%, w3a 98\%, noise 0.2 93\%; size 25: 86 / 96 / 92\%); on small mazes many arrived and then left for a
  stable wrong fixed point (size 9 w4t 70\%; size 13 56\%). \src{analyze_openq.py q1c}
\item \textbf{Chess and prefix sums}: chess (2 target cells) fp32 peaks at 85.4 at 40 iterations and drifts to 83.8 by
  500 (overthinking); w4c caps at 76.5, w4a 80.7, w3g32 82.2, w3a 22.5, w4t 0.5. Prefix sums 256/512: every quantizer
  incl.\ w4t and w3a reaches 100 at fp32's iteration count (150 / 300).
\end{itemize}

\subsection{TRM and HRM on Sudoku: a difficulty axis and a depth axis to 512 steps}
\label{r:tts-sudoku}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/x1_difficulty_first1000.pdf}
\caption{\textbf{Read-out A: accuracy against ACT steps (1--64) by tdoku rating bin}, first 1000 test puzzles (easy
0--4, $n{=}269$; medium 5--30, $n{=}450$; hard $\ge$31, $n{=}281$), fp32 and three quantizers per model; p4d.
\src{EdgeTRM/plots/x1_difficulty_first1000.pdf (analyze_difficulty.py fig)}}
\label{fig:x1a}
\end{figure}

\begin{table}[H]
\caption{\textbf{Read-out A} (existing p4d records, first 1000 puzzles, rating bins easy / medium / hard). Accuracy \%
at $n_{\text{sup}}$ 16 and 64, gain, and gap to fp32 at 64 with 95\% paired intervals. fp32 test-time scaling is a
hard-puzzle effect; in-basin quantizers track fp32 in every bin; MLP w3g32 stops scaling; attention w3c lags and
catches up. \src{EdgeTRM/analyze_difficulty.py first; X1.md}}
\label{tab:x1a}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Model & Quantizer & $n_{\text{sup}}$ 16 & $n_{\text{sup}}$ 64 & Gain 16$\to$64 & Gap to fp32 at 64 [95\% CI] \\
\midrule
\inputrows{tables/bank/x1_readoutA.tex}
\bottomrule
\end{tabular}}
\end{table}

\paragraph{Difficulty axis, revisited.} The planned axis (tdoku backtrack rating) is monotone for these models only between
rating 0 and $>$0 (TRM-MLP fp32 at 64 steps: 99.4 / 82.9 / 72.9 / 76.8 / 75.6 / 84.2\% for rating 0 / 1--10 / 11--30 /
31--60 / 61--120 / $>$120; the top bin is 83\% forum-hardest puzzles). A model-independent measure, blanks left after
naked and hidden singles (``singles residual''), tracks fp32's iterations-to-solve better (Spearman 0.55 / 0.55 / 0.58
for TRM-MLP / TRM-attn / HRM vs 0.42 / 0.43 / 0.38 for the rating). Bins fixed once: 0 | 1--45 | 46--50 | 51--55 |
$\ge$56. \caveat{the axis was chosen after seeing that the rating is non-monotone for fp32 (fp32 only, no quantizer);
the paper must say so} \src{EdgeTRM/sudoku_difficulty.py; results/breadth/sudoku_extreme_test_meta.json}

\begin{table}[H]
\caption{\textbf{K=64 stratified sweep, TRM Sudoku-MLP} (Babel L40S; 6000 puzzles; bins by singles residual, $n$ =
755 / 917 / 751 / 1489 / 2088). Accuracy at 64 steps for fp32, gap to fp32 [95\%] for the others (gain 16$\to$64 in
parentheses); w4t / w3c as absolute accuracy. \caveat{Babel-only supplementary file; the p4d K=64 files for attention and
HRM are queued} \src{analyze_difficulty.py strat\_babel --axis residual; job 10553001}}
\label{tab:x1strat}
\centering\footnotesize
\begin{tabular}{@{}llllll@{}}
\toprule
Quantizer & res 0 & res 1--45 & res 46--50 & res 51--55 & res $\ge$56 \\
\midrule
\inputrows{tables/bank/x1_strat64.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/x1_difficulty_deep_residual.pdf}
\caption{\textbf{K=512 deep sweep by singles-residual bin} (p4d A100; 1800 puzzles = 300 per rating bin). Top: TRM
Sudoku-MLP, fp32 / w4c / w3g32; bottom: TRM Sudoku-attn, fp32 / w4c / w3c. Past the MLP basin's edge (w3g32) the curve
stops early and the gap widens with depth on the hard bins; on the attention basin's edge (w3c) the curve rises more
slowly and catches up by 512 steps. \running{w8c, w4g32, three noise draws per model; HRM in-basin cells}
\src{EdgeTRM/plots/x1_difficulty_deep_residual.pdf (commit 34c9562); results/breadth/p4d/x1/deep_*.json}}
\label{fig:x1deep}
\end{figure}

\begin{table}[H]
\caption{\textbf{K=512 deep sweep} (p4d; $n$ per residual bin 225 / 246 / 224 / 465 / 640). Accuracy \% at 16 / 64 /
512 steps; gap to fp32 at 512 [95\%]. \src{analyze_difficulty.py deep --axis residual; X1.md}}
\label{tab:x1deep}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Model, quantizer & res 0 & res 1--45 & res 46--50 & res 51--55 & res $\ge$56 \\
\midrule
\inputrows{tables/bank/x1_deep512.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{fp32 keeps scaling to 512 steps}: MLP 76.5 $\to$ 80.9 $\to$ 85.6, attention 76.6 $\to$ 83.3 $\to$ 88.1 at 16 /
  64 / 512 (all 1800 puzzles); the 64$\to$512 gain is on the hard bins (MLP +0.0 / +1.2 / +1.8 / +4.9 / +8.6).
\item \textbf{Past the edge, a cap that widens}: MLP w3g32 ($\varphi$ 0.54) stops improving by $\sim$8 steps; 64$\to$512
  gains +1 to +3 where fp32 gains +5 to +9; gap on res $\ge$56 goes $-23.4$ at 64 to $-29.2$ at 512. Power-law fits (rmse
  0.2--2 points): $\Delta A$ $-3.6$ / $-12.6$ / $-26.4$ / $-32.3$ / $-29.1$.
\item \textbf{On the edge, a tax}: attention w3c ($\varphi$ 0.85) lags 10--17 points at 16 steps on the hard bins; log
  $\tau$ ratio +0.4 to +0.8, $T_{90}$ 1.8--3.2$\times$; common instances solved 1.4--2.2$\times$ later; at 512 within 4.5--5.8
  points on the lower bins and \textbf{+6.7 [+3, +10]} above fp32 on the hardest bin; a 4--5-point shortfall persists only
  on the easiest puzzles.
\item \textbf{At the MLP edge, a small cap}: MLP w4c ($\varphi$ 0.87) $-8.0$ / $-5.6$ at 512 on res 51--55 / $\ge$56 (same
  as at 64: $-7.7$ / $-3.4$); it gains from 64 to 512 about what fp32 gains; common instances take 5--20\% more steps.
\item \textbf{Inside}: attention w4c ($\varphi$ 0.94) within $\pm1$ point in every bin at every depth, common instances
  solved at the same step.
\item \textbf{New cells (X1, Sep 25)}: MLP w4t (out, $\varphi$ 0.28) keeps a third of the singles-only puzzles and nothing else at every depth;
  attention w4t (per-tensor INT4 on the attention edge) lags at 64 ($-8.0$ on res 51--55) and gains more than fp32 from 64 to 512 on the hard
  bins (+8.8 vs +7.1), ending 0.4--6.2 short: a tax plus a small residual cap. \textbf{HRM} fp32 scales too (54.8 $\to$ 60.6 $\to$ 65.3 at 16 /
  64 / 512, on the hard bins); HRM w2g32 (out, $\varphi$ 0.66) has a cap that widens with depth (res 51--55: $-45.4$ at 64 $\to$ $-52.5$ at
  512; +0.2--0.8 gained where fp32 gains +2.4 to +7.3): the past-the-edge regime holds in a second family.
\item K=64 cap/tax fits (Babel): w8c neither; w4g32 a 1.6--2.5-point cap on res $\ge$46, no tax; w4c a 1--5-point cap
  and $\sim$9\% more steps; w3g32 a 15--26-point cap that plateaus \emph{earlier} than fp32 (log $\tau$ $-0.8$ to $-1.0$)
  while kept instances take 1.7--2.7$\times$ more steps; w3a a 13--35-point cap and a slower rate ($T_{90}$ 2--3$\times$).
\item \textbf{Outside the basin, iterating hurts}: Sudoku-MLP weight noise $\sigma{=}0.15$ (one draw, $n_{\text{sup}}\le16$):
  accuracy falls after 2--4 steps (easy 66.9$\to$59.9, medium 32.9$\to$29.3). \running{three draws to 512 steps}
\item \textbf{Exponential vs power-law}: the exponential form fits the 512-step tails poorly (rmse up to 5--6 points; fp32
  still rising roughly as a power of $T$); quote the power-law $A$ and the model-free gap at 512. \open{which form the paper uses}
\end{itemize}

\paragraph{Read-out B summary (X1, EdgeTRM 8e8ac62; p4d, 1800 puzzles to 512 steps; CI at 512 $\pm$0.7--2.5; REWRITE\_NOTES 61).}
The test-time regimes hold on TRM (both mixers) and HRM. \textbf{Inside}, quantizers track fp32 to 512 steps (w8c +0.2 / $-0.3$ / +0.4; attention w4c
+0.1; HRM w4g32 0.0, w4c $-1.8$, w4t $-2.2$). \textbf{Outside}, a plateau with the gap widening on the hardest puzzles (MLP w3g32 $-22.0$ / $-25.8$ /
$-30.8$ at 16 / 64 / 512; HRM w2g32 $-31.6$ / $-37.3$ / $-43.2$; noise at the cliff: MLP $\sigma$0.15 $-43$..$-57$, attention 0.7 $-27$..$-61$, HRM
1.0 $-36$..$-43$). \textbf{On the edge} (attention), lag then catch up (attention w3c $-10.2$ / $-5.7$ / $-0.7$; hard bin $-10.8 \to +2.0$); partial cells:
attention w4t ($-5.4$ / $-5.2$ / $-4.0$) and MLP w4c ($-3.6$ / $-3.6$ / $-4.6$, a small cap). \redtext{Fidelity orders cells within one model; the bands ($\varphi_H\ge0.92$ tracks, 0.85--0.88 lags, $\le$0.76 caps) do not transfer across
mixers (next paragraph).} HRM fp32 scales 54.8 $\to$ 65.3 (16 $\to$ 512). \textbf{Disclosure (required in the paper)}: the difficulty
axis was changed after seeing that the tdoku rating is non-monotone for fp32; the axis used is the number of blanks left after naked and hidden
singles (Spearman with fp32's solve step 0.55--0.58 vs 0.38--0.43 for the rating). \running{22 near-edge cells, p4d cards 2/6/7}

\paragraph{Near-edge regimes, final set: catch-up under fixed (weight) perturbations is attention-only (X1, Sep 25 07:30; EdgeTRM 9ad72c5; $n{=}1800$ per cell, p4d;
REWRITE\_NOTES 73).}
Attention gaps to fp32 at 16 / 64 / 512 steps: w3a ($\varphi$ 0.88) $-5.8$ / $-3.5$ / $+0.2$; w3g32 ($\varphi$ 0.90) $-1.9$ / $-0.5$ / $+0.1$; w4g32 $-0.4$ at 512.
MLP and HRM near-edge cells at $\varphi$ 0.84--0.92 keep constant or widening gaps (three noise draws agree): MLP w5t $-7.4$ / $-9.7$ / $-12.0$, w4a $-2.3$ and
w4g32 $-2.5$ at 512, noise 0.1 $-7.0$ / $-5.2$ / $-4.9$; HRM w3c $-5.3$ / $-5.3$ / $-5.8$, noise 0.5 $-8.1$, noise 0.7 $\times$3 $-17.3$ / $-18.9$ / $-21.6$ at 512
(hard bin $-20$ to $-25$). \textbf{Fidelity orders cells within one model only}; ``three regimes sorted by fidelity'' holds only as ``catch-up holds in the
attention mixer'' for fixed perturbations. \textbf{Fresh activation noise catches up in both mixers} (X1, EdgeTRM 0ea73eb; REWRITE\_NOTES 84): MLP activation noise 0.2
$-7.8$ / $-4.3$ / $-1.8$ at 16 / 64 / 512, the first MLP cell that catches up; attention weight noise 0.5 catches up only partly ($-8.8 \to -5.4$; $-8.0 \to -6.8$). DT mazes:
nothing changes between 500 and 1000 iterations (size 33: w4t 88.4, w3a 95.3, w3c 50.4), so every DT loss is a fixed cap. Reading (with REWRITE\_NOTES 78): a fixed
perturbation of the map leaves a permanent displacement, and more steps help only where the read-out tolerates it; a fresh perturbation averages out over steps. K=64 MLP sweep on p4d (6000 puzzles, fp32 82.0 at 64 steps): w8c 0.0, w4g32 $-1.6$, w4c $-3.1$, w3g32 $-22.1$, w3a $-22.6$, w3c
$-63.4$, w4t $-75.8$, within 0.4 of the Babel run on every spec. \running{7 cells: DT seeds, attention activation noise 0.5, MLP w4g128 and activation
noise 0.2, attention noise 0.5 $\times$3} \src{EdgeTRM 9ad72c5; results/breadth/p4d/x1/; X1.md}

\paragraph{Where failures sit on Sudoku (G link).} Among puzzles fp32 solves, failures rise with fp32's solve step (K=64,
w3g32: 18\% of step-1--2 solves fail vs 76\% of step-33--64; w4c 2\% vs 49\%; even w8c 0\% vs 28\%) and with the singles
residual (w3g32 4$\to$43\%, w4c 0.3$\to$14\%). Opposite of the mazes, where fp32-fast instances were the long-path ones;
with output length nearly fixed (46--64 blanks) failures follow difficulty. \src{analyze_difficulty.py glink}

% ---------------------------------------------------------------------------------------------------
\section{R7. Maze-Hard re-scored: exact match is not correctness (X1)}
\label{r:maze}

Every one of the 1000 Maze-Hard test mazes has more than one shortest path (min 96, median 3.8 million; BFS count);
the reference is a shortest path for all 1000. The scorer accepts all 1000 references and 1000 alternative BFS shortest
paths (947 differ from the reference) and rejects a broken path, a stray cell and an erased wall.
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{TRM Maze-attn} (job 10553031): fp32 exact 87.0, valid-and-shortest 92.5, valid path 99.7; 127 of 130
  exact-match failures (98\%) are valid paths and 55 (42\%) as short as the reference (cf.\ arXiv 2609.26487: 191 / 212
  valid, 75 shortest). Every in-basin quantizer (w8*, w6*, w5*, w4c/a/g32/g128, w3c/a/g32, w4t) within 0.7 points of
  fp32 on ``shortest'' (92.0--92.7). Past the edge the loss is real under every definition: w2a 75.2 ($-17.3$), w2g32
  27.3 ($-65.2$); weight noise 1.0 / 1.5 / 2.0: 91.5 / 76.5 / 0.0; activation noise 0.7 / 1.0 / 1.2: 90.5 / 22.6 / 0.0;
  w3t, w2t, w2c 0. At noise 1.5, 157 of 293 exact failures are invalid paths.
\item \textbf{HRM Maze} (job 10553040): fp32 exact 74.2, valid-and-shortest 81.4, valid path 92.3; of 258 exact failures
  181 (70\%) valid, 72 (28\%) valid and shortest, 63 (24\%) invalid; the composition is unchanged by every quantizer that
  keeps exact accuracy. Noise 1.0 / 1.5 / 2.0: shortest 76.5 / 53.7 / 2.1 (exact 68.7 / 47.2 / 1.7); activation noise 0.7 /
  1.0: 76.1 / 47.0; w2g32 66.8, w3t 72.2, w2a 78.9; w2t, w2c 0.
\item \textbf{Halting head}: see \S\ref{r:halt}. Maze-Unique (EqR) cannot be built from this test set (0 of 1000 mazes have
  a unique shortest path).
\end{itemize}
\src{EdgeTRM/maze_rescore.py, analyze_maze_rescore.py acc|fails|auroc; results/breadth/x1_maze_rescore.json}

% ---------------------------------------------------------------------------------------------------
\section{R8. Mechanism: what sets the edge (X2)}
\label{r:mech}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/contraction_mechanism.pdf}
\caption{\textbf{The edge follows the size of one perturbed step.} (a) Exact accuracy vs weight-noise $\sigma$, three
draws (points) and median (line), $\sigma_{1/2}$ dashed; $n{=}256$ puzzles (Sudoku), 48 (Maze). (b) Median spectral
radius of one recursion step's Jacobian at the final state over the puzzles fp32 solves; diamonds = fp32. Only HRM (and
the maze at its collapse) crosses 1 at its edge; both Sudoku TRMs sit above 1 already in fp32. (c) All 135 perturbed
cells of six models (weight noise, quantizers, single weight groups; black / light grey = DT mazes 33 / 13): fraction of
fp32-solved puzzles still solved against $\delta_T$; the edge sits at $\delta_T\approx0.25$--0.6 in every model.
Babel L40S, torch 2.10, fp32 without TF32; $T{=}16$ (DT: 100 / 300 iterations).
\src{EdgeTRM/figures/contraction_mechanism.pdf (plots/contraction_fig.py, commit 3a82632); results/breadth/babel/x2/contraction_*.json (41 files)}}
\label{fig:mech}
\end{figure}

\begin{table}[H]
\caption{\textbf{Stability of one recursion step at fp32's end state} (medians over puzzles; power iteration with 40
JVPs, checked by ARPACK on 3--5 inputs per model to 3 decimals). Same task, two mixers: the MLP mixer's step has the
larger spectral radius and absorbs random kicks worse while its spectral \emph{norm} is smaller. DT nets end in
2-cycles with $\rho\approx1$. \src{EdgeTRM/results/breadth/x2_contraction_readout.md; x2_contraction_summary.json}}
\label{tab:x2rho}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
Model & Acc & $\rho$ all / solved / unsolved & Solved with $\rho<1$ & FTLE $\Lambda$ solved / unsolved & $\lVert J\rVert_2$ solved & Kick growth (16 steps) & Residual solved \\
\midrule
\inputrows{tables/bank/x2_rho.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[H]
\caption{\textbf{Does the edge sit where the perturbed recursion's spectral radius reaches one?} Yes for HRM, roughly
for the TRM maze, no for the TRM Sudoku solvers ($\rho>1$ in fp32) and the DT nets ($\rho\approx1$ throughout).
Median $\rho$ over fp32-solved puzzles at the $\sigma$ nearest $\sigma_{1/2}$, three draws. \src{X2.md (b)}}
\label{tab:x2edge}
\centering\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Model & $\sigma_{1/2}$ & $\rho$ fp32 & $\rho$ near $\sigma_{1/2}$ & Verdict \\
\midrule
\inputrows{tables/bank/x2_edge.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[H]
\caption{\textbf{Sensitivity sets the width.} $S = \delta_T/\sigma$ at the smallest $\sigma$; $\delta_T$ at $\sigma_{1/2}$
is 0.24--0.59 in every model while $\sigma_{1/2}$ spans $12\times$; $\sigma^* = \delta^*/S$ with $\delta^*$ the geometric
mean of the other models' $\delta_T$ at their edge. On these six models $\log S$ explains 84\% of the variance of $\log\sigma_{1/2}$
(slope fixed at $-1$); \redtext{superseded by the extended fit on 20 models: $R^2$ 0.72 with a family-dependent tolerance (text below).} \src{X2.md; contraction.py --analyze --figdata}}
\label{tab:x2sens}
\centering\footnotesize
\begin{tabular}{@{}llllll@{}}
\toprule
Model & $\sigma_{1/2}$ & $S$ & $\delta_T$ at $\sigma_{1/2}$ & $S\times\sigma_{1/2}$ & $\sigma^*$ \\
\midrule
\inputrows{tables/bank/x2_sens.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Extended sensitivity fit, 20 models (X2, EdgeTRM 519d21e; pre-registered in X2.md; REWRITE\_NOTES 67).} Models: the 6 above
  + HRM Maze + 10 trained Sudoku variants (3 undertrained attention-256 shown, not scored) + MDEQ-Small, MDEQ-XL, DEQ-Transformer. $S$ is stable
  per model (within 5\% across $\sigma$ 0.02--0.1, except TRM-MLP). Width law $\sigma_{1/2} = \delta^*/S$: $R^2(\log)$ \textbf{0.72}, Spearman
  $-0.74$, $\delta^* = 0.35$; the tolerated edge step still spans 5.4$\times$ (0.17--0.89). Held out by family: HRM $\times$1.11, DT $\times$1.25, TRM
  $\times$1.40 (worst $\times$2.38); leave-one-model-out median $\times$1.51. \textbf{It fails to transfer to DEQs} (fit on TRM+HRM: MDEQ-S $\times$0.48,
  MDEQ-XL $\times$0.38, DEQ-T $\times$1.78; MDEQs tolerate 0.70--0.89, DEQ-T 0.19). The earlier ``84\% of variance'' was 6 models; the number to use is
  $R^2$ 0.72 on 20 with a family-dependent tolerance.
\item \textbf{One-step collapse test} (threshold $\delta_T > 0.338$ fixed from TRM+HRM noise widths only; 233 cells): TRM accuracy 0.92 (AUROC
  0.98), HRM 0.96 (1.00), DT 1.00, \textbf{held-out looped LMs 0.92 (AUROC 0.98; per model 1.00; all 7 misses at the threshold)}, DEQ 0.56 (0.82;
  needs its own threshold: MDEQ INT4 holds to 0.48). Wording: width = tolerance / sensitivity; sensitivity carries the mixer and width effects;
  one step-size threshold decides the side in four of five families; the tolerance is family-dependent. \running{6 new mixer seeds}
  \src{EdgeTRM/results/breadth/x2_sens_fit_readout.md; figures/sens_fit.pdf}
\item \textbf{$\delta_T$ orders all 135 cells}: fraction of fp32-solved puzzles still solved is 0.92--1.00 for $\delta_T<0.1$
  (median 0.99, $n{=}32$ cells), median 0.94 for 0.1--0.2 (min 0.78, $n{=}23$), 0.86 for 0.2--0.3, 0.81 for 0.3--0.45,
  0.54 for 0.45--0.6 (range 0.00--0.90, $n{=}22$), 0.08 for 0.6--0.8 (max 0.40), 0.01 above 0.8; Spearman $-0.88$
  ($\varphi_H$ orders them equally well, +0.92). $\delta_T$ needs one step of the perturbed map at fp32's end state instead
  of a full run. MLP vs attention on the same task: $S$ 2.4$\times$ larger for the MLP, and the MLP's $\delta_T$ grows
  faster than linearly ($S$ 1.6 at $\sigma$ 0.02 $\to$ 3.5 at 0.15).
\item \textbf{The MLP model's sensitivity is its token mixer} ($\sigma{=}0.2$, 3 draws; fp32 71.5): noise on the token-mixing
  MLP only $\to$ 4.7 / 5.9 / 7.8 ($\delta_T$ 0.73--0.77; all weights 5.9--9.4, 0.73--0.80); channel MLP only $\to$ 69.9 /
  71.1 / 71.9 ($\delta_T$ 0.17--0.18). Per-tensor INT4 on the mixer only 5.9 (all weights 10.2), channel MLP only 44.9,
  heads only 71.5. The attention model has no single culprit ($\sigma{=}1.0$: attention only 38--49, channel MLP only
  52--54, both 5--16). \caveat{X3's candidate reason, the MLP model's larger residual stream (max 59 vs 11; RMSNorm variance
  range 1673 vs 7.7), is untested in X2}
\item \textbf{How the answer is lost differs by family.} Sudoku (TRM MLP / TRM attn / HRM): a puzzle loses its answer when its
  own perturbed trajectory stops settling; AUROC for ``answer lost'' (cells with 5--95\% lost): FTLE 0.76 / 0.94 / 0.99,
  random-kick growth 0.80 / 0.96 / 0.97, residual 0.79 / 0.97 / 0.99; the puzzle's own $\delta_T$ only 0.63 / 0.51 / 0.53.
  At the TRM edges the fraction of solved puzzles that settle (residual $<$0.1) falls 0.88$\to$0.10--0.21 (MLP) and
  0.85$\to$0.41--0.49 (attention); $\lVert J\rVert_2$ jumps 8.6$\to$71--97 and 13.6$\to$34--68. Mazes (TRM Maze, DT):
  trajectories stay settled through the cliff (TRM Maze residual $\le$0.02, kicks 0.003--0.014 up to $\sigma{=}2.0$);
  instability does not predict which maze is lost (AUROC 0.5--0.6): the fixed point is displaced past the read-out.
\item \textbf{A reference-free warning}: random-kick growth crosses 1 at $\sigma$ 0.11 (MLP; edge 0.14) and 0.63 (attention;
  edge 0.80); none for HRM, Maze, DT, whose kicks stay below 1.
\item \textbf{Cross-seeding (basin identity)}: the fp32 map run 16 steps from the perturbed end state recovers 95--99\% of
  fp32-solved puzzles for TRM Sudoku through the edge (MLP even at $\sigma{=}0.3$ with 1\% accuracy); TRM attention
  switches only past its cliff (30--39\% at 1.0); HRM 7--18\% at $\le$1.0 and 75--87\% at 1.5; TRM Maze $\le$14\%; DT maze
  33 0--50\% at 0.3 and 100\% at 0.5 (DT collapse = basin switch). This is the evidence behind M1.
\item \textbf{Linear response}: where the fp32 resolvent exists ($\rho<1$ along $\delta_T$: HRM 37\%, TRM Maze 79\%, attention
  12\%, MLP 0\% of puzzles) the measured displacement equals $\lVert(I-J)^{-1}\delta_T\rVert$: $R = D/D_{\text{lin}}$ =
  1.00--1.05 inside the basin, 1.1--1.3 at the edge, 1.4 past it. TRM Sudoku small-perturbation displacement is amplified
  3--15$\times$ over $\delta_T$ (w8c 15$\times$) yet the answer holds. Decoder-margin extrapolation over-predicts $\sigma_{1/2}$
  5--13$\times$ (the cliff is not a smooth read-out crossing).
\item \textbf{Path independence} (random initial carry; cells agreeing with the default-init answer): MLP 0.92, attention
  0.66, HRM 0.50, TRM Maze 0.99.
\end{itemize}

\begin{table}[H]
\caption{\textbf{Sudoku-attn weight-noise grid, per draw} ($n{=}256$, puzzles 0--255, $T{=}16$, L40S): accuracy, $\rho(J_T)$
on solved puzzles, fraction with $\Lambda<1$, random-kick growth, residual and basin switch. fp32: 72.7, $\rho$ 1.38 (1.24
solved; 15\% of puzzles below 1). \src{results/breadth/babel/x2/contraction_sudoku_attn_n*.json}}
\label{tab:x2attn}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
$\sigma$ & Acc (\%) & $\rho(J_T)$ solved & Frac.\ $\Lambda<1$ & Kick growth & Residual & Basin switch \\
\midrule
\inputrows{tables/bank/x2_attn.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/contraction_appendix.pdf}
\caption{\textbf{Appendix twin of Figure~\ref{fig:mech}: every model $\times$ metric against $\sigma$.}
\src{EdgeTRM/figures/contraction_appendix.pdf (plots/contraction_appendix.py)}}
\label{fig:mech-app}
\end{figure}

\paragraph{Sentence X2 proposed for the paper.} ``At the edge of every basin one recursion step of the perturbed map moves
the fp32 solution by 25--60\% of its norm; the mixer sets how fast weight noise gets there (sensitivity 2.4$\times$ higher for
the MLP mixer, located in its token-mixing MLP), and that sensitivity alone predicts the basin width within 1.8$\times$ across
six models (12$\times$ range). Whether the edge is a loss of stability depends on the model: HRM's fixed points lose linear
stability there ($\rho\to1$); the TRM Sudoku solvers are not linearly stable even in fp32 ($\rho$ 1.2--1.7) and lose the
answer when their trajectories stop settling; maze solvers keep stable fixed points that are displaced past the read-out.''
The Ingolfsson contraction-vs-drift account does not describe the TRM Sudoku solvers: they are not contractions even in fp32.

\input{sections/results_bank2}


==> sections/results_bank2.tex <==
% Results bank, part 2 (R9-R16).

% ---------------------------------------------------------------------------------------------------
\section{R9. Fidelity: what it predicts, and in what unit}
\label{r:fid}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/fidelity_scatter.pdf}
\caption{\textbf{Fidelity places compressed models on the correct side of the boundary once the unit is the output
cell.} Accuracy retained (\% of fp32) against $\varphi$ for every quantizer and noise cell. (a) TRM and HRM (each cell
paired with fp32 at its own $H$): the 0.85 line classifies 217 of 225 cells (96\%) by ``retained $\ge$90\%''. (b)
Deep-thinking networks: 323 of 353 by exact match (92\%; every miss at $\varphi\ge0.86$ with exact accuracy 2--89\%, where DT exact match falls with path length while
per-cell accuracy holds; an onset-hazard effect, not independent cell errors) and 16 of 18 maze cells by per-cell accuracy (filled; the two misses are collapsed noise draws
at $\varphi$ 0.85 / 0.82 keeping 93\% / 90\% of cells while exact match keeps 21\% / 4\%).
\src{EdgeTRM/figures/fidelity_scatter.pdf (plots/fidelity_scatter.py, HRM H-fix 6aa9c3c); results/breadth/*.json}}
\label{fig:fid}
\end{figure}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Definition as the harness computes it}: one cosine between the flattened final $z_H$ of the compressed and
  fp32 models per input, averaged over inputs (\texttt{breadth\_sweep.py fidelity()}; Eq.~\ref{eq:fidelity}). The Sep 13
  draft's per-token equation did not match the numbers (REWRITE\_NOTES 21).
\item \textbf{The unit is the cell.} On the convnets in-basin quantizers keep per-cell accuracy at 99.5--100\% while exact
  match drops up to 12 points (size 33 at 300 iterations: w4t exact 87.6, cell 99.9 all / 99.5 target, $\varphi$ 0.987;
  w3a 95.3 with 100.0 / 100.0, $\varphi$ 0.980); the one collapsed noise draw ($\sigma{=}0.3$ seed 0) is a per-cell collapse
  (cell 90.5, exact 4.0) at $\varphi$ 0.817. TRM Maze under activation noise 1.0: cell 99.4, exact 24.6, $\varphi_H$ 0.915.
  Masking the cosine to the path (Q2) lowers violators' median $\varphi$ from 0.949 to 0.905--0.910 (intact cells 0.992)
  but does not rescue the band; the unit does.
\item \textbf{Correction (X8 final, REWRITE\_NOTES 39): the cell-independence model fails on every TRM/HRM task.} Schaeffer et
  al.'s product model, exact $\approx$ mean$_i\,p_{\text{cell}}^{L_i}$, predicts $<$1\% exact match for fp32 in almost every
  length quartile of all five TRM/HRM models (worst case 14\%, one TRM-maze quartile) where 29--91\% is observed. Wrong answers
  are wholesale, not a few independent flips: a wrong Sudoku grid has a median of 29--34 wrong cells (of 46--64 blanks) at
  every precision; a wrong maze a median of 26--30 (a different path; 21--24 at 2 bits). Exact match does not fall with output
  length inside a task (TRM Maze fp32 by path-length quartile 84 / 87 / 91 / 85; HRM Maze 72 / 76 / 75 / 74); on Sudoku it falls
  with the number of blanks (75$\to$66 MLP, 72$\to$29 HRM), i.e.\ with difficulty. The one near-miss regime is TRM-maze activation
  noise at $\sigma$1.0 (exact 22.6, cell 99.4, median 2 wrong cells per wrong maze), where the product model still predicts 0.3\%.
  \textbf{Every ``exact match compounds a small per-cell risk'' or ``multiplies independent per-cell errors'' statement is withdrawn
  for TRM/HRM.} What stays: fidelity certifies per-cell agreement, and one threshold in the cell unit works across output lengths
  (Table~\ref{tab:x8filter}). The deep-thinking-maze length dependence is an empirical fact about those models, fitted by an
  onset-hazard model $(1-h)^L$ whose $h$ is 1/40 of the per-cell error (\S\ref{r:tts-dt}): not independent cells either.
  \src{EdgeTRM/analyze_x8.py indep; X8.md D part 2}
\end{itemize}

\begin{table}[H]
\caption{\textbf{Fidelity is a filter, not a ranker} (X8 D part 1). Spearman($\varphi$, accuracy retained) with 95\%
bootstrap intervals over cells, for all cells, in-basin cells (retained $\ge$0.9), near-baseline cells ($\ge$0.97, count in
parentheses) and near-baseline cells at 16 steps only. Every Sep 13--23 breadth record at the default $H$, $n_{\text{sup}}$
1--64, 23 weight quantizers, weight noise and activation noise; $n{=}1000$ per cell (500 for the Babel activation-noise maze
file). \src{EdgeTRM/analyze_x8.py fid; X8.md}}
\label{tab:x8spear}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
Model & Cells & In-basin & All & In-basin (ret.\ $\ge$0.9) & Near-baseline ($\ge$0.97) & 16 steps, near-baseline \\
\midrule
\inputrows{tables/bank/x8_spearman.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[H]
\caption{\textbf{One threshold works once the unit is the cell.} AUROC of $\varphi$ for ``damaged'' (exact retained $<$0.9;
cell unit: per-cell accuracy retained $<$0.99), best threshold and its balanced accuracy, and the balanced accuracy of one
global threshold $t{=}0.893$. Against exact match the threshold climbs with output length (0.85 at 81 cells, 0.97--0.98 at
900); against the cell, 0.89 works everywhere. \caveat{per-model thresholds still differ within an output length (Sudoku
0.83 / 0.87 / 0.93; maze 0.95 TRM vs 0.99 HRM); the DT per-cell reruns are small (6 damaged cells each)}
\src{EdgeTRM/analyze_x8.py fid; X8.md}}
\label{tab:x8filter}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Group (output length) & Cells & Exact unit: AUROC, best $t$, bal.\ acc. & Exact unit, $t{=}0.893$ & Cell unit: AUROC, best $t$, bal.\ acc. & Cell unit, $t{=}0.893$ \\
\midrule
\inputrows{tables/bank/x8_filter.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Out-of-family validation (X8, \texttt{analyze\_x8.py oof}; REWRITE\_NOTES 59).} Thresholds fitted on 1146 TRM/HRM cells only (exact unit
  0.874, cell unit 0.893, collapse 0.828), applied unchanged. \textbf{As a collapse detector it transfers}: misses 0/28 collapsed looped-LM cells,
  0/120 DEQ-Transformer, 0/279 MDEQ, 0/51 Q7-final, 3/163 Q8, at the cost of false alarms in families that degrade gracefully (MDEQ keeps $\ge$50\%
  down to cosine $\sim$0.69); it breaks on DT mazes (23 collapsed cells keep whole-map cosine $\ge$0.874: the long-output problem). \textbf{As a
  10\%-loss release threshold it needs one per family} (balanced accuracy MDEQ 0.93, DEQ-T and variants 0.82--0.86, looped LMs 0.76, DT mazes 0.63;
  family-optimal $t$ 0.74--0.975). Scope for the paper: fidelity is a cross-family collapse detector, not a universal quality threshold.
\item \textbf{Per input, fidelity is weak}: reference fidelity as a per-puzzle wrong-answer detector 0.95 on Sudoku-MLP
  w8c/w4c but 0.36--0.76 on Sudoku-attn and $\le$0.63 on mazes (Table~\ref{tab:auroc}); the halting head is better per
  puzzle.
\item \textbf{The map-level counterpart}: $\delta_T$ (one perturbed step) orders cells with Spearman $-0.88$ vs $\varphi_H$ +0.92
  (\S\ref{r:mech}); it costs one step instead of a full run.
\item \textbf{Other families}: DEQ accuracy tracks the cosine to the fp32 equilibrium ($\ge$0.92$\to\ge$92\% retained;
  0.85$\to$78--83\%; 0.78$\to$64--72\%; 0.61--0.62$\to$14--25\%; $\le$0.54$\to$0) for noise and quantizers alike
  (\S\ref{r:transfer}); looped LMs: fidelity gap at $\sim$0.8 over 92 cells (\S\ref{r:lm}).
\item \textbf{Operator generality untested}: low-rank / SVD truncation at matched $\varphi$ (lit 05 D-3). \pending{not scheduled}
\end{itemize}

% ---------------------------------------------------------------------------------------------------
\section{R10. The halting head and other label-free detectors}
\label{r:halt}

\begin{table}[H]
\caption{\textbf{AUROC for a wrong answer at supervision step 16}: halting head / convergence residual / fidelity to fp32
(reference-based); accuracy in parentheses. Sep 23 read (Q3). The head separates right from wrong on Sudoku at every precision inside the
basin and stays at 0.81 at 6\% accuracy (w4t); on mazes it reads 0.63--0.76 against \emph{exact match}, which the maze
re-scoring explains (text). $n{=}1000$. Superseded in detail by the X8 final tables below. \src{EdgeTRM/tables/tab_auroc_rows.tex (plots/auroc_table.py); results/breadth/{p4d,babel}/residual_*.json}}
\label{tab:auroc}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l lllll@{}}
\toprule
& TRM Sudoku, MLP & TRM Sudoku, attn & TRM Maze & HRM Sudoku & HRM Maze \\
\midrule
\inputrows{tables/tab_auroc_rows.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Early warning: dropped.} \redtext{The Sep 23 statement ``the head is 1.00 at step 2'' measured the step-2 answer, not the
  final one, and is withdrawn.} Predicting the step-16 answer's wrongness from step $k$ (X8 final): the head reaches AUROC 0.72--0.80 at
  $k{=}1$, 0.81--0.84 at 2, 0.90--0.92 at 4, 0.97 at 8, and the hand-coded checker applied to the step-$k$ answer tracks it within
  0.02--0.07 at every $k$ (HRM $k{=}1$: head 0.80, checker 0.73). The head verifies the current answer with at most a small look-ahead
  (HRM); it is not an early-warning oracle.
\item \textbf{The defer rule, set once and applied unchanged (X8 final; 88 Sudoku cells, 3 models, $n{=}1000$ each; weight and
  activation noise as 3 draws).} The model's own rule sigmoid$(q){>}0.5$, never recalibrated:
  \emph{in the basin} (43 cells, incl.\ 3-bit HRM, 4-bit TRM, +a8, noise draws) selective risk $\le$0.7\% and $\ge$99\% of correct answers
  kept in every cell of every model; \emph{at the edge} Sudoku-attn and HRM keep 99--100\% of correct answers at risk 0--7.2\% (worst:
  HRM noise 1.0 draw s1, 7.2\%; attn noise 0.7 s2, 5.3\%), and TRM-MLP fails safe (keeps 6--44\%: w3g32 6\%, w3a 44\%, noise 0.15 35--43\%,
  activation noise 0.3 $\sim$20\%, at risk $\le$3.4\%); \emph{out of the basin} it breaks model by model (21--92\% risk: Sudoku-attn weight
  noise 1.0 accepts 1--24\% with 28--92\% wrong; HRM 2-bit accepts 16--18\% with 21--26\% wrong; TRM-MLP accepts almost nothing, w3c 1\% at
  62\% wrong). A threshold calibrated on fp32 to 1\% risk is fragile inside the basin (Sudoku-attn w3c 11\%, w4t 6\%, noise 0.5 4--7\%):
  fp32 is nearly separable (mean $q$ +7 correct, $-$11 wrong), so the calibrated point sits on the wrong cluster's edge and compression
  shifts that cluster up by 1--2 logits; the gap midpoint is as robust as the native rule. The head's \emph{ranking} survives where its
  threshold drifts: at the MLP edge (w3g32, AUROC 0.99) best-of-16 by argmax $q$ is within 0.7 points of the oracle.
  \src{Babel breadth_results/x8/det_{sudoku_mlp,sudoku_attn,hrm_sudoku}__{A,B,C}.json; EdgeTRM a414568; analyze_x8.py select|basin}
\item \textbf{What the head is}: among wrong answers its logit tracks the conflict count (Spearman$(q,-\text{conflicts})$ 0.55--0.78 in the
  basin, all three models) and not the number of wrong cells ($-0.13$ to 0.21): a learned, graded constraint checker.
\item \textbf{$\varphi$ filter + defer rule together (the release-check combination)}: the $\varphi$ filter with per-length thresholds fitted on
  the Sep 13--23 records (0.845 for 81-cell outputs; independent of these runs) passes 47 of 88 Sudoku cells (40 in basin, 7 edge, 0 out); in
  every passed cell the native defer rule has risk $\le$0.7\% and keeps $\ge$99.1\% of correct answers. The 41 flagged cells contain every
  out-of-basin cell and every cell where the rule broke (plus 3 in-basin false alarms: MLP +a8 at $\varphi$ 0.80--0.84, attn w3c 0.83). On
  mazes (threshold 0.981) it passes 11 TRM and 10 HRM cells, all in basin, with valid-path defer risk $\le$0.4\% (TRM) and $\le$3.8\% (HRM;
  fp32 itself 2.7\%), and flags every edge and out-of-basin maze cell. In total 68 cells pass, none out of the basin.
\item \textbf{Baselines}: the hand-coded Sudoku checker is exact (AUROC 1.00 everywhere; unique solutions); min-over-blanks
  max-softmax matches the head (0.99--1.00 in basin) and stays better outside it on TRM-MLP (w3c 1.00 vs 0.87; w4t 0.98 vs
  0.80); on HRM 2-bit both break at fixed thresholds. Path independence from a random carry: TRM-MLP reproduces 93\% of
  its correct answers and none of its wrong ones (AUROC 0.94); TRM-attn and HRM mostly fail from that carry (20\% / 2\%),
  uninformative (0.50).
\item \textbf{Mazes (X8 final, 27 + 27 cells, $n{=}1000$)}: of TRM Maze fp32's 130 exact failures, 55 are alternative shortest paths, 72
  valid but longer, 3 invalid; HRM Maze fp32's 258: 72 / 109 / 77 (X1's ``63 invalid'' does not add up; $258-181=77$). The hand-coded
  path checker reaches 0.77--0.81 (TRM) / 0.84--0.90 (HRM) for exact match, the ceiling of any label-free signal. HRM's head is a validity
  verifier at every precision (``not a valid path'' 0.92 fp32; 0.89--0.94 in basin, 0.88--0.96 edge, 0.93--0.98 out); nothing label-free
  separates the reference from an alternative shortest path (0.46--0.72). Max-softmax is useless on TRM mazes (0.50--0.58 exact). Defer
  rule, valid-path definition: TRM in basin 0.2--2.5\% risk at 97--100\% coverage; HRM fp32 2.7\%, in basin 2.0--5.8\%, edge 10--29\%, out
  13--95\%; under exact match the rule defers nothing useful (the head fires on valid alternatives).
\item \textbf{Mazes, re-scored} (X1): HRM's head gives AUROC 0.67 (exact) and 0.69 (shortest) but \textbf{0.93 for ``not a
  valid path''} under fp32; 0.91--0.94 for every in-basin quantizer, 0.96 for w2g32, 0.88--0.95 under noise. TRM: 0.69 /
  0.72; for ``invalid'' 0.67 under fp32 with only 3 invalid answers in 1000 (uninformative), and where compression produces
  invalid answers the head flags them (w4t 0.86, w3c 0.83, noise 1.0 0.91, w2a 0.93). Among exact-match failures neither
  head separates shortest from longer valid paths (0.56--0.64). The maze head is a validity verifier, not an optimality
  verifier. \src{analyze_maze_rescore.py auroc}
\item X8 is complete except one PTRM cell (Sudoku-MLP activation noise $\sigma$1.0).
\end{itemize}

\begin{table}[H]
\caption{\textbf{Detectors ranked on Sudoku (X8 final, 88 cells)}: AUROC for a wrong answer (Hanley--McNeil CIs $\pm$0.00--0.02). Class by
exact accuracy retained: in $\ge$0.9 (43 cells), edge 0.3--0.9 (26), out $<$0.3 (19, three all-wrong without AUROC). On Sudoku the head adds
nothing to the checker and little to max-softmax. \src{EdgeTRM/analyze_x8.py auroc; X8.md}}
\label{tab:x8rank}
\centering\footnotesize
\begin{tabular}{@{}p{0.34\textwidth}p{0.17\textwidth}p{0.17\textwidth}p{0.24\textwidth}@{}}
\toprule
Detector & In basin & Edge & Out of basin \\
\midrule
\inputrows{tables/bank/x8_rank.tex}
\bottomrule
\end{tabular}
\end{table}

\paragraph{PTRM reconciliation (X8 final).} PTRM \citep{sghaier2026ptrm} perturbs the carried latent once per supervision step
($z_L \mathrel{+}= \mathcal N(0,\sigma^2 I)$) and keeps the best of $K$ rollouts by the halting head; it never reports a single noisy rollout.
On our checkpoints that kick costs a single rollout nothing at any $\sigma$ up to 1.0 (Sudoku-MLP 71.2--71.5 vs 70.5 deterministic;
Sudoku-attn 66.4--66.7 vs 65.9; maze 87.9--88.4 vs 88.4), and on Sudoku the head picks the best rollout every time (best-Q@16 = pass@16,
+10 points), also on a 4-bit model (+10.4) and a 3-bit model at the basin edge (+14.5, 0.7 below the oracle) where the head's absolute
threshold has already failed. Our activation noise perturbs the map at every one of the 170 linear inputs of a Sudoku supervision step
(21 recursion calls $\times$ 8 linears + 2 heads; 122 on the maze TRM). At the same $\sigma$ a single rollout collapses (Sudoku-MLP 69.7 /
32.1 / 2.3 at $\sigma$ 0.1 / 0.3 / 0.5; Sudoku-attn 64.1 / 45.2 / 0 at 0.3 / 0.5 / 1.0; maze 88.1 / 23.4 at 0.5 / 1.0), and best-of-16 helps
only inside or at the edge of the basin (MLP $\sigma$0.3: 32$\to$53; attn $\sigma$0.5: 45$\to$58) and not beyond it (pass@16 5\% and 0\%). On
the maze the head cannot select ($\sigma$1.0: pass@8 78, best-Q@8 29, majority 59), as PTRM report. A kick to the state inside the basin
is contracted away within the step and only moves borderline puzzles between attractors, which the head exploits; a perturbation of the
map on every call moves the model out of its basin, and no selection rule recovers answers no rollout reaches.
\running{Sudoku-MLP activation noise at $\sigma$1.0}

\begin{table}[H]
\caption{\textbf{PTRM's latent kick vs our per-linear activation noise} (Babel L40S, $D{=}16$, $n{=}1000$ Sudoku / 500 mazes; single = mean
of one noisy rollout). \src{EdgeTRM/analyze_x8.py ptrm; Babel breadth_results/x8/ptrm_*.json}}
\label{tab:x8ptrm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
Model (deterministic acc) & Noise & $\sigma$ & Single rollout & pass@$K$ & best-Q@$K$ & mode@$K$ \\
\midrule
\inputrows{tables/bank/x8_ptrm.tex}
\bottomrule
\end{tabular}}
\end{table}

% ---------------------------------------------------------------------------------------------------
\section{R11. Looped language models (X4)}
\label{r:lm}

\begin{table}[H]
\caption{\textbf{Ouro at 4 loops, GSM8K test[:200], 512 new tokens} (p4d, transformers 4.55.4): latent fidelity to bf16,
teacher-forced gold NLL (bf16 in parentheses), $\Delta$NLL, top-1 agreement with bf16, greedy accuracy (bf16) and accuracy
retained. Per-channel INT4 sits inside Ouro-2.6B's basin and outside Ouro-1.4B's; per-tensor INT4 outside both.
\src{EdgeTRM/analyze_looped.py boundary; results/looped/p4d/q6/}}
\label{tab:x4}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
Model, 4 loops & Fidelity & Gold NLL (bf16) & $\Delta$NLL & Top-1 agree & Greedy acc (bf16) & Retained \\
\midrule
\inputrows{tables/bank/x4_boundary.tex}
\bottomrule
\end{tabular}}
\end{table}

\paragraph{All 92 looped-LM cells with generation data} (Huginn-0125, Ouro-1.4B, Ouro-2.6B; every loop count; 16 weight
formats; retained = greedy GSM8K / bf16 at the same loops; collapse = retained $<$50\%; cells with bf16 $<$10\% excluded):
64 hold, 28 collapse. \textbf{Latent fidelity separates with a gap}: every collapsed cell $\le$0.784 (Huginn w3a), every held
cell $\ge$0.807 (Ouro-2.6B w4c at 2 loops, keeps 77\%); AUROC 1.000; the gap sits where the TRM/HRM activation-noise cliff
sits. \textbf{Teacher-forced NLL ranks almost as well but has no threshold}: relative $\Delta$NLL AUROC 0.997, absolute 0.982
(0.960 among the 77 cells with fidelity $\ge$0.5), yet collapsed cells start at +16\% / +0.137 nats (Huginn w3a at 64 steps)
while held cells reach +20\% / +0.364 nats (Ouro-1.4B w8t at 1 loop, keeps 59\%). A deployer reading +0.14 nats would ship
Huginn w3a (keeps 15\%). \caveat{the 50\% cut is a choice (the ordering does not depend on it); three models, two families;
the Lambda cells ran on a different transformers version (two cells rerun on p4d match: 0.736 / 0.853); $n$ = 50--200 per
cell} \src{analyze_looped.py boundary; Sep 13--15 Lambda grid + p4d}

\paragraph{Third looped model: Recurrent-OLMo-2 (retrofitted recurrence, 1.36B; X4, Sep 25 00:15 UTC).} 2-shot GSM8K, greedy, 512 new
tokens, $n{=}100$ per cell (Wilson half-width $\sim\pm$10 points); teacher-forced sweep $n{=}200$. Loop count changes neither fidelity nor
retention (w4c keeps 70 / 84 / 80 / 90\% at 4 / 8 / 16 / 32 loops with $\varphi$ constant). All 20 generation cells fall on the correct side
of the Huginn/Ouro threshold (held: $\varphi$ 0.942--1.000, 70--116\% retained; collapsed: w4t $\varphi$ 0.11, 0\%). \textbf{Pooled over 109
cells the gap holds}: collapsed max 0.784, held min 0.807, AUROC 1.000; relative $\Delta$NLL AUROC 0.998 with overlapping ranges.
Teacher-forced only: w4a $\varphi$ 0.96, $\Delta$NLL +0.05; w3a $\varphi$ 0.76--0.79, NLL 1.58--1.70 vs 0.77 (+0.8 nats), KL 0.80--0.92.
\textbf{The decisive cell landed: looped LMs share the $\sim$0.8 threshold} (X4, EdgeTRM 67826cd; p4d, own bf16 references; REWRITE\_NOTES 85). OLMo w3a:
$\varphi$ 0.760 / 0.785 / 0.790 at 4 / 8 / 32 loops; greedy 2.0 / 5.0 / 2.0\% vs bf16 44 / 44 / 42.5 ($n$ = 100 / 100 / 200), 2--11\% retained. Teacher-forced NLL rises
only +0.80--0.90 nats, and gold-answer likelihood ranking still gets 39--83\%. The w4a control ($\varphi$ 0.96) holds at 68--86\% retained. \textbf{Pooled over
4 models and 118 cells: AUROC 1.000, collapsed max 0.790, held min 0.807} \redtext{(a narrow gap; its exact location is not pinned down; band cells are
queued).}
\src{EdgeTRM/results/looped/p4d/olmo/olmo_rec32_*; EdgeTRM 3de9866; analyze_looped.py sweep boundary}

\begin{table}[H]
\caption{\textbf{Recurrent-OLMo-2 on GSM8K by loop count} (accuracy \%, $n{=}100$; $\varphi$ and $\Delta$NLL where measured; teacher-forced
KL(bf16$\|$q): w4g32 0.02, w4c 0.09, w4t 9.6). \src{X4.md ``Third looped model''}}
\label{tab:x4olmo}
\centering\footnotesize
\begin{tabular}{@{}llllll@{}}
\toprule
Loops & bf16 & w8c & w4g32 & w4c & w4t \\
\midrule
\inputrows{tables/bank/x4_olmo.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Decoding controls do not rescue Ouro-1.4B w4c} (4 loops, $n{=}200$): accuracy [95\% Wilson CI],
degenerate / loop / capped rates. Repetition controls cut the degenerate rate (86.5$\to$9.0) but recover at most 15 of the
70.5-point gap and wreck bf16 at strength. 138 of 200 w4c greedy outputs open by echoing the system prompt (bf16 0 of 200);
the first generated character differs from bf16 on every problem. \src{analyze_looped.py q6; X4.md}}
\label{tab:x4q6}
\centering\footnotesize
\begin{tabular}{@{}lllll@{}}
\toprule
Decode & bf16 acc & w4c acc [95\% CI] & w4c degenerate / loop / capped & w4t acc \\
\midrule
\inputrows{tables/bank/x4_q6.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Looped LMs across loop counts and formats} (master Table E, Sep 13--15 Lambda grid): GSM8K greedy
accuracy \% [$n$], teacher-forced NLL and latent fidelity $\varphi$. Huginn's depth is flat under compression; no looped LM in
full precision gains past its training depth (Ouro peaks at 2--4 loops). \src{reports/EDGETRM_MASTER_TABLES.md E; results/breadth/huginn_gsm8k_*.json, ouro_*.json}}
\label{tab:mtE}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l llllllll@{}}
\toprule
Model, depth & bf16 & w8c & w6c & w4g32 & w4c & w4a & w4t & w3a \\
\midrule
\inputrows{tables/bank/mt_E.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item Ouro-2.6B, 4 loops: greedy bf16 82.5, w4c 77.5 (degenerate 11.5), w4t 0.0 (NLL 12.7: destroyed; no decoding can help).
\item Steven's decision (Sep 24 $\sim$22:40): generators follow the same boundary; the third paper F folds into ICLR.
\item \textbf{Huginn Q6} (Babel, $n{=}200$): bf16 38.0, w3a 3.5, w4t 2.0, w4c 31.0; no decoding control lifts w3a above 5.5. \textbf{Ouro-1.4B w4c with
  oracle bf16 prefixes} of 1 / 8 / 32 tokens: 19.5 / 22.5 / 29.5 (greedy 7.5, bf16 78.0): the start is not the whole failure. At $n{=}500$: Ouro-1.4B bf16 76.6,
  w4c 8.6, w8c 76.0; Ouro-2.6B bf16 83.0, w4c 76.8. \src{X4.md; EdgeTRM 67826cd}
\item \running{fidelity-band cells (0.75--0.90) to pin the threshold; KL for Ouro-2.6B}
\item \caveat{Ouro degrades past $T{=}4$ in full precision and has no fixed point (lit 03); the OLMo retrofit (flat in loop count in
  full precision) now supplies the full-precision-stable looped generator; its decisive w3a cell collapses at $\varphi$ 0.76--0.79, as the threshold predicts. Angle I needs a scope sentence: looped
  LMs' KV cache grows with loop count.}
\end{itemize}

% ---------------------------------------------------------------------------------------------------
\section{R12. Can the basin be trained? QAT and regularisers (X5; M6)}
\label{r:qat}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Recipe verified} (TRM-MLP w256; p4d, seeded 1000-puzzle training build): at step 6,510, fp32 12.0 / 15.1 / 12.9
  and w4t 6.9 / 9.7 / 9.0 (fidelity 0.96) vs the Lambda runs 12.3 / 12.4 / 11.7 and 7.7 / 7.9 / 6.7; step 13,020 seed 0: fp32
  25.9, w4t 19.5 (0.917) vs Lambda 24.3--28.7 and 11.7--14.6. The evaluation harness reproduces the Lambda finals exactly
  (fp32 59.9 / 62.3 / 64.0; w4t 0.0 / 0.0 / 0.0 with fidelity 0.220 / 0.154 / 0.209; attention w512 s0 fp32 64.8, w4t 65.5).
  MLP s0 noise cliff, three draws: $\sigma$0.1 49.3 / 47.3 / 48.3; 0.15 24.2 / 28.0 / 25.4; 0.2 3.3 / 2.5 / 4.2
  ($\sigma_{1/2}\approx0.14$). \src{results/q7/lambda_finals/; X5.md}
\item \textbf{Naive per-tensor INT4 QAT repairs the collapse} (12k steps from the Lambda finals, STE, AdamW lr 1e-4): endpoints
  w4t \textbf{52.3 / 61.2 / 56.4} for seeds 0 / 1 / 2 (mean 56.6; start fp32 59.9 / 62.3 / 64.0, w4t 0.0, i.e.\ 87 / 98 / 88\% of
  fp32), latent fp32 0.0 / 2.1 / 9.9; intermediate w4t 44.3 / 57.5 / 50.3 at 3k steps, 48.9 / -- / 54.5 at 9k. The latent fp32 weights collapse (0.0--5.2; s2 15.0 at 9k): QAT moves the model to a point where
  only the quantized weights work, so fidelity must be measured against the starting fp32 model (0.80 for s0 at 3k on a
  40-puzzle check). Consistent with Ingolfsson et al.\ (naive Int4 QAT 71.8, weight-LSQ 81.1 on their Sudoku, W+A);
  our own earlier claim ``QAT cannot repair it'' is withdrawn. Ingolfsson et al.\ reach 71.8 of 84.1 (85\%) for W+A. \src{p4d:q7/ckpt/qat_naive_s{0,1,2}/eval_step_12000.json}
\item \textbf{Base trajectory on the same host} (fp32 / w4t / w4t fidelity): step 19,530 s0 38.5 / 23.1 / 0.830, s1 45.4 / 18.0 /
  0.717, s2 42.6 / 30.0 / 0.863; step 26,040 s0 45.0 / 17.2 / 0.773, s1 58.3 / 15.7 / 0.748, s2 54.7 / 21.1 / 0.793 (fragility
  forming, as in master Table F). $S$ implementation checked against X2: released TRM Sudoku-MLP $S_{0.02}$ = 1.63 (X2: 1.60);
  Lambda w256 s0 final $S_{0.02}$ 1.25, $S_{0.1}$ 1.28.
\item \textbf{QAT roughly doubles basin width around its deployed INT4 point, by lowering $S$} (X5; REWRITE\_NOTES 66): seeds 0 / 1, 12k steps,
  $n{=}1000$, 3 draws, noise on top of the per-tensor INT4 weights: $\sigma_{1/2}$ 0.28 / 0.30 vs $\sim$0.14 for the fp32 models (seed 0: 49.5 / 45.3 /
  41.2 / 22 at $\sigma$ 0.1 / 0.15 / 0.2 / 0.3; fp32 at 0.2 keeps 2.5--4.2); $S$ around the quantized weights 0.84 / 1.12 vs 1.28 / 2.10 for the fp32
  finals, as the mechanism predicts; w4t fidelity to the starting fp32 0.841 / 0.871. \redtext{Control pending: an fp32 fine-tune for the same 12k steps
  (does fine-tuning alone widen it?). The sensitivity-penalty hinge at $S^*{=}0.7$ held $S\approx0.6$ but fp32 fell to 10--13\% (applied at early
  recursion states where the map must move); retrying on carries $\ge$8 ACT steps. Maze-MLP w512/w1024 diagnostics running.}
\item \textbf{$S$ separates the mixers on the trained variants} (256 puzzles, 3 draws): MLP w256 s0/s1/s2 $S_{0.02}$ = 1.25 / 2.04 / 1.28;
  attention w512 s0/s1 0.70 / 0.82 (MLP 1.5--2.9$\times$ more sensitive); $\lVert J\rVert_F^2/\text{dim}$ goes the other way (0.14--0.20 vs
  0.23--0.26). This is the quantity the \texttt{sens} penalty targets. \src{p4d:q7/ckpt/lambda_*/eval_step_65100.json}
\item \redtext{\textbf{M6 fine-tune arms (Sep 25 00:20; p4d cards 3--4, card 5 to M1)}: 12k steps from the Lambda w256 finals, the QAT
  protocol: \texttt{sensft\_s*} (sensitivity penalty, $\lambda$ 0.5, $\sigma_p$ 0.1) and \texttt{gqatft\_s*} (per-tensor INT4 introduced by a
  homotopy over 6,000 steps, then QAT) against \texttt{qat\_naive\_s*} (abrupt) and \texttt{ft\_fp32\_s*} (no compression). Endpoints expected
  Sep 25 $\sim$02:30 (sensft s0/s1) to $\sim$11:00 (last). No M6 endpoint exists yet; smoke runs trained cleanly (penalty's $S$ at random
  init 12.8 vs $\sim$1.3 trained).}
\item \textbf{M6 arms added Sep 24 23:30} (p4d cards 3--5): sensitivity penalty \texttt{sens} (penalise $\delta/\sigma_p$ of one full
  ACT step under fresh weight noise at the training-time end state; last 20\%, forked at 52,080; $\lambda$ 0.5 / 2 / 0.1); in-training
  compression \texttt{gqat} (per-tensor INT4 introduced by a homotopy $W + a(Q(W)-W)$, $a$ ramped 0$\to$1 from 20\% to 60\% of
  training, then QAT; CompreSSM's lesson) with a late-and-gradual control. \running{fine-tune endpoints first (Sep 25 02:30--11:00); then lsens forks,
  full gqat runs, other forks, W+A bridge, noise and Jacobian arms (Sep 25--26); q7\_base\_s2 paused behind the fine-tunes}
\item \running{QAT endpoints s1/s2 with the reference-fidelity rescan; weight-LSQ; fp32 fine-tune control; W+A bridge (static
  per-tensor INT4 activations) $\sim$08:30 Sep 25; late-phase forks (QAT / clip / noise) $\sim$10:00; noise injection
  throughout $\sim$17:30; Jacobian penalty and extras Sep 25 20:00 -- Sep 26 05:00; M6 adds a $\delta_T$ penalty and a
  CompreSSM-style arm}
\item Prediction under test (arm a): a Jacobian penalty will not widen the MLP basin, since the attention mixer already has the
  larger one-step Jacobian (\S\ref{r:mixer}). If the noise cliff stays at 0.15--0.2 under every regulariser, the mixer fixes
  the basin.
\end{itemize}

% ---------------------------------------------------------------------------------------------------
\section{R13. Transfer to DEQs and diffusion (X6, final)}
\label{r:transfer}

\paragraph{Summary (X6 final, EdgeTRM 9b90e44; REWRITE\_NOTES 53).} The boundary transfers, as a \emph{fidelity} boundary, to all three
published DEQs and to the stochastic diffusion sampler: a flat plateau, a steep edge, collapse; quantizers sit on the noise curve at their
relative weight error. \textbf{Extra solver iterations never help past saturation, and outside the basin they give nothing (MDEQ) or make it
worse} (DEQ-Transformer at $\sigma$0.7: perplexity 923 $\to$ 1182 from 10 to 60 iterations). \textbf{The residual does not flag collapse}: the
solvers converge as well or better on broken models (MDEQ-Small: $\ge$99.4\% of images below $10^{-2}$ at every $\sigma$, collapsed w4t fastest;
DEQ-Transformer w4t's residual is 500$\times$ \emph{below} fp32's; per-image AUROC 0.42--0.67). The collapse is a \textbf{displaced equilibrium},
tracked by the cosine to the fp32 equilibrium, with the drop below $\sim$0.8, the TRM band (aggregate only; per image AUROC $\le$0.67).
\textbf{Scope}: ancestral DDPM (fresh noise each step) shows the basin with a step-flat cost, while deterministic DDIM compounds with steps
($\sigma$0.05: FID vs fp32 46 $\to$ 190 from 10 to 100 steps; w4g32 40 $\to$ 304). Accumulation is real for a deterministic, non-contracting
iteration; the boundary claim is for fixed-point iterations.

\begin{table}[H]
\caption{\textbf{MDEQ-Small on ImageNet has a plateau, an edge and a cliff, and its solver never notices.} Broyden top-1 \%
by iteration budget $k$ (26 = default), cosine to the fp32 equilibrium, fraction converged (residual $<10^{-2}$) at $k{=}100$
and median steps to $10^{-2}$; noise rows mean [min, max] over 3 directions; quantizer rows give the mean relative weight error,
which places each quantizer on the noise curve. $n{=}5000$ val images (resized-JPEG copy; absolute accuracy $\sim$1--3 points
below the original JPEGs; fp32 74.0 on originals, $n{=}1000$). \src{EdgeTRM/results/transfer/babel/deq_small_{noise_s0,s1,s2,quant}.json (jobs 10553354-7); analyze_x6.py deq}}
\label{tab:x6mdeq}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
Cell & $k{=}8$ & $k{=}16$ & $k{=}26$ & $k{=}100$ & Cos.\ to fp32 eq. & Converged at $k{=}100$ & Median steps \\
\midrule
\inputrows{tables/bank/x6_mdeq.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[H]
\caption{\textbf{DEQ-Transformer on WikiText-103: iterations help inside the basin and hurt outside it; the collapsed model
has the smallest residual.} Test perplexity (Anderson) by iteration cap, median relative residual and cosine to fp32 at cap 60;
full test set (245,569 tokens); noise rows mean [min, max] over 3 directions. fp32 reaches the published 23.1 at cap 60.
\src{EdgeTRM/results/transfer/babel/deqlm_{noise_s0,s1,s2,quant}.json (jobs 10554367-70); analyze_x6.py deqlm}}
\label{tab:x6deqlm}
\centering\footnotesize
\begin{tabular}{@{}llllll@{}}
\toprule
Cell (rel.\ err.) & $k{=}10$ & $k{=}30$ & $k{=}60$ & Median residual $k{=}60$ & Cos.\ to fp32 $k{=}60$ \\
\midrule
\inputrows{tables/bank/x6_deqlm.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=0.49\textwidth]{figures/x6_mdeq_small.png}\hfill
\includegraphics[width=0.49\textwidth]{figures/x6_deq_transformer.png}
\caption{\textbf{X6 read-out figures (draft, not house style).} Left: MDEQ-Small accuracy and residual against $\sigma$ /
quantizer relative weight error. Right: DEQ-Transformer perplexity by iteration cap and median residual at cap 60.
\src{EdgeTRM/figures/x6_mdeq_small.png, x6_deq_transformer.png (analyze_x6.py deqfig, deqlmfig)}}
\label{fig:x6}
\end{figure}

\begin{table}[H]
\caption{\textbf{MDEQ-XL (ImageNet): the larger published DEQ has the wider basin.} Broyden top-1 \% at $k{=}100$, $n{=}2000$; noise mean [min,
max] over 3 directions at $\sigma$ 0.1--0.5 (one direction at 0.05, 0.15, 0.7, 1.0); cosine to the fp32 equilibrium where measured.
\src{results/transfer/babel/deq_xl_*.json; X6.md RESULT 3}}
\label{tab:x6xl}
\centering\footnotesize
\begin{tabular}{@{}llll@{}}
\toprule
Cell & Top-1 & Cell & Top-1 \\
\midrule
fp32 & 75.5 & $\sigma$0.3 & 60.2 [56.6, 65.8] (cos 0.765) \\
$\sigma$0.05 & 75.0 & $\sigma$0.5 & 11.8 [5.4, 20.8] (cos 0.524) \\
$\sigma$0.1 & 74.7 [74.1, 75.5] & $\sigma$0.7 / 1.0 & 0.4 / 0.1 \\
$\sigma$0.15 & 72.9 & w8c / w4g32 / w4g128 & 75.4 / 73.8 / 73.7 \\
$\sigma$0.2 & 70.9 [69.8, 72.8] (cos 0.879) & w4a / w4c / w4t & 72.5 / 69.5 / 0.1 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Diffusion control (DDPM CIFAR-10): the ancestral sampler has a step-flat cost inside its basin; the deterministic one compounds.}
FID-5k against the fp32 samples drawn from the same $x_T$ and step noise, mean over 3 noise directions; quantizer rows give the relative weight
error. fp32 FID vs train: DDIM 10 / 25 / 50 / 100 = 35.2 / 22.0 / 18.2 / 15.8; DDPM 50 / 100 / 250 = 137.2 / 82.4 / 39.3. DDPM-1000 control (seed 0):
$\sigma$0.1 44.5, w4g32 22.3 (in-basin cost unchanged from 50 to 1000 steps), w4c 189 (still growing).
\src{results/transfer/babel/diff_{fp32,noise_s0,noise_s1,noise_s2,quant}.json; analyze_x6.py diff; X6.md RESULT 4}}
\label{tab:x6ddpm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
$\sigma$ / quantizer (rel.\ err.) & DDIM 10 & DDIM 25 & DDIM 50 & DDIM 100 & DDPM 50 & DDPM 100 & DDPM 250 \\
\midrule
\inputrows{tables/bank/x6_ddpm.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/x6_ddpm_cifar10.png}
\caption{\textbf{X6 diffusion read-out (draft figure).} FID vs fp32 samples against $\sigma$ / quantizer error, by sampler and step count.
\src{EdgeTRM/figures/x6_ddpm_cifar10.png (analyze_x6.py difffig)}}
\label{fig:x6ddpm}
\end{figure}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{MDEQ-Small}: flat to $\sigma$0.05 ($-0.7$), steep edge over 0.1--0.3 ($-4.9$, $-12.3$, $-24.7$, $-59.0$), chance
  by 0.5; half accuracy near $\sigma$0.2 (like TRM-MLP). Grouped INT4 is not free here (w4g32 $-7.3$). Budget: $k$ 8$\to$100
  adds +1.5--1.6 inside, +2.2--3.1 on the edge, exactly 0 at $\sigma\ge0.5$ and for w4t. Residual as a wrong-answer detector
  AUROC 0.42--0.67; w4t converges fastest (19 steps). Displacement from the fp32 equilibrium 0.08 / 0.20 / 0.38 / 0.68 /
  0.92 / 1.30 at $\sigma$ 0.02 / 0.05 / 0.1 / 0.2 / 0.3 / 0.5 ($\sim$4$\times$ the relative weight perturbation). Picard
  (TRM-style plain iteration) never converges on MDEQ even in fp32 (residual $\sim$0.7; 66--68\%), and its residual
  \emph{falls} under noise (0.71$\to$0.18 at $\sigma$1.0).
\item \textbf{MDEQ-XL: the larger published DEQ has the wider basin} ($n{=}2000$, Broyden, $T{=}100$; 3 noise directions at
  $\sigma$ 0.1 / 0.2 / 0.3 / 0.5, one at 0.05 / 0.15): fp32 75.5; $\sigma$ 0.05 75.0, 0.1 74.7 [74.1, 75.5], 0.15 72.9, 0.2 70.9
  [69.8, 72.8], 0.3 60.2 [56.6, 65.8], 0.5 11.8 [5.4, 20.8], 0.7 0.4, 1.0 0.1 (seed 0); w8c 75.4, w4g32 73.8, w4g128 73.7, w4a 72.5,
  w4c 69.5, w4t 0.1. Same shape as Small with the edge shifted right (Small at 0.2 / 0.3 / 0.5: 49.1 / 14.8 / 0.3); INT4 costs XL
  1.7 (w4g32) / 6.0 (w4c) points vs 7.3 / 15.9 for Small; its equilibrium moves less per unit noise (cosine 0.879 at $\sigma$0.2
  vs 0.779; 0.765 at 0.3 $\to$ 80\% retained; 0.524 at 0.5 $\to$ 16\%), so accuracy still follows the cosine. Residual falls as
  $\sigma$ grows (AUROC 0.45--0.53). \caveat{XL differs from Small in width, expansion and training: ``the larger published DEQ has
  the wider basin'', not a controlled width ablation} \src{results/transfer/babel/deq_xl_{noiseA_s0,B_s0,noise_s1,noise_s2,C_s0}.json (jobs 10554686/7, 10555307-9)}
\item \textbf{DEQ-Transformer}: plateau to $\sigma$0.1 (+3\%), edge 0.15--0.3, cliff between 0.3 and 0.5, collapse by 0.7;
  quantizers on the noise curve at their relative error; at $\sigma$0.7 / 1.0 more iterations make it worse (923$\to$1182,
  6181$\to$8059). Picard never converges here either (residual 0.42--0.53; fp32 ppl 57 at 60).
\item \textbf{Diffusion (DDPM CIFAR-10, $n{=}5000$ samples per cell, 3 noise directions)}: DDPM (fresh noise every step) behaves like the latent
  recursions: inside the basin ($\sigma\le0.1$, w8c, w4g32, w4g128) the distance to the fp32 samples is a fixed cost at every step count ($\sigma$0.1:
  43.2 / 42.8 / 42.1; w4g32 24.3 / 23.5 / 22.1; paired pixel RMSE 0.146 / 0.149 / 0.151) and FID vs train keeps improving at fp32's rate; outside
  ($\sigma\ge0.2$, w4a, w4c, w4t) more steps make it worse ($\sigma$0.3: 213 $\to$ 290). DDIM ($\eta{=}0$) compounds like the token-feedback generators:
  at $\sigma$0.05 paired RMSE 0.079 / 0.099 / 0.185 / 0.296 from 10 to 100 steps and FID vs fp32 190; the edge moves from $\sigma\approx0.1$ at 10
  steps to $\approx0.03$ at 100; w4g32 is near-harmless at 10--25 steps and destroys the 100-step sampler (304). \redtext{Interpretation, not
  measured: the injected noise re-randomises the state, playing the role of contraction; the ODE sampler has no such forgetting.}
\item \textbf{No usable checkpoints} for SE-RRM (code only) or AdRNN (no code); no monDEQ checkpoint is published.
\end{itemize}

% ---------------------------------------------------------------------------------------------------
\section{R14. Head-to-head with Ingolfsson et al.\ (X7)}
\label{r:x7}

\paragraph{Zero-mean noise vs fixed bias at matched norm (X7 section 3; p4d A100, 3 draws, $n_{\text{sup}}{=}16$, $H{=}3$).} Ingolfsson et
al.\ attribute the 4-bit collapse to a systematic (nonzero-mean) bias that accumulates with reuse; their Prop.~1 says fresh zero-mean
perturbation converges to $E[e]{=}0$ and should not displace the fixed point. Arms, all at matched per-call Frobenius norm: \texttt{an} fresh
zero-mean activation noise at every linear input (zero mean in time and in elements: their zero-mean case); \texttt{af} the same noise drawn
once and reused every call (step-coherent, element-mean zero); \texttt{ab} a fixed sign-consistent bias (80\% of its norm is the mean);
\texttt{wn} / \texttt{wb} zero-mean weight noise and sign-consistent weight bias. $\rho$ is the per-application output perturbation of each
linear, $\lVert y-W_0x\rVert/\lVert W_0x\rVert$, measured along the cell's own trajectory: the layer-level $\varepsilon$ of their Prop.~1.

\begin{table}[H]
\caption{\textbf{TRM Sudoku-MLP: zero-mean noise alone produces the cliff; bias and step-coherence shift it.} Exact \% at each $\sigma$,
mean [min--max] over 3 draws; $\sigma_{1/2}$ and $\rho_{1/2}$ = where exact falls below half of fp32 (71.4), per draw. $n{=}1000$, $H{=}3$, $L{=}6$.
Weight bias (\texttt{wb}, own grid): $\sigma$0.02 $\to$ 66.3 [64--69], 0.05 $\to$ 3.1 [2--4]; $\sigma_{1/2}$ 0.034--0.035, $\rho_{1/2}$ 0.047--0.049.
\src{p4d:x7/results/bn_sudoku_mlp_d{0,1,2}.json; EdgeTRM c5077fc; x7_ingolfsson.py --analyze; X7.md}}
\label{tab:x7mlp}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
Arm & $\sigma$ 0.1 & 0.15 & 0.2 & 0.3 & 0.5 & $\sigma_{1/2}$ (3 draws) & $\rho_{1/2}$ \\
\midrule
\inputrows{tables/bank/x7_mlp.tex}
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[H]
\caption{\textbf{TRM Maze-attn: bias leaves the basin where fresh noise does.} Exact \% mean [min--max] over 3 draws; $\sigma_{1/2}$ on exact
match and on valid path (any 4-connected start--goal path through open cells); fp32 88.4. $n{=}500$, $H{=}3$, $L{=}4$. Weight bias flat to
$\sigma$0.2 (88.1--88.7, $\rho\le0.06$): grid too short \running{extended to 0.3--2.0}.
\src{p4d:x7/results/bn_maze_attn_d{0,1,2}{a,w}.json; EdgeTRM a21a138; X7.md}}
\label{tab:x7maze}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
Arm & $\sigma$ 0.5 & 0.7 & 1.0 & 1.5 & $\sigma_{1/2}$ exact & $\sigma_{1/2}$ valid path & $\rho_{1/2}$ \\
\midrule
\inputrows{tables/bank/x7_maze.tex}
\bottomrule
\end{tabular}}
\end{table}

\paragraph{W4A4 ladder with Ingolfsson et al.'s definitions (X7 section 1; TRM Sudoku-MLP, $n{=}1000$, p4d, $H{=}3$, $L{=}6$; EdgeTRM 3054461).}
Their ordering reproduces on our checkpoint: with per-tensor weights, per-tensor activations 0.0, per-token 3.5, group-32 5.3, group-16 5.0; MXInt4
on both 65.4; group-32 on both 66.6. One difference: per-tensor \emph{weight-only} INT4 already collapses our MLP model (5.9\%; theirs 78.5), so our
$\sim$5\% ceiling with per-tensor weights comes from the weights, not the activation grid. \textbf{$\rho$ predicts every cell's side}: in-basin cells
have $\rho\le0.066$, collapsed cells $\rho\ge0.093$, and the fresh zero-mean noise cliff sits at $\rho$ 0.080--0.082. The quantizers' activation
error is partly coherent (0.38--0.57, between independent noise 0.25 and a fixed bias 1.0), and coherence does not separate in-basin from collapsed
cells (MXInt4 0.40 in; group-32 with per-tensor weights 0.40 out). The per-step perturbation relative to the basin decides survival, not the
quantizer's time-consistency. The ladders on the other three models are below (section 1b).

\begin{table}[H]
\caption{\textbf{W4A4 ladder on TRM Sudoku-MLP}: exact and cell accuracy, $\varphi_H$, $\rho_{\text{out}}$ and activation-error coherence (1 = fixed
bias, 0.25 = independent per step at $T{=}16$); static per-tensor rows mean [min--max] over 3 calibration draws; their Sudoku number (FP 84.1) for
comparison. \src{p4d:x7/results/ladder_sudoku_mlp.json; EdgeTRM 3054461; X7.md section 1; REWRITE_NOTES 42}}
\label{tab:x7ladder}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
Cell & Exact & Cell acc & $\varphi_H$ & $\rho_{\text{out}}$ & Coherence & Their Sudoku number (FP 84.1) \\
\midrule
\inputrows{tables/bank/x7_ladder.tex}
\bottomrule
\end{tabular}}
\end{table}

\paragraph{Reading.}
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Zero-mean noise alone produces the cliff.} Fresh zero-mean activation noise, the case Prop.~1 says should not displace the fixed
  point, takes Sudoku-MLP from 62.9\% to 2.3\% between $\sigma$0.2 and 0.5 (draw spread $\le$2 points), and the maze from 85.5\% at 0.7 to 23.3\%
  at 1.0 and 0 at 1.5, with the same plateau-then-collapse shape as every other arm.
\item \textbf{Bias and step-coherence shift the cliff by 1.3--1.9$\times$; they do not create it.} On Sudoku-MLP step-coherence moves
  $\sigma_{1/2}$ from 0.29 to 0.22 (1.3$\times$) and a sign-consistent bias of equal norm to 0.15--0.19 (1.5--1.9$\times$).
\item \textbf{On $\rho$, every arm collapses within a factor-3 band}: $\rho_{1/2}$ 0.04--0.12 across all five Sudoku-MLP arms against a factor-8
  band in $\sigma$. Per unit $\rho$ the bias is \emph{not} more harmful than fresh noise ($\rho_{1/2}$ 0.09--0.12 vs 0.08): its extra damage in
  $\sigma$ comes from a larger per-step effect, not from accumulation. At equal Frobenius norm a sign-consistent \emph{weight} bias is
  4$\times$ more damaging in $\sigma$ (0.034 vs 0.14) but collapses at the same $\rho$ as zero-mean weight noise (0.047--0.049 vs 0.038--0.042):
  its mean is a rank-1 component with a large operator norm.
\item \textbf{On the attention maze, bias leaves the basin where fresh noise does} ($\sigma_{1/2}$ 0.82--0.90 vs 0.90; $\rho$ 0.18--0.20 vs 0.20);
  step-coherent zero-mean noise is the most damaging activation arm (1.2--1.5$\times$). The basin is $\sim$3$\times$ wider than Sudoku-MLP's on
  every arm (\texttt{an} 0.90 vs 0.29): the mixer contrast of \S\ref{r:mixer}.
\item \textbf{Meaning for framing A}: this is the rebuttal evidence against the accumulation account. No bias is needed to cross the
  boundary, and bias moves the edge by a bounded factor that disappears on the per-application scale.
\end{itemize}

\paragraph{Depth dose-response at test time: depth does not compound inside the basin (X7 section 2; EdgeTRM a5a14d0; REWRITE\_NOTES 74).}
Fixed checkpoint and quantizer; static activation scales calibrated once at the default depth; each series pairs the quantized model with fp32 on the same
examples, same $H$/$L$/$n_{\text{sup}}$, same p4d run; 95\% paired bootstrap CIs (2000 resamples; $n{=}1000$ Sudoku and HRM, 500 Maze).

\begin{table}[H]
\caption{\textbf{Exact \% along $n_{\text{sup}}$ at the default $H$/$L$} (fp32 / w4c / MXInt4 W4A4 / w4t weight-only / per-tensor W4A4 static), and the change in the
gap to fp32 from $n_{\text{sup}}$ 1 to 32 for the in-basin cells [95\% paired CI]. \src{results/breadth/p4d/x7/depth_*.json; x7_depth_ci.py -> results/breadth/x7_depth_ci.json; X7.md section 2}}
\label{tab:x7depth}
\centering\scriptsize
{%
\begin{tabular}{@{}p{0.09\textwidth}p{0.13\textwidth}p{0.13\textwidth}p{0.13\textwidth}p{0.13\textwidth}p{0.27\textwidth}@{}}
\toprule
Model & $n_{\text{sup}}$ 1 & 4 & 16 & 32 & Gap change 1 $\to$ 32, in-basin cells \\
\midrule
Sudoku-MLP & 28.4 / 23.4 / 15.0 / 2.1 / 0.0 & 61.0 / 59.4 / 55.6 / 5.0 / 0.0 & 71.4 / 67.9 / 65.4 / 5.9 / 0.0 & 74.2 / 70.3 / 68.3 / 5.7 / 0.0 & w4c +1.1 [$-1.8$, +4.0]; MX +7.5 [+4.4, +10.8] \\
Sudoku-attn & 3.1 / 2.3 / 2.1 / 1.8 / 0.0 & 52.5 / 51.2 / 48.1 / 44.6 / 0.0 & 65.7 / 66.2 / 66.2 / 62.8 / 0.0 & 69.7 / 69.6 / 70.1 / 65.6 / 0.0 & w4c +0.7 [$-1.0$, +2.3]; MX +1.4 [$-0.5$, +3.4]; w4t $-2.8$ [$-5.0$, $-0.6$] \\
Maze-attn & 80.2 / 80.6 / 77.8 / 77.8 / 0.0 & 88.4 / 88.0 / 88.4 / 87.2 / 0.0 & 88.4 / 88.0 / 88.4 / 87.4 / 0.0 & 88.6 / 88.2 / 88.4 / 87.6 / 0.0 & w4c $-0.8$ [$-2.2$, +0.4]; MX +2.2 [$-0.4$, +4.6]; w4t +1.4 [$-1.2$, +3.8] \\
HRM Sudoku & 1.3 / 1.0 / 0.7 / 1.0 / 0.0 & 30.8 / 30.5 / 29.2 / 29.1 / 0.0 & 49.2 / 48.9 / 49.9 / 46.9 / 0.0 & 51.7 / 52.0 / 52.0 / 50.8 / 0.0 & w4c +0.6 [$-1.0$, +2.3]; MX +0.9 [$-1.0$, +2.9]; w4t $-0.6$ [$-2.5$, +1.3] \\
\bottomrule
\end{tabular}}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Verdict}: for in-basin quantizers the gap to fp32 from $n_{\text{sup}}$ 1 to 32 is flat or shrinking in \textbf{11 of 12} series (the CI of the change
  includes 0 or is positive). \textbf{$H$ sweeps are flat} within $\sim$1 point per model (gap at $n_{\text{sup}}$ 16 along $H$: Sudoku-MLP w4c $-2.7$ / $-3.2$ / $-3.5$ /
  $-3.1$ / $-3.9$ at $H$ 1 / 2 / 3 / 4 / 6, MX $-6.0$ / $-5.3$ / $-6.0$ / $-6.0$ / $-5.9$; Sudoku-attn MX $-3.1$ / $-0.8$ / +0.5 / +0.7 / +0.4; Maze MX 0.0 to $-0.2$; HRM
  ($H$ 1--4) MX $-1.2$ / +0.7 / +0.1 / +0.3).
\item \textbf{Two bounded exceptions, both stated}: Sudoku-attn per-tensor weight-only INT4 widens by 2.8 [0.6, 5.0] and stays at a $-3$-point offset; Sudoku-MLP
  MXInt4 along $L$ (Ingolfsson's dose-response axis, here at test time) goes from +4.6 at $L{=}1$ (where fp32 is 44.2\%) to $-6.7$ [$-9.0$, $-4.4$] at $L{=}8$ and stops at
  its default-depth gap ($-6$) rather than growing without bound. Other $L$ series: Sudoku-MLP w4c $-5.8$ / $-0.4$ / $-1.0$ / $-3.5$ / $-4.4$ (not monotone);
  Sudoku-attn MX +0.1 / +0.4 / $-1.0$ / +0.5 / +0.8; Maze MX $-1.0$ / +0.6 / 0.0 / +0.4; HRM ($L$ 1 / 2 / 4) MX $-2.5$ / +0.7 / +0.1.
\item \textbf{Past the edge} (our clipping: absmax over all calls), per-tensor W4A4 static is 0.0\% at every $n_{\text{sup}}$, $H$ and $L$ on all four models; the gap ``widens'' only because fp32 improves
  (Sudoku-MLP fp32 28.4 $\to$ 74.2), which is what Ingolfsson's Sudoku dose-response shows too. Weight-only per-tensor INT4 on Sudoku-MLP: 2.1 $\to$ 5.7 while fp32
  28.4 $\to$ 74.2.
\item \textbf{Ingolfsson's Maze INT4 reproduces under their clipping} (X7 section 2b; EdgeTRM 8b9a60a; p4d, $n{=}500$, one calibration draw; REWRITE\_NOTES 83).
  Matched config (their calibration statistic is unstated; we used a 99.99th-percentile scale; block linears only, heads fp32): Maze W4A4 exact at
  $n_{\text{sup}}$ 1 / 4 / 16 / 32 = 39.6 / 81.8 / \textbf{82.2} / 82.2 vs fp32 80.2 / 88.4 / 88.4 / 88.6 (valid path 98.2). The paired gap is $-40.6 \to -6.6 \to -6.2 \to -6.4$:
  it closes over the first steps and then holds a constant offset, the in-basin shape; flat along $L$. Sudoku-MLP under the same config stays collapsed
  (0.5--1.0\%, 3 draws). Our earlier 0.0\% came from our own clipping rule (max over all calls), not from head coverage. Their ``improves with depth'' is the
  early-step closing of an in-basin gap, which then stays constant. \running{3-calibration-draw version}
\end{itemize}

\paragraph{W4A4 ladder on the other three models (X7 section 1b; $n{=}1000$ / 500).} Exact \% (fp32 / W8A8 / W4A4 per-tensor static [3 calibration draws] /
dynamic / T-weights + per-token / T-weights + group-32 / W4 per-channel + A4 per-token / group-32 both / MXInt4 both): Sudoku-attn 65.7 / 66.5 / 0.0 / 0.0 /
26.7 / 61.4 / 39.4 / 67.5 / 66.2; Maze-attn 88.4 / 88.9 / 0.0 / 0.0 / 85.6 / 87.6 / 86.4 / 88.0 / 88.4 (valid path 99.8 fp32, 0.0 per-tensor, 99.6 MX); HRM Sudoku
49.2 / 50.9 / 0.0 / 0.0 / 28.1 / 48.5 / 31.6 / 50.8 / 49.9. Per-tensor activations collapse all four models; per-token is the edge; group-32 and MX are inside.
$\rho$ orders them as on Sudoku-MLP with a wider edge band: cells at $\rho\le0.074$ keep $\ge$97\% of fp32; per-token cells at $\rho$ 0.10--0.14 are partial; every
collapsed cell has $\rho\ge0.19$ (the fresh-noise cliffs sit at $\rho$ 0.17, 0.20 and 0.12).

\paragraph{Bias arms on Sudoku-attn and HRM (X7 section 3b; 3 draws, $n{=}1000$).} $\sigma_{1/2}$ ($\rho_{1/2}$): Sudoku-attn \texttt{an} 0.551--0.553 (0.167--0.168),
\texttt{af} 0.354--0.359 (0.11), \texttt{ab} 0.383--0.418 (0.116--0.130), \texttt{wn} 0.62--0.81 (0.20--0.28); HRM \texttt{an} 0.421--0.427 (0.118--0.119), \texttt{af}
0.24--0.35 (0.07--0.10), \texttt{ab} 0.25--0.36 (0.07--0.10), \texttt{wn} 0.99--1.03 (0.30--0.31). \textbf{Zero-mean noise alone collapses every model} (Sudoku-attn 44.0 at
0.5 $\to$ 1.1 at 0.7; HRM 12.0 at 0.5 $\to$ 0 at 0.7). The fixed arms leave the basin at 0.6--0.8$\times$ the fresh-noise $\sigma$; \textbf{on HRM fixed zero-mean noise and a
bias of equal norm are indistinguishable} (\texttt{af} 0.24--0.35 vs \texttt{ab} 0.25--0.36), so the extra damage comes from time coherence, not from a nonzero mean.
\running{weight-bias $\sigma$ 0.3--2.0 extension on attention and HRM, p4d card 0}

\begin{redpar}
\noindent\textbf{Still pending (X7):} the 3-draw version of the Maze config match; the weight-bias extension. Their checkpoint reaches 84.1\% on Sudoku, ours 70.8--71.4\%;
absolute numbers are not comparable, the ordering is.
\end{redpar}
\src{EdgeTRM/x7_ingolfsson.py (879b027, 2a261f5, 349c0b3, c5077fc, a21a138); X7.md; REWRITE_NOTES 41}

% ---------------------------------------------------------------------------------------------------
\section{R15. Devices: host simulation of the vendor graphs, chip quantizers, MCU (X3)}
\label{r:devices}

\begin{redpar}
\noindent\textbf{Scope of every number here.} AI Hub profiles are latency and memory only. Correctness numbers name their runtime:
\textbf{QNN HTP} (on the phone, AI Hub inference chains), \textbf{ORT-fused} (ONNX Runtime at its default optimization level, fused
integer QDQ kernels, on a host CPU), \textbf{reference QDQ} (ORT with optimizations disabled, or the torch QDQ executor). The two host
executors agree on the pure 8-bit and 16-bit graphs and differ only on mixed 8/16 graphs; the phone's fused RMSNorm departs from the literal
QDQ semantics (REWRITE\_NOTES 40, 43, 51). No energy number exists (D1).
\end{redpar}

\paragraph{On the phone: the narrow-basin MLP model survives the vendor's 8-bit activations on the S24} (X3, Sep 25 02:10--03:00 UTC;
REWRITE\_NOTES 43--49). Samsung Galaxy S24 (Snapdragon 8 Gen 3), AI Hub graphs compiled with qnn\_dlc and run on QNN HTP, $H{=}1$, 8 steps,
carry through the quantized I/O, one clean 8-job chain per cell; the host columns run the same QDQ graph in ONNX Runtime.

\begin{table}[H]
\caption{\textbf{S24 on-device results, every number labelled by its runtime.} Exact solved after 8 steps (cells); ORT-fused = ONNX Runtime
at its default optimization level on a host CPU, same graph. Sudoku rows: puzzles 0--99; Maze: 50 mazes. Halting-head AUROC on the device 1.00
for every Sudoku chain. \src{EdgeTRM/results/devices/infer/<task>/dev_*_Samsung_Galaxy_S24.json; results/devices/device_faithful_acc.json (ON DEVICE rows); EdgeTRM 98f0945, 5ca44a2, e71c772, f216346, 651ff51; X3.md}}
\label{tab:x3device}
\centering\footnotesize
\begin{tabular}{@{}p{0.17\textwidth}p{0.29\textwidth}p{0.31\textwidth}p{0.17\textwidth}@{}}
\toprule
Task, graph & QNN HTP on the S24 & Host, same graph: ORT-fused / reference QDQ & Host fp32 \\
\midrule
Sudoku-MLP fp32 graph (fp16 on HTP) & 58/100 (cells 84.3\%; 98.5\% cell agreement with host fp32) & -- & 58/100 \\
Sudoku-MLP w8a8 & \textbf{61}/100 (cells 84.6\%) & 0/100 (41.6\% cell agreement with the device) / 0/100 & 58/100 \\
Sudoku-MLP w8a16 & 56/100 (83.8\%) & 56/100 (93.9\% cell agreement) / 66 (16 steps) & 58/100 \\
Sudoku-attn w8a8 & 50/100 (83.6\%) & 49/100 (89.0\% cell agreement) & 51/100 (w8a16 53) \\
Maze w8a8 & \redtext{0/50 (cells 61.1\%, flat): device-toolchain divergence at step 1} & 42/50 & 44/50 (S24 fp32 chain) \\
Any W4A16 / W4A8 graph & \redtext{wrong from step 1 (no number quotable)} & Sudoku-MLP w4a16 69/100; Maze 44/50 & \\
\bottomrule
\end{tabular}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{What holds}: at literal per-tensor 8-bit activations the MLP model is outside its basin on any faithful executor (0/100 under
  ORT-fused and under reference QDQ semantics); the phone's execution keeps it inside: the vendor compiler replaced the RMSNorm's declared 8-bit intermediate
  encodings with a fused RmsNorm op (QNN HTP: MLP w8a8 61 vs host fp32 58; the fused op's internal precision is not visible). The attention model absorbs the same 8-bit activations everywhere (S24 50, ORT-fused 49, fp32 51). This fits the basin
  story: 8-bit activations are a perturbation the narrow basin cannot absorb and the wide one can, consistent with the MLP model's larger RMSNorm
  variance range (1673 vs 7.7). At w8a16 host and device agree (56 and 56). (Correction, REWRITE\_NOTES 51: the earlier wording ``the ORT-fused
  collapse is the runtime's'' is withdrawn; it is the literal QDQ semantics, and the vendor kernel departs from them.)
\item \textbf{Device fp baseline (X3, acct3; REWRITE\_NOTES 82; MLSys material)}: the S24 HTP runs the fp32 graph in fp16: 58/100 at step 8 (per step
  1 / 2 / 26 / 36 / 43 / 53 / 55 / 58), host fp32 58/100. Against this device baseline, on the same puzzles and 8 steps, w8a8 61, w8a16 56 and the mixed w8a8rms16u
  54 are all within $\pm$4 (host run-to-run noise).
\item \textbf{Every device number names its runtime}, and device-vs-host gaps run both ways: Sudoku-MLP device 61 vs host 0 (both host
  executors); Maze device 0 vs host 42. The S24 Maze w8a8 chain diverges from the host at step 1 ($z_H$ cosine 0.695, argmax agreement 0.60) while the same I/O path works
  for all three Sudoku chains; the log shows tiling and fp16 concat-replacement warnings (candidate: RoPE/Concat handling at sequence length 916).
  It is a device-toolchain correctness failure, not model accuracy; any device INT8 correctness claim is per task and per runtime.
\item \redtext{\textbf{INT4 on the HTP computes the wrong function} (REWRITE\_NOTES 47, 49): every W4A16 chain (S24 Sudoku-MLP, Maze, Sudoku-attn;
  RB3 Sudoku-MLP) is wrong from step 1 ($z_H$ cosine 0.14 to the host), and W4A8 Sudoku-MLP too (cosine 0.086, argmax agreement 0.28); the runtime
  log shows the disabled op \texttt{q::QNN\_CastInt4ToInt8\_cp} for every INT4 weight. So every INT4 device latency and memory figure (qnn\_dlc, and
  the Sep 10 $H{=}3$ qnn\_context\_binary rows, e.g.\ the Sep 13 draft's ``58 ms on a Snapdragon 8 Gen 3 NPU'' and ``6 MB on QCS6490'') times a
  graph that was never shown to compute the model. No INT4 device figure is quoted as INT4 inference until an INT4 path matches its reference.
  Pending: W4A16 via precompiled\_qnn\_onnx (jpxlljylp).}
\item \textbf{Reference QDQ confirms the host collapse is semantic} (ORT\_DISABLE\_ALL, Sudoku-MLP, $n{=}100$, 16 steps; REWRITE\_NOTES 51):

\begin{center}\footnotesize
\resizebox{0.97\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
Row & Activation precision & Reference QDQ & ORT-fused (M3 executor) \\
\midrule
A0 & w8a16 unmodified & 66 & 66 (66) \\
A2b & RMSNorm variance path at 8 bit, rest 16 & 0 & 0 \\
A8 & all 555 activation tensors at 8 bit (the AI Hub w8a8 graph) & 0 & 0 \\
B2b2 & all 8 bit except the variance path at 16 & 51 & 0 (48) \\
\textbf{B2ab} & \textbf{all 8 bit except x$\ast$x + variance path at 16 (84 of 555 tensors; norm output at 8)} & \textbf{68} & \textbf{0 (68)} \\
B2 & all 8 bit except every RMSNorm tensor at 16 & 68 & 69 (66) \\
\bottomrule
\end{tabular}}
\end{center}
  The faithful 8-bit QDQ graph collapses on every host executor; only the S24 QNN HTP (fused RMSNorm) avoids it. ORT's fusions matter only for
  the mixed 8/16 rows. Under reference semantics the variance path alone both breaks the model and, kept at 16, mostly recovers it, and x$\ast$x
  + variance at 16 (B2ab, 84 of 555 activation tensors) is a complete fix. \textbf{The minimal fix differs per runtime}: QNN HTP (S24) none (61/100
  unmodified); reference QDQ x$\ast$x + variance at 16; ORT-fused the whole RMSNorm. The earlier ``keep the whole RMSNorm at 16'' was ORT-specific.
  Candidate deployment sentence: two small groups of norm tensors decide whether the narrow-basin model survives 8-bit activations, and each
  runtime needs a different minimal override.
  \src{p4d:aihub_artifacts/h1/sudoku_mlp/infer/ablate/eval_*_0_100_ref.json; X3.md; REWRITE_NOTES 51}
\item \textbf{What the S24 actually ran} (X3, EdgeTRM 6164dcc; \texttt{results/devices/wa\_collapse/dlc\_encodings\_w8a8.json}; REWRITE\_NOTES 63): in the DLC of
  the S24 Sudoku-MLP w8a8 chain our declared scales survive on every kept tensor (matmul outputs 112/112, injection adds 14/15, embed 5/6), so the
  compiler did not re-derive scales; but only 4 of 140 RMSNorm-internal tensors exist in the DLC and none carries our scales: 27 of 28 norms were fused
  into a vendor RmsNorm op, so the 8-bit variance-path encodings (which alone give 0/100 on the host) never run. Wording: ``the vendor compiler replaced
  the RMSNorm's declared 8-bit intermediate encodings with a fused RmsNorm op''; ``computes the norm at higher precision'' is an inference (the fused
  op's internal precision is not visible).
\item \redtext{\textbf{INT4 is wrong on both QNN runtimes} (REWRITE\_NOTES 64): W4A16 via precompiled\_qnn\_onnx and via qnn\_dlc give identical cell
  accuracy 42.25\% (host W4A16 55.83\%, fp32 55.85\%). \textbf{Two HTP legality rules} for mixed-precision overrides (REWRITE\_NOTES 65; MLSys material):
  a Gather's table and output share one encoding; data-movement ops keep their input's encoding; graphs violating them fail validation at step 0.}
\item \running{20 new chains (S24 and Snapdragon 8 Elite QRD: fp32 / w8a8 / w8a16 / w8a8sqvar16, attention, Maze; the rebuilt B2 graphs w8a8rms16u,
  w8a8sqvar16u)}
\end{itemize}

\paragraph{Host simulation, Sudoku-MLP, 100 puzzles, $H{=}1$, 16 steps, carry through the quantized I/O.} fp32 68/100 (cell
87.9\%); AI Hub w8a8 0/100 (cell 41.9\%); w4a8 0/100 (51.6\%); w8a16 70/100 (88.0\%); w4a16 69/100. AI Hub (AIMET) quantizes
every activation tensor (residual adds, RMSNorm internals, gates) to per-tensor UINT8, which the harness's +a8 (linear inputs
only; w8c+a8 61.6\%) does not model. Sudoku-attn w8a8 69/100 vs fp32 65; w4a8 62/100 (cell 86.8\%). ARC (100 canonical rows,
$H{=}1$, 8 steps, token exact): fp32 23/100 (cells 91.5\%), w8a16 23/100 (91.4\%), w8a8 14/100 (87.3\%), still rising at step 8.
16-bit activations recover fp32 on every model tested; 8-bit activations cost Sudoku-MLP everything, ARC part, Sudoku-attn
nothing. Device-faithful accuracy table (host simulation of every compiled graph, exact, $H{=}1$): Sudoku-MLP (16 steps) fp32 70.2 / w8a16
69.7 / w8a8 0.0 ($n{=}1000$), w4a16 69 / w4a8 0 ($n{=}100$); Sudoku-attn (16 steps, $n{=}100$) fp32 65, w8a8 69, w4a8 62, w8a16 65, w4a16 63;
Maze (8 steps, $n{=}50$) fp32 44, w8a8 42, w4a8 42, w8a16 44, w4a16 44; ARC (8 steps, 100 rows, token exact) fp32 23, w8a8 14, w8a16 23
(\texttt{results/devices/device\_faithful\_acc.json}). \caveat{the ARC ``99 of 126 MB'' embedding share came from a notebook-era export; for
the checkpoint every result uses (step\_518071) the puzzle-embedding table is 1,795 of 1,822 MB (98.5\%)} $n{=}1000$ (puzzles 1000--1999): w8a8 0/1000 at every step 1--16; fp32 70.2\% at step 16.
\running{w8a16, the fix B2 and A2b2 at $n{=}1000$; B2ab}
\src{p4d:aihub_artifacts/h1/<task>/infer/host_*.npz; logs x3/logs/infer_prep_host.log; X3.md}

\begin{table}[H]
\caption{\textbf{Localising the w8a8 collapse} (Sudoku-MLP, 100 puzzles, $H{=}1$, 16 steps; start from the w8a16 graph and move
one activation group to the w8a8 graph's own 8-bit encoding (A rows), or take everything to 8 bit and keep one group at 16 (B
rows)). Run-to-run spread $\pm$4 puzzles (A0 = 66 here, 70 in an earlier run). The RMSNorm variance path is the only single group
that kills the model at 8 bit. The SwiGLU product has the heaviest tails and is harmless (outlier ratio does not predict damage).
\caveat{Runtime column: every row here is ORT-fused; reference-QDQ reruns (X3) give A0 66, A2b 0, A8 0, B2b2 51, B2 68 (table with the S24 results). M3 (Sep 25 00:30--00:40): ONNX Runtime's extended graph optimizations (integer QLinear fusions, the default ENABLE\_ALL used here)
change the arithmetic of graphs that mix uint8 and uint16 encodings. Under reference QDQ semantics (torch executor; ORT BASIC agrees) B2b2
(variance path at 16) gives \textbf{48} not 0, and B2ab (x$\ast$x + variance at 16) \textbf{68} not 0; rows that agree under both: A0 66/66, A8 0/0,
A2b2 0/0, A2a 59/58, A3 69/71, B2 66/69, B236 67/70. So ``the whole RMSNorm at 16 bit is needed'' came from ORT's fused kernels; the smallest
fix under QDQ semantics is x$\ast$x + variance path at 16. The B rows marked 0 must be rerun with ORT\_ENABLE\_BASIC before any claim} \src{EdgeTRM/wa_collapse.py (20e0ba6); p4d:aihub_artifacts/h1/sudoku_mlp/infer/ablate/eval_*.json}}
\label{tab:x3ablate}
\centering\footnotesize
\begin{tabular}{@{}p{0.18\textwidth}p{0.5\textwidth}lll@{}}
\toprule
Row & Activation change & Exact /100 & Cell \% & Runtime \\
\midrule
\inputrows{tables/bank/x3_ablate.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Cross-mixer: the same perturbation is outside one basin and inside the other.} Only the RMSNorm variance path at
8 bit (A2b2), host simulation, 100 puzzles. \src{X3.md}}
\label{tab:x3cross}
\centering\footnotesize
\begin{tabular}{@{}lllll@{}}
\toprule
Model & fp32 & w8a16 & A2b2 (variance path at 8 bit) & w8a8 \\
\midrule
\inputrows{tables/bank/x3_cross.tex}
\bottomrule
\end{tabular}

\vspace{6pt}
\begin{tabular}{@{}lll@{}}
\toprule
Group & Sudoku-MLP max abs / median max/std / 8-bit step/std & Sudoku-attn (same) \\
\midrule
\inputrows{tables/bank/x3_cross_ranges.tex}
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\caption{\textbf{Activation ranges per group}, Sudoku-MLP (fp32 values on 8 calibration carries; step = the w8a8 encoding's
step). \src{results/devices/wa_collapse/act_stats_by_group.json}}
\label{tab:x3groups}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
Group & Tensors & Max abs & Median std & Median max/std & Max max/std & Median 8-bit step/std & Median frac.\ within half a step \\
\midrule
\inputrows{tables/bank/x3_groups.tex}
\bottomrule
\end{tabular}}
\end{table}

\paragraph{Carry precision is not the constraint} (Babel, $n{=}1000$, deterministic; static scales on 64 held-out puzzles).
Sudoku-MLP with fp32 weights at $H{=}1$, $n{=}16$: fp32 carry 64.2; fp16 64.4, bf16 64.6; INT8 per-tensor / per-channel /
per-token 64.3 / 64.8 / 63.7; INT4 63.3 / 65.8 / 64.3 ($\varphi_H$ falls to 0.84--0.91, accuracy does not). With chip
weights: w4l64 61.6 (fp16 carry), 61.8 (INT8), 62.9 (INT4 per-channel); w4l64+a16+INT8 carry 61.8; the AI-Hub-like
w4c+a8+INT8 carry 57.6. All within $\sim$1.5 points of the fp32-carry cell at $H{=}1$ and 3. The ``4-bit state freezes
recurrent updates'' failure (arXiv 2609.04490, post-June) does not occur for TRM. \src{results/devices/chipq/carry_sudoku_mlp.json (job 10553047)}

\paragraph{AI Hub facts.} The quantize job writes per-output-channel symmetric INT4 weights and per-tensor asymmetric UINT8
activations; there is no granularity option. Compiled S24 binaries: \redtext{6.3 MB (INT4; not a working INT4 graph)}, 8.7 MB (INT8), 11.6 MB (FP16) for
Sudoku-MLP $H{=}3$. The \texttt{qnn\_context\_binary} target was removed after Sep 10; new rows use \texttt{qnn\_dlc}. 35
chipsets reachable (21 with QNN v68--v81; 14 TF-Lite-only). FP16 is missing on exactly the five chips where fp32 compiles failed
(Snapdragon 888, 778G, QCS6490, 7 Gen 4, QCM6690): ``integer-only'' is a per-SoC attribute. Accuracy depends on $H\times n$ only,
so per-answer latency at $H{=}1$ is $n\times$ step($H{=}1$). \running{$H{=}1$ profiling fan-out; granularity compile matrix (LPBQ
on v69+)}

\begin{table}[H]
\caption{\textbf{AI Hub latency and memory of one supervision step at $H{=}3$} (Sep 10 sweep; 260 compiles on 32 devices
succeeded, 124 failed; 325 profiles). ms per step for fp32 (FP16 on HTP), INT8 and INT4 graphs, and INT4 peak memory (MB).
\caveat{every INT4 column is red: INT4-weight graphs on the HTP compute the wrong function (disabled
\texttt{QNN\_CastInt4ToInt8} op) and these Sep 10 INT4 rows were never correctness-checked; the INT8 graphs carry 8-bit activations (the S24
runs them correctly for Sudoku, not for Maze); the $H{=}3$ step is not the recommended $H{=}1$ configuration} \src{reports/EDGETRM_MASTER_TABLES.md G; results/breadth/aihub_status.json}}
\label{tab:aihub}
\centering\footnotesize
\begin{tabular}{@{}llrrrr@{}}
\toprule
Task & Device & fp32 ms & INT8 ms & INT4 ms & INT4 MB \\
\midrule
\inputrows{tables/bank/mt_G_pivot.tex}
\bottomrule
\end{tabular}
\end{table}

\paragraph{Arm microcontroller at $H{=}1$ (Vela / Corstone-300 FVP).} Usable: the Sudoku-MLP INT8 step on Ethos-U55-256, Vela
5.2 at 500 MHz: 104 ms per step at $H{=}1$, 312 ms at $H{=}3$ (ratio 3.0); the FVP measures 110.8 / 332.6 ms (6.5\% above Vela;
$H{=}3$ reproduces the Sep 10 figure to 0.015\%); SRAM 1.2 MiB either way. \caveat{not usable: every attention FVP cycle count
(2,254 invalid MUL/REDUCE\_SUM commands per step); any TFLM output (the reference INT8 REDUCE\_SUM in the RMS norm returns $-1$
where exact arithmetic gives $-127$/$-128$, so every TFLM graph emits one repeated value; arena sizes stay valid); INT4 through
TFLite (Vela 5.1/5.2 crash on INT4 FULLY\_CONNECTED); the FVP MLP graph's output has not been checked, so the MCU claim is a
latency and memory claim only}. \redtext{The TOSA route compiles INT4 (one SwiGLU block: weights 2.19$\to$0.91 MB, U55 cycles
2.26 M$\to$1.83 M); output not checked, so not an INT4 inference figure.} \src{EdgeTRM/results/devices/mcu_h1.md (6ed02a7)}

\paragraph{Energy.} \redtext{None. AI Hub, Qualcomm Device Cloud, Vela/FVP and the phone farms report no power; the laptop PPT
sensor does not track CPU load (12 s of 8-thread matmul read 10.7 W vs 12.4--13.3 W idle). An analytical estimate (Horowitz
45 nm op/byte energies) is in \texttt{results/devices/energy\_estimate.json}, labelled as an estimate; an L40S reference
measurement is queued. Real energy waits on AWS credits ($\sim$two weeks) or a device purchase (D1).}

% ---------------------------------------------------------------------------------------------------
\section{R16. Sep 13 results kept in the legacy appendix}
\label{r:legacy}
Structured pruning, knowledge distillation, linear-attention approximation (Maze), context-length truncation, QAT
configurations, the Sep 10 SRAM footprints and device tables, the sequence-length INT8 penalty and static-vs-dynamic
quantization are in the legacy appendix (Appendix~\ref{app:pruning_distill}, \ref{app:linattn}, \ref{app:context},
\ref{app:qat}, \ref{app:sram_footprint}, \ref{app:latency}). \caveat{unrevised: HRM tables there may mix $H$; the device rows
time 8-bit-activation graphs at $H{=}3$; the MCU/TFLM rows are affected by the REDUCE\_SUM bug; the ``QAT cannot repair it''
and ``errors compound across cycles'' statements are withdrawn}


==> tables/bank/m1_attn.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/M1.md; header: | compressed (c16) | c15+f1 | c14+f2 | c12+f4 | c8+f8 | c16+f8 (24 steps) | worth in fp32 steps (k=1/2/4/8) |
w4t (62.9) & 62.9 & 64.2 & 65.4 & 66.7 & 69.8 & +8.7 / +9.8 / +10.0 / +11.0 \\
n8t4 nested (62.1) & 62.1 & 63.3 & 65.4 & 66.9 & 68.1 & +7.8 / +8.2 / +10.0 / +11.4 \\
w3c (59.7) & 60.1 & 62.8 & 66.0 & 68.0 & 69.3 & +6.0 / +7.6 / +12.0 / +16.5 \\
w3a (61.8) & 62.0 & 62.5 & 64.5 & 67.1 & 69.6 & +7.6 / +7.2 / +8.2 / +11.8 \\
w3g32 (66.4) & 66.8 & 67.2 & 67.7 & 67.9 & 70.4 & (above fp32 at 16) \\
noise 0.7 x3 (45.6 [45.5-50.6]) & 48.4 & 55.5 & 62.5 & 65.5 & 67.2 & +2.3 / +3.0 / +5.2 / +6.2 \\
noise 1.0 x3 (6.9 [3.6-11.6]) & 11.3 & 23.5 & 36.4 & 44.6 & 42.2 & +0.3 / -0.4 / -1.9 / -5.2 \\
w3t (0.0) & 0.0 & 1.7 & 8.5 & 23.4 & 17.4 & -1.0 / -1.5 / -2.8 / -6.4 \\
w2g32 (0.0) & 0.4 & 6.2 & 21.3 & 28.2 & 27.2 & -0.9 / -0.9 / -2.4 / -6.2 \\


==> tables/bank/m1_mlp.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/M1.md; header: | compressed (c16) | c15+f1 | c14+f2 | c12+f4 | c8+f8 | c16+f8 (append, 24 steps) | worth in fp32 steps (k=1/2/4/8; k_eq - k, k_eq read off the fp32 c
w4t (5.9) & 32.6 & 52.0 & 64.6 & 69.1 & 69.6 & +0.2 / +0.3 / +1.8 / +3.0 \\
w3c (17.3) & 30.1 & 51.8 & 62.0 & 68.0 & 67.8 & +0.1 / +0.3 / +0.5 / +0.8 \\
w3g32 (51.2) & 58.9 & 62.7 & 66.7 & 69.5 & 71.0 & +2.6 / +2.8 / +3.3 / +3.8 \\
w3a (50.8) & 56.0 & 62.5 & 67.3 & 70.5 & 72.3 & +2.0 / +2.7 / +3.8 / +7.5 \\
noise 0.15, 3 draws (28.6 [25.8-31.5]) & 50.7 & 60.4 & 64.7 & 68.8 & 68.5 & +1.1 / +1.9 / +1.8 / +2.5 \\
noise 0.2 draw 0 (8.0) & 46.7 & 56.3 & 63.4 & 69.0 & 69.0 & +0.9 / +1.0 / +1.1 / +2.8 \\


==> tables/bank/m2_main.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/M2.md; header: | model, spec | single rollout | best-Q@4 / @16 / @32 | max-Q over (rollout, step) @16 / @32 | pass@32 | + 2 fp32 polish steps, best-Q (fp32 head) |
MLP fp32 & 71.2 & 77.4 / 81.0 / 82.3 & 81.0 / 82.3 & 82.3 & 82.3 \\
MLP noise 0.1 s2 (K16) & 66.8 & 73.3 / 77.8 / - & 77.8 & - & 80.0 \\
MLP noise 0.15 s2 (K16, det. 36.8) & 36.4 & 48.3 / 56.7 / - & 69.2 & - & 74.6 \\
MLP noise 0.2 s2 (K16) & 10.2 & 15.5 / 22.0 / - & 37.5 & - & 72.4 \\
attn fp32 & 66.6 & 73.2 / 76.0 / 77.4 & 76.0 / 77.4 & 77.4 & 78.0 \\
attn w4c & 66.0 & 73.2 / 76.4 / 77.7 & 77.7 & 77.7 & 78.0 \\
attn noise 1.0 s2 & 0.3 & 0.7 / 2.4 / 3.3 & 10.2 / 11.1 & 3.8 & 35.5 \\
HRM fp32 & 49.6 & 55.2 / 59.1 / 61.4 & 61.5 & 61.5 & 61.6 \\
HRM w4c / w4t & 48.6 / 47.7 & 54.5 / 57.6 / 59.7; 53.3 / 58.4 / 60.1 & 59.7 / 60.1 & 59.8 / 60.1 & 60.3 / 60.4 \\
HRM noise 1.3 s0 & 7.8 & 12.4 / 15.5 / 16.9 & 17.0 & 18.8 & 25.0 \\


==> tables/bank/m5_rules.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/M5.md; header: | model | sel rule | fp32: fixed 16 -> sel (steps) | in-basin cells: sel delta, steps (speedup) | fixed depth on fp32 (0.5 pt) | edge cells: sel delta
TRM Sudoku-MLP & patience 2 & 70.8 $\to$ 70.8 (7.25 steps, 2.2x) & +0.0 [+0.0, +0.1], 7.6 steps (2.1x), n=8 & 16 (no shorter depth keeps accuracy) & +3.2 [+0.3, +8.3], 12.0 steps & head silent: 15.8 steps, delta 0 [-0.1, +3.2] \\
TRM Sudoku-attn & native & 66.0 $\to$ 65.5 (7.76, 2.1x) & -0.3 [-0.9, -0.1], 7.9 (2.0x), n=12 & 15 & -0.0 [-0.8, +1.7], 11.1 & silent: 15.3 \\
HRM Sudoku & min-step 4 + q>0 & 49.4 $\to$ 48.9 (10.7, 1.5x) & -0.7 [-1.2, -0.2], 10.8 (1.5x), n=9 & 15 & -0.9 [-2.0, -0.8], 11.7 & 15.0 \\
TRM Maze (exact) & min-step 2 + native & 87.0 $\to$ 87.0 (2.03, 7.9x) & +0.0 [-0.2, +0.4], 2.04 (7.8x), n=19 & 2 & -0.5 [-1.3, +0.3], 4.1 (vs depth 2: -8.2 [-12.3, -4.0]) & 14.6 \\
HRM Maze (exact) & min-step 2 + q>0 & 74.2 $\to$ 74.2 (2.53, 6.3x) & -0.2 [-2.6, +1.4], 2.54 (6.3x), n=20 & 4 & -5.1 [-14.6, +0.1], 4.1 & 16 \\


==> tables/bank/mt_B.tex <==
% generated by tables/bank/md2tex.py from reports/EDGETRM_MASTER_TABLES.md; header: | family / task (fp32) | w8c | w6c | w4g32 | w4c | w4a | w4t | w3g32 | w3a | w2g32 |
TRM attn, ARC-AGI-1 pass@1, H=3 n=16 (30.2) & 30.5 (0.99) & 31.5 (0.97) & 30.0 (0.93) & 28.7 (0.90) & 30.2 (0.91) & 20.2 (0.74) & 26.2 (0.83) & 23.0 (0.77) & 0.0 (0.14) \\
TRM attn, Sudoku-Extreme, H=3 n=16 (65.7) & 65.9 (0.95) & 67.1 (0.95) & 66.2 (0.94) & 66.2 (0.93) & 65.0 (0.92) & 62.8 (0.88) & 65.2 (0.89) & 62.0 (0.87) & 0.0 (0.20) \\
TRM MLP, Sudoku-Extreme, H=3 n=16 (71.4) & 71.0 (0.94) & 71.6 (0.92) & 69.0 (0.89) & 67.9 (0.86) & 69.5 (0.86) & 5.9 (0.30) & 51.4 (0.57) & 51.1 (0.59) & 0.0 (0.13) \\
HRM, Sudoku-Extreme, n=16 (51.0) & 51.3 (0.98) & 50.8 (0.97) & 51.7 (0.96) & 50.4 (0.96) & 50.8 (0.96) & 49.1 (0.93) & 50.1 (0.95) & 51.8 (0.94) & 15.1 (0.69) \\
TRM attn, Maze-Hard, H=3 n=16 (87.0) & 87.1 (1.00) & 87.0 (1.00) & 86.8 (1.00) & 86.9 (1.00) & 86.7 (1.00) & 86.2 (0.99) & 86.7 (1.00) & 86.6 (0.99) & 25.4 (0.76) \\
HRM, Maze-Hard, n=16 (74.1) & 74.4 (1.00) & 74.5 (1.00) & 74.0 (1.00) & 74.9 (1.00) & 74.6 (1.00) & 74.8 (0.99) & 74.4 (1.00) & 74.6 (0.99) & 60.8 (0.95) \\
Deep-thinking maze 33$\times$33, 100 iters (55.1) & 55.0 (1.00) & 54.3 (1.00) & 55.3 (0.99) & 44.4 (0.98) & 53.6 (0.99) & 41.3 (0.98) & 52.2 (0.97) & 47.8 (0.97) & 0.0 (0.50) \\
Deep-thinking chess (600k--700k), 60 iters (84.4) & 84.8 (1.00) & 84.3 (1.00) & 84.1 (0.99) & 75.0 (0.95) & 77.5 (0.97) & 0.4 (0.41) & 80.7 (0.98) & 21.6 (0.74) & 17.9 (0.75) \\
Deep-thinking prefix sums 512-bit, 100 iters (0.3) & 0.3 (1.00) & 0.3 (1.00) & 0.4 (1.00) & 0.4 (0.98) & 0.2 (0.99) & 0.2 (0.98) & 0.4 (0.98) & 0.2 (0.98) & 0.2 (0.90) \\


==> tables/bank/mt_D.tex <==
% generated by tables/bank/md2tex.py from reports/EDGETRM_MASTER_TABLES.md; header: | task | setting | w8c | w8c+a8 | w4g32 | w4g32+a8 | w4c | w4c+a8 |
ARC pass@1 (fp32 30.5) & H=3 n=1 & 30.2 (1.00) & 21.5 (0.87) & 27.8 (0.97) & 20.0 (0.85) & 27.8 (0.94) & 17.5 (0.83) \\
ARC pass@1 (fp32 30.2) & H=3 n=16 & 30.5 (0.99) & 25.2 (0.78) & 30.0 (0.93) & 21.5 (0.75) & 28.7 (0.90) & 20.0 (0.74) \\
Sudoku-MLP (fp32 28.4) & H=3 n=1 & 28.3 (1.00) & 14.6 (0.80) & 26.2 (0.92) & 13.2 (0.78) & 23.4 (0.86) & 13.1 (0.75) \\
Sudoku-MLP (fp32 71.4) & H=3 n=16 & 71.0 (0.94) & 72.2 (0.83) & 69.0 (0.89) & 70.3 (0.83) & 67.9 (0.86) & 68.7 (0.80) \\
Sudoku-attn (fp32 3.1) & H=3 n=1 & 3.1 (1.00) & 2.4 (0.99) & 2.7 (0.99) & 2.2 (0.98) & 2.3 (0.98) & 2.2 (0.97) \\
Sudoku-attn (fp32 65.7) & H=3 n=16 & 65.9 (0.95) & 66.8 (0.93) & 66.2 (0.94) & 66.8 (0.92) & 66.2 (0.93) & 66.7 (0.92) \\
HRM Sudoku (fp32 2.2) & H=3 n=1 & 2.2 (1.00) & 2.3 (1.00) & 2.2 (1.00) & 2.2 (1.00) & 2.2 (1.00) & 2.2 (0.99) \\
HRM Sudoku (fp32 51.0) & H=3 n=16 & 51.3 (0.98) & 51.6 (0.96) & 51.7 (0.96) & 52.3 (0.95) & 50.4 (0.96) & 52.1 (0.95) \\
Maze-attn (fp32 78.5) & H=3 n=1 & 78.4 (1.00) & 77.5 (1.00) & 78.1 (1.00) & 77.9 (1.00) & 78.3 (1.00) & 78.1 (1.00) \\
Maze-attn (fp32 87.0) & H=3 n=16 & 87.1 (1.00) & 87.2 (1.00) & 86.8 (1.00) & 86.8 (1.00) & 86.9 (1.00) & 87.1 (1.00) \\
HRM Maze (fp32 59.6) & H=3 n=1 & 59.7 (1.00) & 58.0 (0.99) & 59.7 (1.00) & 56.9 (0.99) & 60.2 (1.00) & 58.1 (0.99) \\
HRM Maze (fp32 74.1) & H=3 n=16 & 74.4 (1.00) & 75.1 (1.00) & 74.0 (1.00) & 74.4 (1.00) & 74.9 (1.00) & 75.0 (0.99) \\


==> tables/bank/mt_E.tex <==
% generated by tables/bank/md2tex.py from reports/EDGETRM_MASTER_TABLES.md; header: | model, depth | bf16 | w8c | w6c | w4g32 | w4c | w4a | w4t | w3a |
Huginn-0125, 4 steps & 0.5 [200] nll 1.26 & 0.5 [200] nll 1.26 $\varphi$ 0.96 & 2.5 [200] nll 1.26 $\varphi$ 0.96 & 1.0 [200] nll 1.27 $\varphi$ 0.95 & 1.5 [200] nll 1.30 $\varphi$ 0.92 & 1.5 [200] nll 1.31 $\varphi$ 0.93 & 1.5 [200] nll 1.80 $\varphi$ 0.74 & 0.0 [200] nll 1.60 $\varphi$ 0.80 \\
Huginn-0125, 8 steps & 13.0 [200] nll 0.86 & 17.5 [200] nll 0.86 $\varphi$ 0.99 & 11.0 [200] nll 0.86 $\varphi$ 0.99 & 15.5 [200] nll 0.87 $\varphi$ 0.97 & 11.0 [200] nll 0.90 $\varphi$ 0.93 & 8.5 [200] nll 0.92 $\varphi$ 0.95 & 1.5 [200] nll 1.34 $\varphi$ 0.70 & 2.0 [200] nll 1.05 $\varphi$ 0.78 \\
Huginn-0125, 16 steps & 40.0 [200] nll 0.83 & 37.5 [200] nll 0.83 $\varphi$ 1.00 & -- nll 0.83 $\varphi$ 0.99 & 35.0 [200] nll 0.84 $\varphi$ 0.98 & 27.5 [200] nll 0.82 $\varphi$ 0.93 & -- nll 0.91 $\varphi$ 0.95 & -- nll 1.24 $\varphi$ 0.70 & 2.5 [200] nll 0.98 $\varphi$ 0.78 \\
Huginn-0125, 32 steps & 40.0 [100] nll 0.84 & 40.0 [100] nll 0.84 $\varphi$ 1.00 & -- nll 0.83 $\varphi$ 1.00 & 32.0 [100] nll 0.84 $\varphi$ 0.98 & 27.0 [100] nll 0.81 $\varphi$ 0.93 & -- nll 0.91 $\varphi$ 0.95 & -- nll 1.24 $\varphi$ 0.70 & 5.0 [100] nll 0.98 $\varphi$ 0.78 \\
Huginn-0125, 64 steps & 40.0 [50] nll 0.85 & 42.0 [50] nll 0.85 $\varphi$ 1.00 & -- nll 0.84 $\varphi$ 1.00 & 30.0 [50] nll 0.85 $\varphi$ 0.98 & 26.0 [50] nll 0.81 $\varphi$ 0.93 & -- nll 0.91 $\varphi$ 0.95 & -- nll 1.24 $\varphi$ 0.70 & 6.0 [50] nll 0.99 $\varphi$ 0.78 \\
Ouro-1.4B, 1 loops & 45.5 [200] nll 1.81 & 47.0 [200] nll 1.81 $\varphi$ 1.00 & 41.0 [200] nll 1.87 $\varphi$ 0.98 & 31.5 [200] nll 2.04 $\varphi$ 0.90 & 0.0 [200] nll 3.20 $\varphi$ 0.73 & -- nll 2.77 $\varphi$ 0.80 & -- nll 11.89 $\varphi$ 0.02 & 0.5 [200] nll 6.48 $\varphi$ 0.28 \\
Ouro-1.4B, 2 loops & 80.0 [200] nll 1.05 & 77.0 [200] nll 1.06 $\varphi$ 1.00 & -- nll 1.08 $\varphi$ 0.98 & 68.5 [200] nll 1.10 $\varphi$ 0.89 & 9.5 [200] nll 1.65 $\varphi$ 0.71 & -- nll 1.33 $\varphi$ 0.78 & -- nll 12.58 $\varphi$ 0.01 & 0.0 [200] nll 5.37 $\varphi$ 0.23 \\
Ouro-1.4B, 3 loops & 76.0 [100] nll 0.88 & 77.0 [100] nll 0.88 $\varphi$ 1.00 & -- nll 0.89 $\varphi$ 0.98 & 72.0 [100] nll 0.89 $\varphi$ 0.89 & 0.0 [100] nll 1.10 $\varphi$ 0.73 & -- nll 0.97 $\varphi$ 0.79 & -- nll 12.93 $\varphi$ 0.01 & 0.0 [100] nll 5.64 $\varphi$ 0.18 \\
Ouro-1.4B, 4 loops & 75.0 [100] nll 0.88 & 76.0 [100] nll 0.88 $\varphi$ 1.00 & -- nll 0.90 $\varphi$ 0.97 & 76.0 [100] nll 0.89 $\varphi$ 0.89 & 4.0 [100] nll 1.04 $\varphi$ 0.74 & -- nll 0.93 $\varphi$ 0.79 & -- nll 13.00 $\varphi$ 0.00 & 0.0 [100] nll 5.53 $\varphi$ 0.16 \\
Ouro-1.4B, 6 loops & 63.0 [100] nll 0.88 & 66.0 [100] nll 0.87 $\varphi$ 1.00 & -- nll 0.89 $\varphi$ 0.98 & 66.0 [100] nll 0.88 $\varphi$ 0.90 & 2.0 [100] nll 1.23 $\varphi$ 0.73 & -- nll 1.44 $\varphi$ 0.51 & -- nll 12.90 $\varphi$ 0.00 & 0.0 [100] nll 5.57 $\varphi$ 0.22 \\
Ouro-1.4B, 8 loops & 68.0 [100] nll 0.90 & 65.0 [100] nll 0.89 $\varphi$ 1.00 & -- nll 0.90 $\varphi$ 0.97 & 49.0 [100] nll 0.88 $\varphi$ 0.89 & 2.0 [100] nll 1.41 $\varphi$ 0.70 & -- nll 1.76 $\varphi$ 0.49 & -- nll 12.81 $\varphi$ 0.00 & 0.0 [100] nll 5.86 $\varphi$ 0.20 \\
Ouro-2.6B, 1 loops & 51.0 [200] nll 1.39 & 49.0 [200] nll 1.40 $\varphi$ 1.00 & 44.5 [200] nll 1.40 $\varphi$ 0.99 & 47.0 [200] nll 1.45 $\varphi$ 0.92 & 29.0 [200] nll 1.60 $\varphi$ 0.81 & -- nll 1.41 $\varphi$ 0.85 & -- nll 11.24 $\varphi$ 0.03 & 0.0 [200] nll 4.02 $\varphi$ 0.43 \\
Ouro-2.6B, 2 loops & 47.0 [200] nll 0.94 & 48.0 [200] nll 0.95 $\varphi$ 1.00 & -- nll 0.94 $\varphi$ 0.99 & 51.0 [200] nll 0.97 $\varphi$ 0.92 & 36.0 [200] nll 1.00 $\varphi$ 0.81 & -- nll 0.96 $\varphi$ 0.85 & -- nll 11.81 $\varphi$ 0.02 & 0.0 [200] nll 3.15 $\varphi$ 0.33 \\
Ouro-2.6B, 3 loops & 64.0 [100] nll 0.82 & 63.0 [100] nll 0.82 $\varphi$ 1.00 & -- nll 0.81 $\varphi$ 0.99 & 65.0 [100] nll 0.85 $\varphi$ 0.93 & 73.0 [100] nll 0.88 $\varphi$ 0.85 & -- nll 0.86 $\varphi$ 0.86 & -- nll 12.26 $\varphi$ 0.01 & 0.0 [100] nll 2.99 $\varphi$ 0.33 \\
Ouro-2.6B, 4 loops & 80.0 [100] nll 0.80 & 81.0 [100] nll 0.80 $\varphi$ 1.00 & -- nll 0.80 $\varphi$ 0.98 & 68.0 [100] nll 0.83 $\varphi$ 0.92 & 78.0 [100] nll 0.83 $\varphi$ 0.85 & -- nll 0.85 $\varphi$ 0.87 & -- nll 12.75 $\varphi$ 0.01 & 0.0 [100] nll 3.00 $\varphi$ 0.35 \\
Ouro-2.6B, 6 loops & 75.0 [100] nll 0.82 & 78.0 [100] nll 0.82 $\varphi$ 1.00 & -- nll 0.82 $\varphi$ 0.98 & 71.0 [100] nll 0.84 $\varphi$ 0.91 & 64.0 [100] nll 0.85 $\varphi$ 0.84 & -- nll 0.86 $\varphi$ 0.86 & -- nll 13.23 $\varphi$ 0.02 & 0.0 [100] nll 3.74 $\varphi$ 0.33 \\
Ouro-2.6B, 8 loops & 62.0 [100] nll 0.85 & 68.0 [100] nll 0.85 $\varphi$ 1.00 & -- nll 0.84 $\varphi$ 0.98 & 46.0 [100] nll 0.89 $\varphi$ 0.90 & 43.0 [100] nll 0.91 $\varphi$ 0.83 & -- nll 0.91 $\varphi$ 0.83 & -- nll 13.08 $\varphi$ 0.02 & 0.0 [100] nll 4.87 $\varphi$ 0.27 \\


==> tables/bank/mt_G_pivot.tex <==
% generated by tables/bank/md2tex.py from reports/EDGETRM_MASTER_TABLES.md section G (AI Hub, H=3 step graphs); columns: task, device, fp32 ms, int8 ms, int4 ms, int4 peak MB
arc & Samsung Galaxy S24 & 150.37 & 75.34 & \redtext{58.96} & \redtext{98.5} \\
arc & Samsung Galaxy S26 & 106.81 & 50.37 & \redtext{38.33} & \redtext{142.6} \\
arc & Snapdragon 8 Elite QRD & 144.02 & 59.52 & \redtext{48.03} & \redtext{119.8} \\
arc & Snapdragon X2 Elite CRD & 113.00 & 54.64 & \redtext{42.23} & \redtext{16.8} \\
arc & Dragonwing RB3 Gen 2 Vision Kit & -- & -- & \redtext{290.76} & \redtext{7.7} \\
arc & Google Pixel 8 & 519.10 & -- & -- & -- \\
arc & Arduino VENTUNO Q & 205.53 & 91.58 & \redtext{70.97} & \redtext{6.0} \\
arc & Samsung Galaxy S21 & -- & -- & \redtext{192.42} & \redtext{97.6} \\
maze & Samsung Galaxy S24 & 150.17 & 71.28 & \redtext{56.18} & \redtext{100.9} \\
maze & Samsung Galaxy S26 & 106.82 & 49.16 & \redtext{38.87} & \redtext{143.1} \\
maze & Snapdragon 8 Elite QRD & 127.30 & 57.58 & \redtext{39.31} & \redtext{119.6} \\
maze & Snapdragon X2 Elite CRD & 114.81 & 53.84 & \redtext{44.76} & \redtext{16.8} \\
maze & Dragonwing RB3 Gen 2 Vision Kit & -- & -- & \redtext{276.09} & \redtext{7.3} \\
maze & Google Pixel 8 & 509.99 & -- & -- & -- \\
maze & Arduino VENTUNO Q & 205.52 & 89.65 & \redtext{68.89} & \redtext{6.0} \\
maze & Samsung Galaxy S21 & -- & -- & \redtext{179.15} & \redtext{99.1} \\
sudoku attn & Samsung Galaxy S24 & 9.06 & 11.38 & \redtext{7.15} & \redtext{96.8} \\
sudoku attn & Samsung Galaxy S26 & 6.07 & 6.23 & \redtext{3.88} & \redtext{140.1} \\
sudoku attn & Snapdragon 8 Elite QRD & 9.25 & 8.83 & \redtext{6.41} & \redtext{118.1} \\
sudoku attn & Snapdragon X2 Elite CRD & 6.32 & 7.07 & \redtext{4.59} & \redtext{15.6} \\
sudoku attn & Dragonwing RB3 Gen 2 Vision Kit & -- & -- & \redtext{60.14} & \redtext{6.6} \\
sudoku attn & Google Pixel 8 & -- & -- & -- & -- \\
sudoku attn & Arduino VENTUNO Q & 15.33 & 15.24 & \redtext{9.82} & \redtext{4.9} \\
sudoku attn & Samsung Galaxy S21 & -- & -- & \redtext{35.23} & \redtext{96.0} \\
sudoku mlp & Samsung Galaxy S24 & 11.37 & 10.27 & \redtext{6.78} & \redtext{96.4} \\
sudoku mlp & Samsung Galaxy S26 & 9.55 & 6.68 & \redtext{4.62} & \redtext{140.2} \\
sudoku mlp & Snapdragon 8 Elite QRD & 13.62 & 9.66 & \redtext{5.96} & \redtext{117.9} \\
sudoku mlp & Snapdragon X2 Elite CRD & 10.22 & 7.43 & \redtext{5.19} & \redtext{15.1} \\
sudoku mlp & Dragonwing RB3 Gen 2 Vision Kit & -- & -- & \redtext{49.40} & \redtext{4.5} \\
sudoku mlp & Google Pixel 8 & 59.96 & 57.70 & -- & -- \\
sudoku mlp & Arduino VENTUNO Q & 17.94 & 13.57 & \redtext{9.25} & \redtext{4.8} \\
sudoku mlp & Samsung Galaxy S21 & -- & -- & \redtext{29.35} & \redtext{96.0} \\


==> tables/bank/x1_captax33.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X1.md; header: | size 33 | acc@500 | A [95%] | ΔA vs fp32 [95%] | log(tau/tau_fp32) [95%] | log(T90/T90_fp32) [95%] |
fp32 & 100.0 & 100.0 &  &  & (T90 = 178) \\
w8c / w6c / w4g32 / w4g128 & 99.9-100 & 100.0 & 0.0 & +0.04 / +0.04 / 0.00 / +0.04 (all span 0) & 0.00 / 0.00 / 0.00 / 0.00 \\
w4a & 100.0 & 100.0 & 0.0 & +0.04 [-0.13,+0.08] & +0.03 [+0.02,+0.04] \\
w4c & 98.9 & 100.0 & 0.0 & -0.04 [-0.13,+0.13] & +0.07 [+0.05,+0.09] \\
w4t & 88.4 & 92.0 [89.6,94.6] & -8.0 [-10.4,-5.4] & +0.13 [+0.04,+0.29] & +0.06 [+0.04,+0.08] \\
w3a & 95.3 & 98.0 [96.9,100] & -2.0 [-3.1,0.0] & +0.04 [0.00,+0.25] & +0.07 [+0.05,+0.08] \\
noise 0.2 (1 draw) & 57.2 & 60.2 [55.6,63.3] & -39.8 [-44.4,-36.7] & +0.29 [-0.25,+0.46] & +0.22 [+0.13,+0.30] \\
noise 0.3 (1 draw) & 74.8 & 78.3 [75.1,81.1] & -21.7 [-24.9,-18.9] & +0.21 [0.00,+0.34] & +0.10 [+0.07,+0.13] \\


==> tables/bank/x1_deep512.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X1.md; header: | model, quant | res 0 | res 1-45 | res 46-50 | res 51-55 | res >= 56 |
MLP fp32 & 98.7 / 99.1 / 99.1 & 94.7 / 95.5 / 96.7 & 87.1 / 89.7 / 91.5 & 72.7 / 78.5 / 83.4 & 60.8 / 67.5 / 76.1 \\
MLP w3g32 ($\varphi$ 0.54) & 96.4 / 95.6 / 94.2; -4.9 [-8,-2] & 82.9 / 84.6 / 83.7; -13.0 & 62.5 / 62.5 / 65.2; -26.3 & 47.3 / 49.5 / 50.5; -32.9 & 41.2 / 44.1 / 46.9; -29.2 [-33,-25] \\
attn fp32 & 99.1 / 99.1 / 100 & 91.9 / 95.1 / 97.2 & 90.2 / 91.1 / 93.3 & 71.8 / 81.3 / 88.4 & 61.6 / 71.9 / 78.4 \\
attn w3c ($\varphi$ 0.85) & 88.0 / 92.9 / 95.6; -4.4 [-7,-2] & 87.0 / 90.7 / 92.7; -4.5 & 77.7 / 84.4 / 87.5; -5.8 & 55.5 / 70.1 / 83.9; -4.5 [-8,-1] & 54.8 / 70.3 / 85.2; \textbf{+6.7 [+3,+10]} \\
MLP w4c ($\varphi$ 0.87) & 99.6 / 99.6 / 99.6; +0.4 & 93.9 / 95.5 / 95.5; -1.2 [-3,0] & 83.0 / 86.2 / 88.4; -3.1 [-6,0] & 64.3 / 70.8 / 75.5; -8.0 [-11,-5] & 58.3 / 64.1 / 70.5; -5.6 [-8,-3] \\
attn w4c ($\varphi$ 0.94) & 98.2 / 99.1 / 99.6; -0.4 & 91.9 / 95.5 / 97.2; 0.0 & 88.4 / 92.0 / 93.8; +0.4 & 73.8 / 81.1 / 87.5; -0.9 [-3,+1] & 59.7 / 71.1 / 79.4; +0.9 [-1,+3] \\
MLP w4t ($\varphi$ 0.28) & 32.9 / 32.4 / 32.4; -66.7 & 6.5 / 6.9 / 7.3 & 0.4 / 0.9 / 0.4 & 0.4 / 0.9 / 0.9 & 0.0 / 0.0 / 0.3; -75.8 \\
attn w4t (edge) & 98.2 / 98.2 / 98.2; -1.8 [-4,0] & 89.8 / 91.1 / 93.5; -3.7 [-6,-1] & 83.5 / 87.9 / 92.9; -0.4 & 62.8 / 73.3 / 82.2; -6.2 [-10,-3] & 56.4 / 65.9 / 73.9; -4.5 [-8,-2] \\
HRM fp32 & 93.3 / 95.1 / 95.1 & 83.3 / 89.0 / 91.5 & 71.0 / 75.9 / 80.4 & 43.2 / 51.8 / 59.1 & 33.0 / 38.6 / 44.1 \\
HRM w2g32 ($\varphi$ 0.66) & 58.7 / 61.3 / 61.8; -33.3 & 24.0 / 26.0 / 26.8; -64.6 & 13.4 / 16.5 / 17.0; -63.4 & 5.6 / 6.5 / 6.7; -52.5 & 5.8 / 7.2 / 7.7; -36.4 [-40,-32] \\


==> tables/bank/x1_readoutA.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X1.md; header: | model | quantizer | nsup 16 | nsup 64 | gain 16->64 | gap to fp32 at 64 [95% CI] (easy / med / hard) |
MLP & fp32 & 97.8 / 66.7 / 53.7 & 98.9 / 73.8 / 57.3 & +1.1 / +7.1 / +3.6 &  \\
MLP & w8c & 98.1 / 66.7 / 52.0 & 98.5 / 73.6 / 58.4 & +0.4 / +6.9 / +6.4 & -0.4 / -0.2 / +1.1 (all CIs span 0) \\
MLP & w4c & 96.3 / 63.3 / 48.0 & 97.8 / 67.6 / 52.3 & +1.5 / +4.2 / +4.3 & -1.1 [-3,+1] / -6.2 [-10,-3] / -5.0 [-9,-1] \\
MLP & w3g32 (edge) & 83.3 / 44.2 / 32.4 & 84.0 / 44.7 / 33.1 & +0.7 / +0.4 / +0.7 & -14.9 / -29.1 / -24.2 \\
MLP & w3c (out) & 53.2 / 5.1 / 2.5 & 53.5 / 6.0 / 3.6 & +0.4 / +0.9 / +1.1 & -45.4 / -67.8 / -53.7 \\
attn & fp32 & 94.4 / 59.3 / 48.4 & 97.8 / 65.6 / 59.1 & +3.3 / +6.2 / +10.7 &  \\
attn & w4c & 94.4 / 58.9 / 50.9 & 97.0 / 64.2 / 60.1 & +2.6 / +5.3 / +9.3 & -0.7 / -1.3 / +1.1 (span 0) \\
attn & w4t (edge) & 90.0 / 55.8 / 48.0 & 92.6 / 63.6 / 53.4 & +2.6 / +7.8 / +5.3 & -5.2 [-8,-2] / -2.0 [-5,+1] / -5.7 [-10,-1] \\
attn & w3c (edge) & 81.8 / 58.4 / 43.8 & 87.0 / 69.3 / 58.0 & +5.2 / +10.9 / +14.2 & -10.8 [-15,-7] / +3.8 [-0,+8] / -1.1 [-6,+4] \\
HRM & fp32 & 80.3 / 41.1 / 32.4 & 83.6 / 45.3 / 37.7 & +3.3 / +4.2 / +5.3 &  \\
HRM & w4c & 79.2 / 41.3 / 32.0 & 85.9 / 46.0 / 36.7 & +6.7 / +4.7 / +4.6 & +2.2 / +0.7 / -1.1 (span 0) \\
HRM & w4t & 77.0 / 41.1 / 27.4 & 85.1 / 45.1 / 37.7 & +8.2 / +4.0 / +10.3 & +1.5 / -0.2 / 0.0 (span 0; hard was -5.0 at 16) \\
HRM & w2g32 (edge) & 32.3 / 9.3 / 5.0 & 37.2 / 10.4 / 5.3 & +4.8 / +1.1 / +0.4 & -46.5 / -34.9 / -32.4 \\


==> tables/bank/x1_strat64.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X1.md; header: | quant | res 0 | res 1-45 | res 46-50 | res 51-55 | res >= 56 |
fp32 & 99.7 (+0.4) & 97.3 (+0.7) & 89.2 (+2.5) & 76.6 (+5.9) & 70.0 (+6.7) \\
w8c ($\varphi$ 0.93) & 0.0 & 0.0 & +0.8 [0,+2] & 0.0 & +0.7 [0,+2] \\
w4g32 ($\varphi$ 0.89) & 0.0 & -0.1 & -2.1 [-4,-1] & -2.2 [-4,-1] & -2.5 [-4,-1] \\
w4c ($\varphi$ 0.87) & 0.0 & -0.4 & -2.1 [-4,-1] & -5.6 [-8,-4] (+5.0) & -4.2 [-6,-2] (+5.9) \\
w3g32 ($\varphi$ 0.55) & -3.8 & -15.7 & -25.2 & -27.3 (+3.0) & -25.7 (+2.3) \\
w3a ($\varphi$ 0.60) & -6.4 & -13.4 & -21.0 & -36.1 (+9.1) & -24.5 (+10.3) \\
w4t / w3c & 36.0 / 69.8 abs. & 7.6 / 32.3 & 2.5 / 14.9 & 0.6 / 4.8 & 0.4 / 5.2 \\


==> tables/bank/x2_attn.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X2.md; header: | sigma | acc (%) | rho(J_T) solved | frac Lambda<1 | kick growth (random, 16 steps) | residual | basin switch |
0.1 & 74.6 / 72.7 / 73.0 & 1.29 / 1.24 / 1.24 & 0.40 / 0.38 / 0.38 & 0.10 / 0.07 / 0.08 & 0.08 / 0.07 / 0.06 & 0.03 / 0.02 / 0.02 \\
0.3 & 69.5 / 75.0 / 73.4 & 1.00 / 1.68 / 1.08 & 0.54 / 0.18 / 0.49 & 0.01 / 0.38 / 0.03 & 0.01 / 0.12 / 0.03 & 0.02 / 0.03 / 0.02 \\
0.5 & 67.2 / 68.8 / 62.5 & 1.27 / 1.39 / 1.90 & 0.38 / 0.39 / 0.15 & 0.07 / 0.11 / 1.72 & 0.06 / 0.06 / 0.14 & 0.02 / 0.01 / 0.04 \\
0.7 & 54.3 / 52.3 / 47.7 & 1.55 / 1.99 / 1.91 & 0.21 / 0.16 / 0.11 & 1.38 / 2.64 / 20.2 & 0.15 / 0.16 / 0.25 & 0.03 / 0.04 / 0.05 \\
1.0 & 5.1 / 8.2 / 15.6 & 2.02 / 2.17 / 1.39 & 0.12 / 0.20 / 0.29 & 1.83 / 1.96 / 1.28 & 0.16 / 0.17 / 0.18 & 0.32 / 0.39 / 0.30 \\


==> tables/bank/x2_edge.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X2.md; header: | model | sigma_1/2 | rho fp32 | rho near sigma_1/2 | verdict |
HRM Sudoku & 1.05 & 0.88 & 1.00 / 1.02 / 0.99 (sigma 1.0); 1.26-1.36 at 1.5 & \textbf{yes} \\
TRM Maze & 1.71 & 0.74 & 0.89 / 0.65 / 0.85 (1.5); 0.88 / 1.08 / 1.01 (2.0, acc 0-2\%) & roughly: crosses between 1.5 and 2.0 \\
TRM Sudoku attention & 0.80 & 1.24 & 1.55 / 1.99 / 1.91 (0.7) & no: above 1 already in fp32 \\
TRM Sudoku MLP & 0.14 & 1.65 & 1.86 / 2.13 / 1.78 (0.15) & no: above 1 already in fp32 \\
DT maze 13 / 33 & 0.37 / 0.26 & 0.98 / 1.01 & 0.97-1.02 / 1.02-1.14 (0.3) & no: marginal ($\sim$1) throughout \\


==> tables/bank/x2_rho.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X2.md; header: | model | acc | rho all / solved / unsolved | solved with rho < 1 | FTLE Lambda solved / unsolved | ||J||_2 solved | random-kick growth (16 steps) sol
TRM Sudoku MLP & 71.5 & 1.88 / 1.65 / 4.80 & 0\% & 1.10 / 5.11 & 8.6 & 0.32 & 0.045 \\
TRM Sudoku attention & 72.7 & 1.38 / 1.24 / 3.76 & 17\% & 1.00 / 4.52 & 13.6 & 0.04 & 0.051 \\
HRM Sudoku & 47.7 & 1.17 / 0.88 / 1.84 & 79\% & 0.79 / 1.48 & 7.2 & 0.005 & 0.006 \\
TRM Maze attention & 87.5 & 0.74 / 0.74 / 0.83 & 79\% & 0.64 / 0.69 & 9.0 & 0.003 & 0.000 \\
DT maze 13 / 33 (map G) & 100 / 100 & 0.98 / 1.01 & -- & 0.96 / 0.99 & 3.9 / 4.0 & 0.03 / 0.04 & 0.13 / 0.11 \\
DT maze 33 (map G o G) & 100 & 0.98 & -- & 0.98 & 7.1 & 0.02 & 0.002 \\


==> tables/bank/x2_sens.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X2.md; header: | model | sigma_1/2 | S | delta_T at sigma_1/2 | S x sigma_1/2 | sigma* = delta*/S (delta* = geo-mean of the other models) |
TRM Sudoku MLP & 0.14 & 1.60 & 0.44 & 0.22 & 0.25 \\
TRM Sudoku attention & 0.80 & 0.68 & 0.59 & 0.54 & 0.48 \\
HRM Sudoku & 1.05 & 0.35 & 0.38 & 0.37 & 1.01 \\
TRM Maze & 1.71 & 0.32 & 0.58 & 0.55 & 1.03 \\
DT maze 13 & 0.37 & 0.94 & 0.37 & 0.35 & 0.38 \\
DT maze 33 & 0.26 & 0.96 & 0.24 & 0.25 & 0.40 \\


==> tables/bank/x3_ablate.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X3.md; header: | Row | activation change (everything else as stated) | exact /100 | cell % | runtime |
A0 & w8a16 unmodified & 66 & 86.8 & ORT-fused \\
A1 (a) & carry I/O (z\_H, z\_L in and out) at 8 bit & 65 & 86.9 & ORT-fused \\
A4 (d) & extra 8-bit Q/DQ on every MatMul activation input only (the harness's +a8), 57 edges & 70 & 87.9 & ORT-fused \\
\textbf{A2b (b)} & \textbf{RMSNorm mean(x\^{}2)+eps, sqrt, 1/sqrt (and their constants) at 8 bit, 169 tensors} & \textbf{0} & \textbf{54.0} & ORT-fused \\
A8 & all 555 activation tensors at 8 bit (= the AI Hub w8a8 graph, same numbers) & 0 & 41.9 & ORT-fused \\
A2a & RMSNorm x$\ast$x only, 28 tensors & 58 & 85.6 & ORT-fused \\
A2c & RMSNorm output only & 65 & 86.6 & ORT-fused \\
A2 & all RMSNorm tensors & 0 & 51.6 & ORT-fused \\
A3 (c) & residual and injection adds, 71 tensors & 71 & 88.0 & ORT-fused \\
A6 & SwiGLU product (down\_proj input), 28 tensors & 74 & 89.5 & ORT-fused \\
A2b2 & as A2b without the embed-scale scalar (the cross-mixer definition), 168 tensors & 0 & 54.0 & ORT-fused \\
B2b / B2b2 & all 8 bit except the RMSNorm variance path at 16 & 0 & 46.4 & ORT-fused \\
B2a & all 8 bit except x$\ast$x at 16 & 0 & 41.7 & ORT-fused \\
B3 & all 8 bit except residual/inject adds at 16 & 0 & 41.0 & ORT-fused \\
B6 & all 8 bit except SwiGLU product at 16 & 0 & 41.7 & ORT-fused \\
\textbf{B2} & \textbf{all 8 bit except every RMSNorm tensor (x$\ast$x, mean+eps, sqrt, 1/sqrt, output, constants) at 16} & \textbf{69} & \textbf{88.0} & ORT-fused \\
B2ab & all 8 bit except x$\ast$x + variance path at 16 (RMSNorm output at 8) & 0 & 48.6 & ORT-fused \\
A5 (e), A6b, A7, other B rows, unions B23/B26/B236 & running & - & - & ORT-fused \\
1000-puzzle (indices 1000-1999): B2, A2b2; w8a8, w8a16 & running & - & - & ORT-fused \\


==> tables/bank/x3_cross.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X3.md; header: | Model | fp32 | w8a16 | A2b2: RMSNorm variance path at 8 bit | w8a8 |
Sudoku-MLP & 68 & 66 (70) & \textbf{0} (cell 54.0) & 0 \\
Sudoku-attn & 65 & 65 & \textbf{70} (cell 88.6) & 69 \\


==> tables/bank/x3_cross_ranges.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X3.md; header: | group | Sudoku-MLP max abs / median max/std / 8-bit step/std | Sudoku-attn max abs / median max/std / 8-bit step/std |
residual & 59.2 / 9.8 / 0.058 & 11.4 / 6.0 / 0.041 \\
rms\_sq (x$\ast$x) & 3502 / 33.2 / 0.125 & 130 / 22.6 / 0.077 \\
rms\_var (mean, +eps) & 1673 / 12.7 / 0.053 & 7.7 / 8.4 / 0.035 \\
rms\_rsqrt & 40.9 / 8.9 / 0.034 & 2.77 / 11.4 / 0.047 \\
rms\_out & 9.2 / 7.8 / 0.044 & 5.9 / 5.4 / 0.037 \\
swiglu\_prod & 113.7 / 38.7 / 0.279 & 42.3 / 47.8 / 0.283 \\


==> tables/bank/x3_groups.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X3.md; header: | group | tensors | max abs | median std | median max/std | max max/std | median 8-bit step/std | median fraction within half a step of the mean |
carry\_in & 2 & 5.8 & 0.99 & 5.4 & 5.9 & 0.041 & 0.017 \\
embed & 6 & 3.3 & 0.03 & 4.1 & 10.9 & 0.038 & 0.022 \\
inject & 15 & 11.2 & 1.92 & 5.8 & 6.5 & 0.037 & 0.015 \\
residual & 56 & 59.2 & 1.91 & 9.8 & 18.9 & 0.058 & 0.029 \\
rms\_sq (x$\ast$x) & 28 & 3502.1 & 9.12 & 33.2 & 61.9 & 0.125 & 0.056 \\
rms\_var (mean, +eps) & 56 & 1672.7 & 4.25 & 12.7 & 31.9 & 0.053 & 0.016 \\
rms\_rsqrt & 56 & 40.9 & 0.46 & 8.9 & 18.0 & 0.034 & 0.016 \\
rms\_out & 76 & 9.2 & 0.98 & 7.8 & 9.3 & 0.044 & 0.016 \\
linear\_out & 112 & 59.2 & 1.40 & 9.6 & 25.5 & 0.084 & 0.051 \\
swiglu\_other (halves, sigmoid, silu) & 56 & 35.7 & 0.56 & 5.3 & 28.4 & 0.020 & 0.006 \\
\textbf{swiglu\_prod (silu(gate)$\ast$up = down\_proj input)} & 28 & 113.7 & 1.11 & \textbf{38.7} & \textbf{106.3} & \textbf{0.279} & \textbf{0.498} \\
head & 3 & 129.7 & 3.58 & 2.4 & 3.6 & 0.016 & 0.000 \\


==> tables/bank/x4_boundary.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X4.md; header: | model, 4 loops | fidelity | gold NLL (bf16) | ΔNLL | top-1 agree w/ bf16 | greedy acc (bf16) | retained |
Ouro-1.4B w4c & 0.736 & 1.054 (0.893) & +0.160 (+18\%) & 0.844 & 7.5 (78.0) & 10\% \\
Ouro-1.4B w4t & 0.004 & 13.0 (0.893) & +12.1 & 0.000 & 0.0 (78.0) & 0\% \\
Ouro-2.6B w4c & 0.853 & 0.838 (0.810) & +0.028 (+3\%) & 0.922 & 77.5 (82.5) & 94\% \\
Ouro-2.6B w4t & 0.010 & 12.7 (0.810) & +11.9 & 0.000 & 0.0 (82.5) & 0\% \\


==> tables/bank/x4_olmo.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X4.md; header: | loops | bf16 | w8c | w4g32 | w4c | w4t |
4 & 44.0, NLL 0.79 & 43.0, $\varphi$ 1.00 & 41.0, $\varphi$ 0.98 & 31.0, $\varphi$ 0.942, $\Delta$NLL +0.058 & 0.0, $\varphi$ 0.12, NLL 10.4 \\
8 & 44.0, NLL 0.78 & 51.0, $\varphi$ 1.00 & 40.0, $\varphi$ 0.98 & 37.0, $\varphi$ 0.947, +0.062 & 0.0, $\varphi$ 0.11 \\
16 & 45.0, NLL 0.78 & 47.0, $\varphi$ 1.00 & 41.0, $\varphi$ 0.98 & 36.0, $\varphi$ 0.947, +0.063 & 0.0, $\varphi$ 0.12 \\
32 & 42.0, NLL 0.78 & 44.0, $\varphi$ 1.00 & 42.0, $\varphi$ 0.98 & 38.0, $\varphi$ 0.946, +0.063 & 0.0, $\varphi$ 0.11 \\


==> tables/bank/x4_q6.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X4.md; header: | decode | bf16 acc | w4c acc [95% CI] | w4c degenerate / loop / capped | w4t acc |
greedy & 78.0 & 7.5 [4.6--12.0] & 86.5 / 62.5 / 96.0 & 0.0 \\
rep 1.1 & 75.5 & 15.0 [10.7--20.6] & 61.5 / 26.0 / 66.5 & 0.0 \\
rep 1.3 & 27.5 & 1.5 [0.5--4.3] & 32.5 / 18.5 / 34.5 & 0.0 \\
no-repeat-3gram & 2.0 & 2.5 [1.1--5.7] & 9.0 / 0.0 / 25.0 & 0.0 \\


==> tables/bank/x6_ddpm.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X6.md; header: | sigma / quant (rel. err) | DDIM 10 | DDIM 25 | DDIM 50 | DDIM 100 | DDPM 50 | DDPM 100 | DDPM 250 |
0.01 & 7.4 & 6.6 & 6.1 & 6.7 & 1.5 & 2.1 & 2.6 \\
0.02 & 17.1 & 13.0 & 11.7 & 18.0 & 3.7 & 4.5 & 5.3 \\
0.03 & 26.5 & 17.0 & 17.2 & 49.8 & 6.2 & 7.1 & 7.9 \\
0.05 & 45.7 & 21.2 & 61.4 & 189.5 & 12.7 & 13.3 & 13.8 \\
0.1 & 95.6 & 136.5 & 345.8 & 397.6 & 43.2 & 42.8 & 42.1 \\
0.2 & 283 & 346 & 354 & 356 & 144 & 167 & 185 \\
0.3 & 386 & 358 & 356 & 312 & 213 & 255 & 290 \\
w8c (0.010) & 6.4 & 5.4 & 5.0 & 6.0 & 2.0 & 2.6 & 3.2 \\
w4g32 (0.105) & 39.5 & 49.5 & 164 & 304 & 24.3 & 23.5 & 22.1 \\
w4g128 (0.135) & 79.8 & 99.9 & 331 & 337 & 28.2 & 30.3 & 29.6 \\
w4a (0.147) & 199 & 273 & 431 & 438 & 76.3 & 94.2 & 110 \\
w4c (0.179) & 205 & 367 & 396 & 375 & 116 & 139 & 159 \\
w4t (0.369) & 405 & 407 & 382 & 318 & 205 & 235 & 268 \\


==> tables/bank/x6_deqlm.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X6.md; header: | cell (rel. err) | k=10 | k=30 | k=60 | median residual k=60 | cosine to fp32 k=60 |
fp32 & 91.2 & 24.48 & 23.14 & 2.5e-2 & 1 \\
noise 0.02 & 90.8 & 24.51 & 23.17 [23.16,23.17] & 2.5e-2 & 0.999 \\
noise 0.05 & 91.4 & 24.66 & 23.31 [23.30,23.32] & 2.5e-2 & 0.995 \\
noise 0.1 & 92.3 & 25.23 & 23.84 [23.82,23.86] & 2.4e-2 & 0.981 \\
noise 0.15 & 92.7 & 26.27 & 24.81 [24.79,24.84] & 2.4e-2 & 0.959 \\
noise 0.2 & 92.5 & 27.92 & 26.37 [26.35,26.40] & 2.4e-2 & 0.930 \\
noise 0.3 & 98.5 & 34.59 & 32.65 [32.63,32.70] & 2.3e-2 & 0.846 \\
noise 0.5 & 219 & 124.7 & 127.1 [124.2,132.0] & 2.9e-2 & 0.55 \\
noise 0.7 & 923 & 1071 & 1182 [1142,1204] & 6.1e-2 & 0.29 \\
noise 1.0 & 6181 & 7866 & 8059 [7547,9077] & 1.5e-1 & 0.14 \\
w8c (0.008) & 90.2 & 24.48 & 23.14 & 2.5e-2 & 1.000 \\
w4g32 (0.09) & 96.8 & 25.11 & 23.74 & 2.5e-2 & 0.984 \\
w4g128 (0.11) & 92.6 & 25.38 & 23.96 & 2.4e-2 & 0.978 \\
w4a (0.13) & 73.1 & 25.48 & 24.09 & 2.4e-2 & 0.971 \\
w4c (0.15) & 67.1 & 25.61 & 24.35 & 2.0e-2 & 0.956 \\
w4t (0.61) & 2556 & 2401 & 2395 & 5.2e-5 & 0.27 \\


==> tables/bank/x6_mdeq.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X6.md; header: | cell | k=8 | k=16 | k=26 (default) | k=100 | cos to fp32 eq. | converged (res<1e-2) @k=100 | median steps to 1e-2 |
fp32 & 72.2 & 73.9 & 73.8 & 73.8 & 1 & 99.7\% & 24 \\
noise 0.02 & 72.2 & 73.6 & 73.7 [73.5,73.8] & 73.7 & 0.996 & 99.7\% & 24 \\
noise 0.05 & 71.4 & 72.9 & 73.1 [72.7,73.7] & 73.0 & 0.978 & 99.7\% & 24 \\
noise 0.1 & 67.3 & 69.0 & 68.9 [67.1,70.7] & 68.9 & 0.923 & 99.8\% & 24 \\
noise 0.15 & 58.9 & 61.5 & 61.5 [59.2,64.3] & 61.5 & 0.855 & 99.8\% & 25 \\
noise 0.2 & 46.0 & 49.1 & 49.1 [47.1,52.9] & 49.1 & 0.779 & 99.8\% & 25 \\
noise 0.3 & 12.6 & 14.6 & 14.8 [10.5,18.4] & 14.8 & 0.614 & 99.8\% & 25 \\
noise 0.5 & 0.3 & 0.2 & 0.3 & 0.3 & 0.334 & 99.5\% & 26 \\
noise 0.7 / 1.0 & 0.1 & 0.1 & 0.1 & 0.1 & 0.18 / 0.08 & 99.7 / 99.4\% & 26 / 31 \\
w8c (0.009) & 72.2 & 74.0 & 73.8 & 73.8 & 0.999 & 99.7\% & 24 \\
w4a (0.137) & 66.1 & 67.9 & 67.9 & 68.0 & 0.901 & 99.8\% & 23 \\
w4g32 (0.107) & 64.8 & 66.6 & 66.6 & 66.5 & 0.882 & 99.6\% & 26 \\
w4g128 (0.137) & 59.1 & 61.3 & 61.5 & 61.6 & 0.852 & 99.3\% & 26 \\
w4c (0.171) & 56.2 & 58.0 & 57.8 & 57.9 & 0.850 & 99.5\% & 25 \\
w4t (0.408) & 0.2 & 0.2 & 0.2 & 0.2 & 0.540 & 99.9\% & 19 \\


==> tables/bank/x7_ladder.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X7.md; header: | cell | exact | cell acc | phi_H | rho_out | coherence | their Sudoku number (FP 84.1) |
fp32 & 71.4 & 88.2 & 1 & - & - & 84.1 \\
W8A8 per-tensor static & 70.9 [69.5-71.8] & 88.5 & 0.84 & 0.036 & 0.43 & Int8 84.0 \\
W4 per-tensor + A4 per-tensor static & 0.0 [0-0] & 49.9 & 0.19 & 0.466 & 0.55 & Int4 0.0 \\
W4 per-tensor + A4 per-tensor dynamic & 0.0 & 47.6 & 0.21 & 0.412 & 0.52 & 0.0 \\
W4 per-tensor + A4 per-token & 3.5 & 63.8 & 0.34 & 0.183 & 0.44 & 4.6 \\
W4 per-tensor + A4 group-32 & 5.3 & 65.4 & 0.31 & 0.137 & 0.40 & 14.5 \\
W4 per-tensor + A4 group-16 & 5.0 & 65.3 & 0.31 & 0.135 & 0.40 & 15.0 \\
W4 per-channel + A4 per-token & 20.5 & 75.3 & 0.50 & 0.116 & 0.39 & - \\
W4 group-32 + A4 group-32 & 66.6 & 86.6 & 0.87 & 0.045 & 0.38 & - \\
W4 MXInt4 + A4 MXInt4 & 65.4 & 86.2 & 0.84 & 0.066 & 0.40 & MXInt4 80.1 \\
weight-only W4 per-tensor / per-channel / g32 / MX & 5.9 / 67.9 / 69.0 / 69.8 &  &  & 0.131 / 0.058 / 0.031 / 0.047 &  & weight-only 78.5 \\
act-only A4 per-tensor static / dynamic / token / g32 / MX & 0.0 / 0.0 / 17.0 / 69.8 / 68.9 &  &  & 0.453 / 0.375 / 0.093 / 0.032 / 0.043 &  & - \\


==> tables/bank/x7_maze.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X7.md; header: | arm | 0.5 | 0.7 | 1.0 | 1.5 | sigma_1/2 exact | sigma_1/2 valid path | rho_1/2 |
\texttt{an} fresh zero-mean & 87.5 [87-88] & 85.5 [85-87] & 23.3 [23-24] & 0.0 & 0.897-0.902 & 1.20-1.21 & 0.198-0.199 \\
\texttt{af} fixed zero-mean & 77.7 [70-82] & 34.9 [20-48] & 0.0 & 0.0 & 0.60-0.73 & 0.78-0.83 & 0.13-0.16 \\
\texttt{ab} fixed sign-consistent bias & 86.1 [84-88] & 79.5 [72-84] & 9.3 [0-25] & 0.0 & 0.82-0.90 & 0.83-0.91 & 0.18-0.20 \\
\texttt{wn} weight noise & 87.7 [87-88] & - & 86.1 [85-87] & 27.1 [0-81] & 1.24-1.73 & 1.73-1.75 & 0.30-0.44 \\


==> tables/bank/x7_mlp.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X7.md; header: | arm | 0.1 | 0.15 | 0.2 | 0.3 | 0.5 | sigma_1/2 (3 draws) | rho_1/2 |
\texttt{an} fresh zero-mean (E\_t eps = 0) & 70.1 [70-70] & 67.4 [67-68] & 62.9 [63-63] & 32.9 [32-34] & 2.3 [2-2] & 0.287-0.293 & 0.080-0.082 \\
\texttt{af} fixed zero-mean (step-coherent) & 66.5 [66-67] & 58.6 [57-60] & 43.8 [41-46] & 10.4 [8-13] & 0.3 & 0.216-0.231 & 0.061-0.064 \\
\texttt{ab} fixed sign-consistent bias & 64.6 [62-67] & 46.5 [35-56] & 22.9 [10-31] & 3.7 [0-6] & 0.0 & 0.149-0.190 & 0.094-0.124 \\
\texttt{wn} weight noise, zero-mean & 64.9 [63-66] & 26.5 [24-31] & 5.5 [4-7] & 1.0 & 0.0 & 0.135-0.144 & 0.038-0.042 \\


==> tables/bank/x8_filter.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X8.md; header: | group (output length) | cells | exact unit: AUROC, best t, bal. acc | exact unit, one global t = 0.893 | cell unit: AUROC, best t, bal. acc | cell u
Sudoku, 3 models (81 cells) & 714 & 0.91, 0.845, 0.90 & 0.88 & 0.96, 0.892, 0.94 & 0.93 \\
Maze, TRM + HRM (900 cells) & 432 & 0.97, 0.981, 0.91 & 0.78 & 1.00, 0.942, 0.97 & 0.96 \\
DT maze 9 / 13 / 19 / 25 / 33 & 112-126 each & 0.99 / 0.91 / 0.94 / 0.89 / 0.91; t 0.971-0.976 & 0.88 / 0.70 / 0.62 / 0.60 / 0.59 & -- & -- \\
DT maze 25 / 33, per-cell reruns & 27 / 27 & 0.93 / 0.78; t 0.969 / 0.968 & -- & 1.00 / 1.00; t 0.936 / 0.931 & 1.00 / 1.00 \\


==> tables/bank/x8_ptrm.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X8.md; header: | model (deterministic acc) | noise | sigma | single rollout | pass@K | best-Q@K | mode@K |
TRM Sudoku-MLP (70.5), K=16 & PTRM kick on z\_L & 0.1 / 0.3 / 0.5 / 1.0 & 71.5 / 71.3 / 71.2 / 71.2 (sd 0.5-0.7) & 79.9 / 80.5 / 81.1 / 80.8 & = pass@K & 78.4-79.3 \\
 & ours, every linear input & 0.1 / 0.3 / 0.5 & 69.7 / 32.1 / 2.3 (sd 0.1-0.9) & 80.5 / 55.4 / 5.1 & 80.5 / 53.2 / 2.4 & 78.5 / 50.5 / 2.9 \\
TRM Sudoku-attn (65.9), K=16 & PTRM & 0.1 / 0.3 / 0.5 / 1.0 & 66.4 / 66.7 / 66.7 / 66.5 & 76.3 / 76.9 / 76.3 / 76.6 & = pass@K & 73.4-74.3 \\
 & ours & 0.1 / 0.3 / 0.5 / 1.0 & 66.7 / 64.1 / 45.2 / 0.0 & 77.2 / 77.7 / 58.4 / 0.0 & 77.2 / 77.7 / 58.3 / 0.0 & 75.4 / 73.9 / 54.6 / 0.0 \\
TRM Maze-attn (88.4, exact), K=8 & PTRM & 0.5 / 1.0 (0.3 at K=16) & 88.3 / 87.9 (88.4) & 89.0 / 88.8 (89.4) & 88.2 / 88.0 (88.8) & 88.4 / 88.0 \\
 & ours & 0.5 / 1.0 & 88.1 / 23.4 (sd 1.9) & 93.4 / 78.0 & 88.6 / 28.6 & 89.0 / 58.6 \\
Sudoku-MLP w4c (68.1), in basin & PTRM & 0.3 & 67.7 & 78.5 & 78.5 & 75.5 \\
Sudoku-MLP w3g32 (51.5), edge & PTRM & 0.3 & 51.0 & 66.7 & 66.0 & 59.8 \\


==> tables/bank/x8_rank.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X8.md; header: | detector | in basin (43 cells) | edge (26) | out of basin (19, of which 3 all-wrong) |
halting head (-q) & 1.00 & 0.96-1.00 & 0.80-1.00 (MLP w4t 0.80, w3c 0.87) \\
hand-coded checker (conflicts + given mismatches) & 1.00 & 1.00 & 1.00 (exact by construction: unique solutions; 0 disagreements with exact match in 88 cells) \\
min max-softmax over blanks & 0.99-1.00 & 0.95-1.00 & 0.90-1.00 \\
combined (logistic on fp32: head, residuals, max-softmax, margin) & 1.00 & 0.94-1.00 & 0.85-1.00 \\
first step with q > 0 (halt time) & 0.98-1.00 & 0.89-1.00 & 0.80-0.99 \\
convergence residual z\_H & 0.87-1.00 & 0.38-0.99 & 0.02-1.00 (attn out of basin 0.02-0.55: inverted) \\
path independence (rerun from z $\sim$ N(0,1)) & MLP 0.93-0.96; attn, HRM 0.44-0.66 & MLP 0.84-0.94 & MLP 0.83-0.87 \\
reference fidelity phi\_H per puzzle & 0.21-0.96 & 0.34-0.98 & 0.65-0.98 \\


==> tables/bank/x8_spearman.tex <==
% generated by tables/bank/md2tex.py from reports/edgetrm_exp/X8.md; header: | model | cells | in-basin | Spearman(phi, retained) all | in-basin (ret >= 0.9) | near-baseline (ret >= 0.97) | nsup 16 only, near-baseline |
TRM Sudoku-MLP & 253 & 114 & 0.92 [0.90, 0.94] & 0.46 [0.29, 0.63] & 0.29 [0.05, 0.51] (83) & 0.32 [-0.21, 0.70] (17) \\
TRM Sudoku-attn & 253 & 158 & 0.64 [0.53, 0.72] & 0.27 [0.08, 0.43] & 0.34 [0.16, 0.49] (125) & 0.34 [-0.01, 0.63] (38) \\
HRM Sudoku & 208 & 147 & 0.65 [0.54, 0.74] & 0.27 [0.09, 0.42] & 0.23 [0.04, 0.39] (121) & 0.33 [-0.04, 0.62] (28) \\
TRM Maze-attn & 214 & 177 & 0.79 [0.70, 0.85] & 0.63 [0.50, 0.74] & 0.59 [0.45, 0.71] (172) & 0.56 [0.29, 0.77] (52) \\
HRM Maze & 218 & 175 & 0.42 [0.28, 0.54] & -0.07 [-0.24, 0.11] & -0.25 [-0.42, -0.08] (154) & 0.05 [-0.30, 0.38] (48) \\


==> tables/tab_auroc_rows.tex <==
% AUROC for a wrong answer at supervision step 16: halting head / residual / fidelity-to-fp32; accuracy in parentheses; generated by plots/auroc_table.py --latex
fp32 & 1.00 / 0.99 / -- (71) & 1.00 / 0.94 / -- (66) & 0.67 / 0.53 / -- (88) & 1.00 / 0.99 / -- (49) & 0.69 / 0.73 / -- (75) \\
INT8 per-channel & 1.00 / 0.99 / 0.96 (71) & 1.00 / 0.92 / 0.76 (66) & 0.67 / 0.52 / 0.52 (88) & 1.00 / 0.99 / 0.96 (50) & 0.69 / 0.73 / 0.63 (75) \\
INT4 per-channel & 1.00 / 0.99 / 0.95 (68) & 1.00 / 0.91 / 0.36 (66) & 0.67 / 0.53 / 0.49 (88) & 1.00 / 0.99 / 0.93 (49) & 0.70 / 0.75 / 0.57 (75) \\
INT3 grouped & 0.99 / 0.85 / 0.48 (51) & 1.00 / 0.95 / 0.47 (65) & 0.68 / 0.49 / 0.58 (88) & 1.00 / 0.99 / 0.93 (47) & 0.63 / 0.73 / 0.74 (76) \\
INT4 per-tensor & 0.81 / 0.66 / 0.89 (6) & 1.00 / 0.88 / 0.45 (63) & 0.69 / 0.52 / 0.56 (87) & 1.00 / 0.98 / 0.92 (47) & 0.68 / 0.73 / 0.60 (76) \\
weight noise 0.1 & 1.00 / 0.99 / 0.95 (66) & 1.00 / 0.95 / 0.52 (67) & 0.65 / 0.49 / 0.48 (89) & 1.00 / 0.98 / 0.92 (50) & 0.68 / 0.74 / 0.65 (75) \\
weight noise 0.3 & 0.98 / 0.97 / 0.81 (1) & 1.00 / 0.90 / 0.35 (66) & -- & 1.00 / 1.00 / 0.92 (48) & -- \\
activation noise 0.3 & 0.96 / 0.90 / 0.62 (32) & 1.00 / 0.97 / 0.36 (64) & -- & 1.00 / 0.98 / 0.93 (45) & -- \\


==> tables/tab_depth_matrix.tex <==
% depth table: gap to fp32 (points) at supervision steps 4 and 32 per model; TRM H=3, HRM H=2; generated by plots/depth_table.py --matrix
fp32 (accuracy) & 61.0 & 74.2 & 52.5 & 69.7 & 87.0 & 87.1 & 30.8 & 51.7 & 73.8 & 74.0 \\
\midrule
INT8 per-channel & ${+}0.8$ & ${-}0.4$ & ${+}0.0$ & ${+}0.7$ & ${+}0.1$ & ${+}0.0$ & ${+}0.1$ & ${+}0.8$ & ${+}0.0$ & ${+}0.3$ \\
INT4 grouped (128) & ${-}1.4$ & ${-}2.9$ & ${-}0.3$ & ${+}0.4$ & ${+}0.0$ & ${-}0.1$ & ${+}0.4$ & ${+}0.2$ & ${-}0.3$ & ${+}0.2$ \\
INT4 per-channel & ${-}1.6$ & ${-}3.9$ & ${-}1.3$ & ${-}0.1$ & ${-}0.1$ & ${-}0.1$ & ${-}0.3$ & ${+}0.3$ & ${+}0.4$ & ${+}0.8$ \\
INT4 per-tensor & ${-}56.0$ & ${-}68.5$ & ${-}7.9$ & ${-}4.1$ & ${-}0.9$ & ${-}0.8$ & ${-}1.7$ & ${-}0.9$ & ${+}0.5$ & ${+}0.7$ \\


==> tables/tab_depth_rows.tex <==
% depth-flat table: fp32 and quantized exact accuracy at steps 1 and 16, and the gap at each; generated by plots/depth_table.py --latex
TRM Sudoku, MLP & INT8 per-channel & 28.4 & 28.3 & -0.1 & 71.4 & 71.0 & -0.4 \\
TRM Sudoku, MLP & INT4 grouped (128) & 28.4 & 25.9 & -2.5 & 71.4 & 68.4 & -3.0 \\
TRM Sudoku, MLP & INT4 per-channel & 28.4 & 23.4 & -5.0 & 71.4 & 67.9 & -3.5 \\
TRM Sudoku, MLP & INT4 per-tensor & 28.4 & 2.1 & -26.3 & 71.4 & 5.9 & -65.5 \\
TRM Sudoku, MLP & INT4 per-channel + INT8 act. & 28.4 & 13.1 & -15.3 & 71.4 & 68.7 & -2.7 \\
TRM Sudoku, attn & INT8 per-channel & 3.1 & 3.1 & +0.0 & 65.7 & 65.9 & +0.2 \\
TRM Sudoku, attn & INT4 grouped (128) & 3.1 & 2.5 & -0.6 & 65.7 & 66.3 & +0.6 \\
TRM Sudoku, attn & INT4 per-channel & 3.1 & 2.3 & -0.8 & 65.7 & 66.2 & +0.5 \\
TRM Sudoku, attn & INT4 per-tensor & 3.1 & 1.8 & -1.3 & 65.7 & 62.8 & -2.9 \\
TRM Sudoku, attn & INT4 per-channel + INT8 act. & 3.1 & 2.2 & -0.9 & 65.7 & 66.7 & +1.0 \\
TRM Maze & INT8 per-channel & 78.5 & 78.4 & -0.1 & 87.0 & 87.1 & +0.1 \\
TRM Maze & INT4 grouped (128) & 78.5 & 78.1 & -0.4 & 87.0 & 87.0 & +0.0 \\
TRM Maze & INT4 per-channel & 78.5 & 78.3 & -0.2 & 87.0 & 86.9 & -0.1 \\
TRM Maze & INT4 per-tensor & 78.5 & 76.6 & -1.9 & 87.0 & 86.2 & -0.8 \\
TRM Maze & INT4 per-channel + INT8 act. & 78.5 & 78.1 & -0.4 & 87.0 & 87.1 & +0.1 \\
HRM Sudoku & INT8 per-channel & 1.3 & 1.3 & +0.0 & 49.2 & 49.5 & +0.3 \\
HRM Sudoku & INT4 grouped (128) & 1.3 & 1.2 & -0.1 & 49.2 & 47.7 & -1.5 \\
HRM Sudoku & INT4 per-channel & 1.3 & 1.0 & -0.3 & 49.2 & 48.9 & -0.3 \\
HRM Sudoku & INT4 per-tensor & 1.3 & 1.0 & -0.3 & 49.2 & 46.9 & -2.3 \\
HRM Sudoku & INT4 per-channel + INT8 act. & 1.3 & 1.0 & -0.3 & 49.2 & 48.9 & -0.3 \\
HRM Maze & INT8 per-channel & 16.4 & 16.3 & -0.1 & 74.3 & 74.3 & +0.0 \\
HRM Maze & INT4 grouped (128) & 16.4 & 16.0 & -0.4 & 74.3 & 74.5 & +0.2 \\
HRM Maze & INT4 per-channel & 16.4 & 16.5 & +0.1 & 74.3 & 74.6 & +0.3 \\
HRM Maze & INT4 per-tensor & 16.4 & 16.5 & +0.1 & 74.3 & 75.0 & +0.7 \\


==> tables/tab_gran_released.tex <==
% Part A: released checkpoints at step 16: fp32, INT4 per-tensor, per-channel, grouped-128; generated by plots/granularity_table.py --latex
TRM Sudoku, MLP & 71.4 & 5.9 & 67.9 & 68.4 \\
TRM Sudoku, attn & 65.7 & 62.8 & 66.2 & 66.3 \\
TRM Maze & 87.0 & 86.2 & 86.9 & 87.0 \\
HRM Sudoku & 49.2 & 46.9 & 48.9 & 47.7 \\
HRM Maze & 74.3 & 75.0 & 74.6 & 74.5 \\


==> tables/tab_gran_variants_rows.tex <==
% trained Sudoku variants (step 65,100): mixer, width, seed, fp32, INT4 per-tensor, INT4 per-channel, sigma_1/2 (median of three draws); copied from tables/tab_granularity_rows.tex Part B (generated by EdgeTRM/plots/granularity_table.py --latex)
attention & 256 & 0 & 10.4 & 0.2 & 10.1 & 0.5 \\
attention & 256 & 1 & 17.2 & 1.5 & 14.2 & 0.3 \\
attention & 256 & 2 & 28.2 & 5.7 & 27.1 & 0.3 \\
attention & 512 & 0 & 64.8 & 65.5 & 66.3 & >0.7 \\
attention & 512 & 1 & 62.9 & 59.5 & 61.8 & 0.7 \\
attention & 512 & 2 & 53.4 & 17.7 & 53.0 & 0.7 \\
MLP & 256 & 0 & 59.9 & 0.0 & 59.4 & 0.15 \\
MLP & 256 & 1 & 62.3 & 0.0 & 61.1 & 0.15 \\
MLP & 256 & 2 & 64.0 & 0.0 & 61.4 & 0.15 \\
MLP & 512 & 0 & 83.6 & 3.0 & 81.9 & 0.2 \\
MLP & 512 & 1 & 82.5 & 2.6 & 81.6 & 0.2 \\
MLP & 512 & 2 & 84.2 & 1.2 & 83.0 & 0.15 \\
MLP & 768 & 0 & 75.3 & 6.2 & 74.1 & 0.2 \\


==> tables/tab_granularity_rows.tex <==
% Part A: released checkpoints at step 16: fp32, INT4 per-tensor, per-channel, grouped-128; generated by plots/granularity_table.py --latex
TRM Sudoku, MLP & 71.4 & 5.9 & 67.9 & 68.4 \\
TRM Sudoku, attn & 65.7 & 62.8 & 66.2 & 66.3 \\
TRM Maze & 87.0 & 86.2 & 86.9 & 87.0 \\
HRM Sudoku & 49.2 & 46.9 & 48.9 & 47.7 \\
HRM Maze & 74.3 & 75.0 & 74.6 & 74.5 \\
% Part B: trained Sudoku variants (step 65,100): mixer, width, seed, fp32, INT4 per-tensor, INT4 per-channel, sigma at which the median of three noise draws halves
attention & 256 & 0 & 10.4 & 0.2 & 10.1 & 0.5 \\
attention & 256 & 1 & 17.2 & 1.5 & 14.2 & 0.3 \\
attention & 256 & 2 & 28.2 & 5.7 & 27.1 & 0.3 \\
attention & 512 & 0 & 64.8 & 65.5 & 66.3 & >0.7 \\
attention & 512 & 1 & 62.9 & 59.5 & 61.8 & 0.7 \\
attention & 512 & 2 & 53.4 & 17.7 & 53.0 & 0.7 \\
MLP & 256 & 0 & 59.9 & 0.0 & 59.4 & 0.15 \\
MLP & 256 & 1 & 62.3 & 0.0 & 61.1 & 0.15 \\
MLP & 256 & 2 & 64.0 & 0.0 & 61.4 & 0.15 \\
MLP & 512 & 0 & 83.6 & 3.0 & 81.9 & 0.2 \\
MLP & 512 & 1 & 82.5 & 2.6 & 81.6 & 0.2 \\
MLP & 512 & 2 & 84.2 & 1.2 & 83.0 & 0.15 \\
MLP & 768 & 0 & 75.3 & 6.2 & 74.1 & 0.2 \\


==> tables/tab_mixer_rows.tex <==
% trained Sudoku models, one row per mixer and width, seeds as s0 / s1 / s2: fp32, INT4 per-tensor, weight-noise sigma at which the median of three draws halves; generated by plots/granularity_table.py --mixer
MLP & 256 & 59.9 / 62.3 / 64.0 & 0.0 / 0.0 / 0.0 & 0.15 / 0.15 / 0.15 \\
MLP & 512 & 83.6 / 82.5 / 84.2 & 3.0 / 2.6 / 1.2 & 0.2 / 0.2 / 0.15 \\
MLP & 768 & 75.3 & 6.2 & 0.2 \\
attention & 256 & 10.4 / 17.2 / 28.2 & 0.2 / 1.5 / 5.7 & 0.5 / 0.3 / 0.3 \\
attention & 512 & 64.8 / 62.9 / 53.4 & 65.5 / 59.5 / 17.7 & >0.7 / 0.7 / 0.7 \\

